Approximate Byzantine Fault-Tolerance in Distributed Optimization

This paper considers the problem of Byzantine fault-tolerance in distributed multi-agent optimization. In this problem, each agent has a local cost function, and in the fault-free case, the goal is to design a distributed algorithm that allows all the agents to find a minimum point of all the agents' aggregate cost function. We consider a scenario where some agents might be Byzantine faulty that renders the original goal of computing a minimum point of all the agents' aggregate cost vacuous. A more reasonable objective for an algorithm in this scenario is to allow all the non-faulty agents to compute the minimum point of only the non-faulty agents' aggregate cost. Prior work shows that if there are up to $f$ (out of $n$) Byzantine agents then a minimum point of the non-faulty agents' aggregate cost can be computed exactly if and only if the non-faulty agents' costs satisfy a certain redundancy property called $2f$-redundancy. However, $2f$-redundancy is an ideal property that can be satisfied only in systems free from noise or uncertainties, which can make the goal of exact fault-tolerance unachievable in some applications. Thus, we introduce the notion of $(f,\epsilon)$-resilience, a generalization of exact fault-tolerance wherein the objective is to find an approximate minimum point of the non-faulty aggregate cost, with $\epsilon$ accuracy. This approximate fault-tolerance can be achieved under a weaker condition that is easier to satisfy in practice, compared to $2f$-redundancy. We obtain necessary and sufficient conditions for achieving $(f,\epsilon)$-resilience characterizing the correlation between relaxation in redundancy and approximation in resilience. In case when the agents' cost functions are differentiable, we obtain conditions for $(f,\epsilon)$-resilience of the distributed gradient-descent method when equipped with robust gradient aggregation.

==> algorithm-backup.tex <==
\begin{lemma}
    If the cost functions of agents satisfy $(2f,\epsilon)$-redundancy then
    \begin{equation*}
        ...
    \end{equation*}
\end{lemma}

\begin{proof}
    For any two agents $i$ and $j$, consider the two sets $S_1$ and $S_2$ where $S_1\backslash\{i\}=S_2\backslash\{j\}$. By $(2f,\epsilon)$-redundancy, for all 
    \begin{equation*}
        x_1\in\arg\min_x\sum_{k\in S_1}Q_k(x),
    \end{equation*}\
    we have $x_1\in B(x^*,\epsilon)$. Therefore, 
    \begin{equation*}
        \sum_{k\in S_1}\nabla Q_k(x_1)=0.
    \end{equation*}
    Similarly,
    \begin{gather}
        x_2\in B(x^*,\epsilon),~\forall x_2\in\arg\min_x\sum_{k\in S_2}Q_k(x), \\
        \sum_{k\in S_2}\nabla Q_k(x_2)=0.
    \end{gather}
    By Assumption~\ref{assum:lipschitz},
    \begin{equation*}
        \begin{aligned}
            \norm{\nabla Q_k(x_1)-\nabla Q_k(x^*)}\leq\mu\norm{x_1-x^*}\leq\mu\epsilon,~\forall k, \\
            \norm{\nabla Q_k(x_2)-\nabla Q_k(x^*)}\leq\mu\norm{x_2-x^*}\leq\mu\epsilon,~\forall k.
        \end{aligned}
        \label{eqn:lipschitz-on-minima}
    \end{equation*}
    By \eqref{eqn:lipschitz-on-minima} and triangle inequality,
    \begin{align}
        %\norm{\sum_{k\in S_1}\nabla Q_k(x^*)-\sum_{k\in S_2}\nabla Q_k(x^*)}&=
         &\norm{\nabla Q_i(x^*) - \nabla Q_j(x^*)} \nonumber \\
        =& \norm{\nabla Q_i(x^*)+\nabla Q_i(x_1)-\nabla Q_i(x_1) - \nabla Q_j(x^*) + \nabla Q_j(x_2) - \nabla Q_j(x_2)} \nonumber \\
        =& \norm{\left[\nabla Q_i(x^*)-\nabla Q_i(x_1)\right]-\left[\nabla Q_j(x^*)-\nabla Q_j(x_2)\right]+\left[\nabla Q_i(x_1)-\nabla Q_j(x_2)\right]} \nonumber \\
        \leq& \norm{\nabla Q_i(x^*)-\nabla Q_i(x_1)}+\norm{\nabla Q_j(x^*)-\nabla Q_j(x_2)}+\norm{\nabla Q_i(x_1)-\nabla Q_j(x_2)} \nonumber \\
        \leq&\,2\mu\epsilon+\norm{\nabla Q_i(x_1)-\nabla Q_j(x_2)}.
        \label{eqn:tri-ineq-1}
    \end{align}
    Similarly,
    \begin{align}
        %\norm{\sum_{k\in S_1}\nabla Q_k(x^*)-\sum_{k\in S_2}\nabla Q_k(x^*)}&=
         &\norm{\nabla Q_i(x_1) - \nabla Q_j(x_2)} \nonumber \\
        =& \norm{\nabla Q_i(x_1)+\nabla Q_i(x^*)-\nabla Q_i(x^*) - \nabla Q_j(x_2) + \nabla Q_j(x^*) - \nabla Q_j(x^*)} \nonumber \\
        \leq& \norm{\nabla Q_i(x_1)-\nabla Q_i(x^*)}+\norm{\nabla Q_j(x_2)-\nabla Q_j(x^*)}+\norm{\nabla Q_i(x^*)-\nabla Q_j(x^*)} \nonumber \\
        \leq&\,2\mu\epsilon+\norm{\nabla Q_i(x^*)-\nabla Q_j(x^*)}.
        \label{eqn:tri-ineq-2}
    \end{align}
    Combine \eqref{eqn:tri-ineq-1} and \eqref{eqn:tri-ineq-2}, we have
    \begin{equation*}
        ?
    \end{equation*}
\end{proof}


==> algorithm.tex <==
\section{Distributed Gradient-Descent (DGD) Method}
\label{sec:grad_des}

In this section, we consider a setting wherein the non-faulty agents' cost functions are differentiable. In this particular case, we study the approximate fault-tolerance of the distributed gradient-descent method coupled with a {\em gradient-filter}, described below. We consider the server-based system architecture, shown in Fig.~\ref{fig:sys}, assuming a synchronous system.\\

The DGD method is an iterative algorithm wherein the server maintains an {\em estimate} of a minimum point, and 
% point that  minimum point $x^*$ of the non-faulty agents' aggregate cost function $\sum_{i \in \H} Q_i(x)$, and 
updates it iteratively using gradients sent by the agents. Specifically, in each iteration $t \in \{0, \, 1, \ldots \}$, the server starts with an estimate $x^t$ and broadcasts to all the agents. Each non-faulty agent $i$ sends back to the sever the gradient of its cost function at $x^t$, i.e., $\nabla Q_i(x^t)$. However, Byzantine faulty agents may send arbitrary incorrect vectors as their gradients to the server. The initial estimate, named $x^0$, is chosen arbitrarily by the server. \\

A {\em gradient-filter} is a vector function, denoted by $\gf$, that maps the $n$ gradients received by the server from all the $n$ agents to a $d$-dimensional vector, i.e., $\gf: \R^{d \times n} \to \R^d$. For example, an average of all the gradients as in the case of the traditional distributed gradient-descent method is technically a gradient-filter. However, averaging is not quite robust against Byzantine faulty agents~\cite{blanchard2017machine, su2016fault}. The real purpose of a gradient-filter is to mitigate the detrimental impact of incorrect gradients sent by the Byzantine faulty agents. In other words, a gradient-filter {\em robustifies} the traditional gradient-descent method against Byzantine faults. We show that if a gradient-filter satisfies a certain property then it can confer fault-tolerance to the distributed gradient-descent method.\\

We first formally describe below the steps in each iteration of the distributed gradient-descent method implemented on a synchronous server-based system. Note that we constrain the estimates computed by the server to a compact convex set $\W \subset \R^d$. The set $\W$ can be arbitrarily large. For a vector $x \in \R^d$, its projection onto $\W$, denoted by $[x]_\W$, is defined to be                                   
\begin{align}
    [x]_\W = \arg \min_{y \in \W} \norm{x - y}. \label{eqn:proj_W}
\end{align}
As $\W$ is compact and convex set, $[x]_\W$ is unique for each $x$ (see~\cite{boyd2004convex}).
% , and a minimum point of the aggregate cost function corresponding to a set of $n-f$ non-faulty agents is bounded or finite, i.e., there exists a compact convex set $\W \subset \R^d$ (arbitrarily large) containing minimum points of the aggregate of $n-f$ non-faulty agents' cost functions.
% Here, we present its fault-tolerance property under the weaker condition of $(2f, \, \epsilon)$-redundancy. \\

% \subsection{Algorithm description}

% Assuming a synchronous distributed system, we adopt the algorithm proposed in \cite{gupta2020fault}, described below:

% hypercube $\W$ of finite dimensions containing a true minimum point. Note that $\W$ is a compact convex set and therefore, projection onto $\W$ is uniquely defined~\cite{boyd2004convex}. For a point $x \in \R^d$, suppose $[x]_\W$ denotes its projection onto $\W$, then
% \begin{align}
%     [x]_\W = \arg \min_{y \in \W} \norm{x - y}. \label{eqn:proj_W}
% \end{align}
% For a vector $v \in \R^d$, let $v[l]$ denote the $l$-th element of $v$. Now, without any loss of generality, let
% \[\W = \left(w \in \R^d ~ \vline ~ w[l] \in [a_l, ~ b_l], ~ a_l < b_l, ~ l = 1, \ldots, \, d \right).\]
% Thus, from~\eqref{eqn:proj_W}, we obtain that, for all $x \in \R^d$ and $l \in \{1, \ldots, \, d\}$,
% \begin{align}
%     [x]_\W[l] = [x]_{[a_l, \, b_l]} = \left\{ \begin{array}{ccc} b_l & , & x \geq b_l \\ x & , & a_l < x < b_l \\ a_l & , & x \leq a_l \end{array}\right.
% \end{align}
% ~


% \noindent\textbf{Steps performed in the $t$-th iteration, $t\geq0$:}

\subsection{Steps in $t$-th iteration}
\label{sub:steps}

In each iteration $t \in \{0, \,1 , \ldots\}$ the server updates its current estimate $x^t$ to $x^{t+1}$ using Steps {S1} and {S2} described as follows. 

\begin{enumerate}[label=\textbf{S\arabic*:}]
    \item The server requests from each agent the gradient of its local cost function at the current estimate $x^t$. Each non-faulty agent $i$ will then send to the server the gradient $\nabla Q_i(x^t)$, whereas a faulty agent may send an incorrect arbitrary value for the gradient.
    
    The gradient received by the server from agent $i$ is denoted as $g_i^t$. If no gradient is received from some agent $i$, agent $i$ must be faulty (because the system is assumed to be synchronous) -- in this case, the server eliminates the agent $i$ from the system, updates the values of $n$, $f$, and re-assigns the agents indices from $1$ to $n$.
    
    % assumes a default value of $\boldsymbol{0}$ vector for the missing gradient $g_i^t$.
    \item \textbf{[Gradient-filtering]} The server applies a gradient-filter $\gf$ to the $n$ received gradients and computes $\gf\left(g^t_1, \ldots, \, g^t_n\right) \in \R^d$. Then, the server updates its estimate to
    \begin{equation}
        x^{t+1}=\left[x^t-\eta_t \, \gf\left(g^t_1, \ldots, \, g^t_n\right) \right]_\W \label{eqn:update}
        % =\left[x^t-\eta_t\sum_{j=1}^{n-f}g_{i_j}^t\right]_\W,
    \end{equation}
    where $\eta_t$ is the step-size of positive value for iteration $t$.
    % , and $\W$ is a hypercube that contains $x^*\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in\H}Q_i(x)$, and $[\,\cdot\,]_{\mathcal{W}}$ denotes a projection onto $\mathcal{W}$.
\end{enumerate}

We propose, in Theorem~\ref{thm:upper-bound-D}, a generic convergence result for the above algorithm. 
% Then, we present its fault-tolerance property for certain specific gradient-filters, under the $(2f, \, \epsilon)$-redundancy and other standard assumptions. 

\begin{theorem}
% [\cite{bottou1998online}]
\label{thm:upper-bound-D}
    Consider the update law~\eqref{eqn:update} in the above iterative algorithm, with diminishing step-sizes $\{\eta_t, \, t = 0, \, 1, \ldots \}$ satisfying $\sum_{t=0}^{\infty}\eta_t=\infty\textrm{ and }\sum_{t=0}^{\infty}\eta_t^2<\infty$.
    % \begin{equation*}
    %     \sum_{t=0}^{\infty}\eta_t=\infty\textrm{ and }\sum_{t=0}^{\infty}\eta_t^2<\infty.
    % \end{equation*}
    Suppose that $\norm{\gf \left(g^t_1, \ldots, \, g^t_n\right)} < \infty$ for all $t$. For some point $x^* \in \W$, if there exists real-valued constants $\D^*\in[0,\max_{x\in\mathcal{W}}\norm{x-x^*})$ and $\xi > 0$ such that for each iteration $t$,
    \begin{equation}
        \phi_t=\iprod{x^t-x^*}{\gf \left(g^t_1, \ldots, \, g^t_n\right)} \geq \xi \textrm{ when }\norm{x^t-x^*} \geq \D^*, \label{eqn:lem_cond}
    \end{equation}
    then $\lim_{t\rightarrow\infty}\norm{x^t - x^*} \leq \D^*$.
    % \begin{equation*}
    %     \lim_{t\rightarrow\infty}\norm{x^t - x^*}\leq\D^*.
    % \end{equation*}
\end{theorem}

The values $\D^*$ and $\xi$ in Theorem~\ref{thm:upper-bound-D} may be interdependent. Proof of Theorem~\ref{thm:upper-bound-D} is deferred to Appendix \ref{apdx:lemma-uppr-bnd-D}. \\

Using Theorem~\ref{thm:upper-bound-D} we can obtain conditions under which a gradient-filter guarantees the approximate fault-tolerance property of $(f, \, \epsilon)$-resilience with $\epsilon \geq 0$, of which exact fault-tolerance is a special case. On the other hand, the prior results on the convergence of DGD method with a gradient-filter, e.g., see~\cite{blanchard2017machine, guerraoui2018hidden}, apply  only to exact fault-tolerance.\\

We demonstrate below the utility of Theorem~\ref{thm:upper-bound-D} to obtain the fault-tolerance properties of two commonly used gradient-filters; namely {\em Comparative Gradient Elimination}~\cite{gupta2020byzantine} and {\em Coordinate-Wise Trimmed Mean}~\cite{su2018finite}.
% , and present their approximate fault-tolerance properties. 

\subsection{Gradient-Filters and their Fault-Tolerance Properties}
\label{sec:grad_filters}

In this subsection, we present precise approximate fault-tolerance properties of two specific gradient-filters; the Comparative Gradient Elimination (CGE)~\cite{gupta2020byzantine, gupta2019byzantine}, and the Coordinate-Wise Trimmed Mean (CWTM)~\cite{su2018finite, yin2018byzantine}. Note that differentiability of non-faulty agents' cost functions, which is already assumed for the DGD method, implies Assumption~\ref{asp:exists} (see~\cite{boyd2004convex}). We additionally make Assumptions~\ref{assum:lipschitz},~\ref{assum:strongly-convex} and~\ref{assum:compact} about the non-faulty agents' cost functions. Similar assumptions are made in prior work on fault-free distributed optimization~\cite{bertsekas1989parallel, boyd2011distributed, nedic2009distributed}. 

% the assumption that $f < n/2$ is implicit in the $(2f, \, \epsilon)$-redundancy property, and need not be stated explicitly.

\begin{assumption}[Lipschitz smoothness]
    \label{assum:lipschitz}
    For each non-faulty agent $i$, we assume that the gradient of its cost function $\nabla Q_i(x)$ is Lipschitz continuous, i.e., there exists a finite real value $\mu>0$ such that 
    \begin{equation*}
        \norm{\nabla Q_i(x)-\nabla Q_i(x')}\leq\mu\norm{x-x'}, \quad \forall x,x' \in \W.
    \end{equation*}
\end{assumption}
% We let $\H$ denote the set of all the non-faulty agents in an execution of the above algorithm. Recall that $\mnorm{\H} \geq n-f$. Also, note that differentiability of the cost functions automatically implies Assumption~\ref{asp:exists}.

\begin{assumption}[Strong convexity]
    \label{assum:strongly-convex}
    For a non-empty set of non-faulty agents $\H$, let $Q_{\H}(x)$ denote the average cost function of the agents in $\H$, i.e.,
    \begin{equation*}
        Q_{\H}(x)=\frac{1}{\mnorm{\H}}\sum_{i\in\H}Q_i(x).
    \end{equation*}
    For each such set $\H$ with $\mnorm{\H} = n-f$, we assume that $Q_{\H}(x)$ is strongly convex, i.e., there exists a finite real value $\gamma > 0$ such that
    \begin{equation*}
        \iprod{\nabla Q(x)-\nabla Q(x')}{x-x'}\geq\gamma\norm{x-x'}^2, \quad \forall x,x' \in \W.
    \end{equation*}
\end{assumption}

Note that, under Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex}, $\gamma \leq \mu$. This inequality is proved in Appendix~\ref{app:gamma_mu}.
Now, recall that the iterative estimates of the algorithm in Section~\ref{sub:steps} are constrained to a compact convex set $\W \subset \R^d$.

\begin{assumption}[Existence]
    For each set of non-faulty agents $\H$ with $\mnorm{\H} = n-f$, we assume that there exists a point $x_{\H} \in \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x)$ such that $x_{\H} \in \W$.
    % \[x_{\H} \in \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x)\]
    % such that $x_{\H} \in \W$. 
    \label{assum:compact}
\end{assumption}

We describe below the CGE and CWTM gradient-filters. Later, we obtain the fault-tolerance properties of these filters using the result stated in Theorem~\ref{thm:upper-bound-D}, under $(2f, \, \epsilon)$-redundancy.\\

% \noindent \fbox{\begin{minipage}{0.98\textwidth}
% \subsubsection{CGE Gradient-Filter}
% \label{sub:cge}
{\bf CGE Gradient-Filter:} To apply the CGE gradient-filter in Step S2, the server sorts the $n$ gradients received from the $n$ agents at the completion of Step S1 as per their Euclidean norms (ties broken arbitrarily):
\begin{equation*}
    \norm{g_{i_1}^t}\leq \ldots \leq \norm{g_{i_{n-f}}^t} \leq \norm{g_{i_{n-f+1}}^t}\leq \ldots \leq \norm{g_{i_n}^t}.
\end{equation*}
That is, the gradient with the smallest norm, $g_{i_1}^t$, is received from agent $i_1$, and the gradient with the largest norm, $g_{i_n}^t$, is received from agent $i_n$. Then, the output of the CGE gradient-filter is the vector sum of the $n-f$ gradients with smallest $n-f$ Euclidean norms. Specifically,
\begin{align}
    \gf\left(g^t_1, \ldots, \, g^t_n \right) = \sum_{j=1}^{n-f}g_{i_j}^t. \label{eqn:cge_gf}
\end{align}
% \end{minipage}}
~

{\bf CWTM Gradient-Filter:} To implement this particular gradient-filter in Step S2, the server sorts the $n$ gradients received from the $n$ agents at the completion of Step S1 as per their individual elements. For a vector $v \in \R^d$, we let $v[k]$ denote its $k$-th element. Specifically, for each $k \in \{1, \ldots, \, d\}$, the server sorts the $k$-th elements of the gradients by breaking ties arbitrarily:
\begin{equation*}
    g_{i_1[k]}^t[k] \leq \ldots \leq g_{i_{f + 1}[k]}^t[k] \leq \ldots \leq g_{i_{n-f}[k]}^t[k] \leq  \ldots \leq g_{i_n[k]}^t[k].
\end{equation*}
The gradient with the smallest of the $k$-th element, $g_{i_1[k]}^t$, is received from agent $i_1[k]$, and the gradient with the largest of the $k$-th element, $g_{i_n[k]}^t$, is received from agent $i_n[k]$. For each $k$, the server eliminates the largest $f$ and the smallest $f$ of the $k$-th elements of the gradients received. Then, the output of the CWTM gradient-filter is a vector whose $k$-th element is equal to the average of the remaining $n-2f$ gradients' $k$-th elements. That is, for each $k \in \{1, \ldots, \, d\}$,
\begin{align}
    \gf\left(g^t_1, \ldots, \, g^t_n \right)[k] = \frac{1}{n-2f}\sum_{j=f+1}^{n-f}g_{i_j[k]}^t[k]. \label{eqn:cwtm_gf}
\end{align}
% \end{minipage}}
~

We present the precise fault-tolerance properties of the two gradient-filters in Theorems~\ref{thm:conv-guarantee} and~\ref{thm:conv-guarantee_cwtm} below. However, the {\bf reader may skip to Section~\ref{sec:experiments} without loss of continuity}. Proofs of the theorems are deferred to Appendices~\ref{app:proof_1} and~\ref{app:proof_2}, respectively. \\

% To present the formal result we define below some parameters. 

% \begin{itemize}
% \setlength{\itemsep}{0.3em}
%     \item We define a \textit{fault-tolerance margin}
%     \begin{equation}
%         \alpha = 1-\dfrac{f}{n}\left(1+\dfrac{2\mu}{\gamma}\right) \label{eqn:alpha}
%     \end{equation}
%     that determines the maximum fraction of Byzantine faulty agents that can be tolerated in an execution of the algorithm.
%     \item We define a coefficient

% that measures the resilience of the algorithm.
% \end{itemize}

% Both $\alpha$ and $\D$ depend upon $f$, the most number of Byzantine faulty agents in any given execution of the algorithm. 
% We present below in Theorem~\ref{thm:conv-guarantee} the {\bf approximation fault-tolerance property of the algorithm} described above in Section~\ref{sub:steps}. Then, we discuss the impact of $f$ on the approximation accuracy of fault-tolerance obtained. 
Note that, under Assumptions~\ref{assum:strongly-convex} and~\ref{assum:compact}, for each non-empty set of non-faulty agents $\H$ with $\mnorm{\H} = n-f$, the aggregate cost function $\sum_{i \in \H} Q_i(x)$ has a unique minimum point, denoted by $x_{\H}$, in the set $\W$. Specifically,
\begin{align}
    \left\{x_{\H}\right\} = \W \cap \arg \min_{x \in \R^d}\sum_{i \in \H} Q_i(x).  \label{eqn:uniq_min}
\end{align}
We first show below, in Theorem~\ref{thm:conv-guarantee}, that when the fraction of Byzantine faulty agents $f/n$ is bounded then the DGD method with the CGE gradient-filter is $(f, \, \O(\epsilon))$-resilient, under $(2f, \,\epsilon)$-redundancy and the above assumptions. 

\begin{theorem}
    \label{thm:conv-guarantee}
    Suppose that the non-faulty agents' cost functions satisfy the $(2f, \, \epsilon)$-redundancy property, and the Assumptions~\ref{assum:lipschitz},~\ref{assum:strongly-convex} and~\ref{assum:compact} hold true. Consider the algorithm in Section~\ref{sub:steps} with the CGE gradient-filter defined in~\eqref{eqn:cge_gf}. The following holds true:
    
    \begin{enumerate}
        \item $\norm{\gf \left(g^t_1, \ldots, \, g^t_n\right)} < \infty$ for all $t$.
        \item If
            \begin{equation}
                \alpha = 1-\dfrac{f}{n}\left(1+\dfrac{2\mu}{\gamma}\right) > 0 \label{eqn:alpha}
            \end{equation}
            then for each set of $n-f$ non-faulty agents $\H$, for each $\delta > 0$,
            \begin{align*}
                & \phi_t =\iprod{x^t-x_{\H}}{\gf \left(g^t_1, \ldots, \, g^t_n\right)} \geq \alpha \, n \gamma \, \delta \left( \left( \dfrac{4\mu f}{ \alpha \,  \gamma} \right)\, \epsilon + \delta \right) \\
                & \textrm{ when }\norm{x^t-x^*} \geq \left( \dfrac{4\mu f}{ \alpha \,  \gamma} \right)\, \epsilon + \delta. 
            \end{align*}
    \end{enumerate}
    
    % , and diminishing step-sizes $\{\eta_0, \eta_1, \ldots \}$ in~\eqref{eqn:update} satisfying: $\sum_{t=1}^{\infty}\eta_t=\infty$ and $\sum_{t=1}^{\infty}\eta_t^2 < \infty$. 
    
\end{theorem}
~

% Proof of Theorem~\ref{thm:conv-guarantee} is deferred to Appendix~\ref{app:proof_1}. 
Let $\H$ denote an arbitrary set of $n-f$ non-faulty agents. If the step-size $\eta_t$ in~\eqref{eqn:update} is diminishing, i.e., $\sum_{t=0}^{\infty}\eta_t=\infty\textrm{ and }\sum_{t=0}^{\infty}\eta_t^2<\infty$, then Theorem~\ref{thm:conv-guarantee}, in conjunction with Theorem~\ref{thm:upper-bound-D} implies that, under the said conditions, 
\begin{equation*}
    \lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \leq \left( \dfrac{4\mu f}{ \alpha \,  \gamma} \right)\, \epsilon + \delta, \quad \forall \delta > 0.
\end{equation*}
The above implies that $\lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \leq \left( 4 \mu f/ \alpha \gamma \right) \, \epsilon$. Thus, Theorem~\ref{thm:conv-guarantee} shows that under $(2f, \, \epsilon)$-redundancy, and Assumptions~\ref{assum:lipschitz},~\ref{assum:strongly-convex} and~\ref{assum:compact}, if $\alpha > 0$, or the fraction of Byzantine faulty agents $f/n$ is less than $1/\left(1 + 2(\mu/\gamma) \right)$, then the DGD method with the CGE gradient-filter is asymptotically {\em $(f, \, \D \epsilon)$-resilient} (by Definition~\ref{def:approx_res}) where 
\begin{align}
    \D  = \frac{4 \mu f}{\alpha \gamma} = \frac{4 \mu \, n}{  (n/f) \, \gamma -  ( \gamma  + 2 \mu) }. \label{eqn:D_cge}
\end{align}
Fewer number of Byzantine faulty agents $f$ implies a smaller value of $\D$, and therefore, better fault-tolerance of the algorithm. Moreover, $\D = 0$ when $f = 0$, i.e., the algorithm indeed converges to the actual minimum point of all the agents' aggregate cost function in the fault-free case. Note that under Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex}, $\gamma \leq \mu$ (see Appendix~\ref{app:gamma_mu}). So, the fault-tolerance guarantee of the CGE gradient-filter, presented in Theorem~\ref{thm:conv-guarantee}, requires $f/n < 1/3$, or $f < n/3$. \\


% However, {\bf the reader can skip to Section~\ref{sec:experiments} without any loss of continuity.}\\

% where 
% \[\sigma = \D \, \epsilon = \dfrac{4\mu f}{ \alpha \,  \gamma} \, \epsilon = \frac{4\mu f}{\left( \gamma -\dfrac{f}{n}\left(\gamma +2\mu\right) \right)} \, \epsilon = \left(\frac{4 \mu  \, n \, f}{(n - f) \gamma + 2 \mu \, f}\right) \, \epsilon.\]

% \subsubsection{CWTM Gradient-Filter}
% \label{sub:cwtm}

Next, we show that when the separation between the gradients of the non-faulty agents' cost functions is sufficiently small then the CWTM gradient-filter can guarantee some approximate fault-tolerance under $(2f, \, \epsilon)$-redundancy. To present the fault-tolerance of the CWTM gradient-filter, we make the following additional assumption.

\begin{assumption}
\label{assum:corr_grad}
For two non-faulty agents $i$ and $j$, we assume that there exists $\lambda > 0$ such that for all $x \in \W$,
\[\norm{\nabla Q_i(x) - \nabla Q_j(x)} \leq \lambda \, \max \left\{ \norm{Q_i(x)}, \, \norm{Q_j(x)}\right\}.\]
\end{assumption}
Due to triangle triangle inequality, Assumption~\ref{assum:corr_grad} trivially holds true when $\lambda = 2$. However, we can presently guarantee fault-tolerance of CWTM gradient-filter when $\lambda < \gamma/(\mu \sqrt{d})$ where $\mu$ and $\gamma$ are the Lipschitz smoothness and strong convexity coefficients, respectively defined in Assumption~\ref{assum:lipschitz} and~\ref{assum:strongly-convex}. Recall the definition of point $x_{\H} \in \R^d$ from~\eqref{eqn:uniq_min} where $\H$ denotes an arbitrary set of $n-f$ non-faulty agents.

\begin{theorem}
\label{thm:conv-guarantee_cwtm}
    Suppose that the non-faulty agents' cost functions satisfy the $(2f, \, \epsilon)$-redundancy property, and the Assumptions~\ref{assum:lipschitz},~\ref{assum:strongly-convex},~\ref{assum:compact} and~\ref{assum:corr_grad} hold true. Consider the algorithm in Section~\ref{sub:steps} with the CWTM gradient-filter defined in~\eqref{eqn:cwtm_gf}. The following holds true:
    \begin{enumerate}
        \item $\norm{\gf \left(g^t_1, \ldots, \, g^t_n\right)} < \infty$ for all $t$.
        \item If $\lambda < \gamma/(\mu \sqrt{d})$ then for each set of $n-f$ non-faulty agents $\H$, for each $\delta > 0$,
    \begin{equation*}
        \phi_t=\iprod{x^t-x_{\H}}{\gf \left(g^t_1, \ldots, \, g^t_n\right)} \geq \left( 2 \sqrt{d} n \mu \lambda \, \epsilon +  \left(\gamma -  \sqrt{d} \lambda \mu \right) \, \delta \right) \, \delta 
    \end{equation*}
    when \(
        \norm{x^t - x_{\H}} \geq \cfrac{2 \sqrt{d} n \mu \lambda}{(\gamma - \sqrt{d} \mu \lambda)} \, \epsilon  + \delta.
    \)
    \end{enumerate}
    % , and diminishing step-sizes $\{\eta_0, \eta_1, \ldots \}$ in~\eqref{eqn:update} satisfying: $\sum_{t=1}^{\infty}\eta_t=\infty$ and $\sum_{t=1}^{\infty}\eta_t^2 < \infty$. 
    
\end{theorem}
~

% \begin{theorem}
% Suppose that the non-faulty agents' cost functions satisfy the $(2f, \, \epsilon)$-redundancy property, and Assumptions~\ref{assum:lipschitz},~\ref{assum:strongly-convex},~\ref{assum:compact} and~\ref{assum:corr_grad}. Consider the iterative algorithm in Section~\ref{sub:steps} with the CWTM gradient-filter defined in~\eqref{eqn:cwtm_gf}, and diminishing step-sizes $\{\eta_0, \eta_1, \ldots \}$ in~\eqref{eqn:update} satisfying: $\sum_{t=1}^{\infty}\eta_t=\infty$ and $\sum_{t=1}^{\infty}\eta_t^2 < \infty$. If $\lambda < \gamma/(\mu \sqrt{d})$ then for each set of $n-f$ non-faulty agents $\H$,
%     % \begin{equation}
%     %     \dfrac{f}{n}<\dfrac{1}{1+(4\mu/\gamma)},
%     %     \label{eqn:fault-fraction}
%     % \end{equation}
%     \begin{equation*}
%         \lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \leq \left( \frac{2 n \lambda}{(\gamma/\mu \sqrt{d}) -\lambda} \right)  \, \epsilon.
%         % \left(\frac{4 \mu \, f}{n - f \left( \gamma + 4 \mu \right)}\right) \, \epsilon.
%     \end{equation*}
% \end{theorem}
By similar arguments as in the case of CGE, Theorem~\ref{thm:conv-guarantee_cwtm}, in conjunction with Theorem~\ref{thm:upper-bound-D}, implies that the DGD method with CWTM gradient-filter and diminishing step-sizes is asymptotically {\em $(f, ~ \D' \, \epsilon )$-resilient} where
\[\D' = \frac{2 \sqrt{d} n \mu \lambda}{(\gamma - \sqrt{d} \mu \lambda)} = \left( \frac{2 n }{(\gamma/ \mu \lambda \sqrt{d}) - 1} \right),\]
under the conditions sated in Theorem~\ref{thm:conv-guarantee_cwtm}.
Smaller is the value of $\lambda$, i.e., closer are non-faulty gradients to each other, the smaller is the value of $\D'$, and therefore, better is the approximate fault-tolerance guarantee of the CWTM gradient-filter. Unlike the CGE gradient-filter, resilience of CWTM presented in Theorem~\ref{thm:conv-guarantee_cwtm} is independent of $f$, as long as $\lambda < \gamma/(\mu \sqrt{d})$. However, the condition on $\lambda$ to guarantee the resilience of CWTM gradient-filter depends upon the dimension $d$ of the optimization problem. Larger dimension result in a tighter bound on $\lambda$. 

% The above inequality is similar to~\eqref{eqn:phi-t-final} in the proof of Theorem~\ref{thm:conv-guarantee} in Appendix~\ref{app:proof_1} where by assumption $\gamma -  \sqrt{d} \lambda \mu > 0$. Also, recall from~\eqref{eqn:cwtm_bnd_grd} that in this particular case of CWTM gradient-filter $\norm{\gf\left(g^t_1, \ldots, \, g^t_n \right)} < \infty, ~ \forall t$. Therefore, using similar arguments as in Appendix~\ref{app:proof_1}, we obtain that 
% % the estimates of our algorithm can be bounded as follows:
% \begin{equation*}
%     \lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \leq \frac{2 \sqrt{d} n \mu \lambda}{(\gamma - \sqrt{d} \mu \lambda)} \, \epsilon  =  \left( \frac{2 n \lambda}{(\gamma/\mu \sqrt{d}) -\lambda} \right) \, \epsilon.
% \end{equation*}
% ~





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse

Finally, we present below the actual convergence rate of our algorithm when the step-size $\eta_t = 1/(t+1)$ for all $t$. This particular step-size indeed satisfies the condition prescribed in Theorem~\ref{thm:conv-guarantee}, see~\cite{rudin1964principles}. As $\W$ is a compact set,
\[\Gamma = \max_{x\in\mathcal{W}}\norm{x-x^*} < \infty.\] 
% We define
% \begin{equation}
%     \L = \dfrac{4\mu^2}{\alpha \, \gamma^2}(\Gamma + 2n\epsilon)^2. \label{eqn:rate_l}
% \end{equation}
% \begin{itemize}
%     \item We define a \textit{fault-tolerance margin}
%     \begin{equation}
%         \alpha = 1-\dfrac{f}{n}\left(1+\dfrac{4\mu}{\gamma}\right).
%     \end{equation}
%     Note that $\alpha > 0$ if and only if~\eqref{eqn:fault-fraction} holds true.
    
%     \item As $\W$ is a hypercube with finite dimensions, $\Gamma = \max_{x\in\mathcal{W}}\norm{x-x^*} < \infty$. We define
%     \begin{equation}
%         \L = \dfrac{4\mu^2}{\alpha \, \gamma^2}\Gamma^2. \label{eqn:rate_l}
%     \end{equation}
%     \item Lastly, we define 
%     \begin{equation*}
%         \D = \dfrac{4\mu f}{ \alpha \,  n \gamma}.
%         % \D = \dfrac{4\mu\epsilon f}{n\gamma\left(1-\dfrac{f}{n}\left(1+\dfrac{4\mu}{\gamma}\right)\right)},
%     \end{equation*}
% \end{itemize}
% ~

\begin{theorem}
    Suppose that the non-faulty agents' cost functions satisfy the $(2f, \, \epsilon)$-redundancy property, and Assumptions~\ref{assum:lipschitz},~\ref{assum:strongly-convex} and~\ref{assum:compact}. Consider the algorithm described in Section~\ref{sub:steps} with CGE gradient-filter. If $\alpha > 0$, and the step size
    \begin{equation}
        \eta_t=\left(\dfrac{2}{\alpha \, n \gamma}\right)\dfrac{1}{t+1}, \quad \forall t\geq0,
        \label{eqn:eta-t}
    \end{equation}
    then for each set of non-faulty agents $\H$ with $\mnorm{\H} = n-f$,
    \begin{equation}
        \norm{x^t-x_{\H}}^2\leq \left(\dfrac{1}{t+1} \right) \left(\frac{2 \mu (\Gamma + 2n\epsilon)}{\alpha \, \gamma} \right)^2  + \D^2 \, \epsilon^2, \quad \forall t\geq0.
    \end{equation}
    % where recall, from~\eqref{eqn:uniq_min}, that $x^*$ is the minimum point of the aggregate cost function of all the non-faulty agents.
    \label{thm:conv-rate}
\end{theorem}

The proof of Theorem~\ref{thm:conv-rate} is deferred to Section~\ref{sub:proof_2}.\\

% The condition $\alpha > 0$ in Theorem~\ref{thm:conv-rate} is equivalent to the condition~\eqref{eqn:fault-fraction} in Theorem~\ref{thm:conv-guarantee}. 
According to Theorem~\ref{thm:conv-rate}, when the value of the maximum fraction of Byzantine faulty agents $f/n$ decreases, $\alpha$ increases. Consequently, the convergence rate of the algorithm improves. Similarly, when the fraction of faulty agents increases, the convergence rate of the algorithm degrades. 
% Also, the radius of the specified neighborhood increases, meaning the output of the algorithm might become more inaccurate.

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> alt_approx.tex <==
\section{Approximate Fault-Tolerance}
\label{sec:approx-fault-tolerance}

As mentioned above, an approximately fault-tolerant distributed optimization algorithm outputs a {\em sub-optimal point} that may only approximately minimize the non-faulty aggregate cost function. Now, as discussed below in Section~\ref{sub:alt_approx}, there are several ways of defining sub-optimality. However, as our goal is to find an approximate minimum point, we define approximate fault-tolerance in terms of the Euclidean distance between the output of a prescribed algorithm and a true minimum point of the non-faulty aggregate cost. Specifically, we formally refer to approximate fault-tolerance as {\em $(f, \, \epsilon)$-resilience} where $\epsilon$ is a positive real value. Notations $\norm{\cdot}$ and $\mnorm{\cdot}$ denote the Euclidean norm and set cardinality, respectively.

% Without loss of generality we assume that each agent $i$ has ``true'' cost function. If an agent $i$ is non-faulty then it sends information to the server corresponding to its true cost function. Otherwise, if an agent $i$ is faulty then it may send arbitrary inforamtion to the server. To be precise, the behavior of the two types of agents can be described as follows.

% \begin{itemize}
%     \item If an agent $i$ is non-faulty, its behavior is consistent with its true cost function, say $Q_i(x)$. For instance, if agent $i$ is required to send to the server the value of its cost function at some point $x^\dagger$, a non-faulty agent $i$ will send $Q_i(x^\dagger)$.
%     \item If an agent $i$ is faulty, its behavior can be arbitrary, and not necessarily consistent with its true cost function, say $Q_i(x)$. For instance, if agent $i$ is required to send to the server the value of its cost function at some point $x^\dagger$, a faulty agent $i$ may send an arbitrary value instead of $Q_i(x^\dagger)$. 
% \end{itemize}
% If an agent is faulty, it may not share with the server any information about its true cost function. Still, it is convenient to define a true cost function, which is the cost function it would use in absence of its failure.

%  present below the definition of 

\begin{definition}[\textbf{$(f, \, \epsilon)$-resilience}]
\label{def:approx_res}
A distributed optimization algorithm $\Pi$ is said to be {\em $(f,\epsilon)$-resilient} if it outputs a point within $\epsilon$ distance from a true minimum of the non-faulty aggregate cost function. Specifically, if $\H$ denotes the set of non-faulty agents then $\Pi$ outputs a point $\widehat{x} \in \R^d$ for which there exists a minimum point $x^*\in\arg\min_x\sum_{i \in \H} Q_i(x)$ such that $\norm{\widehat{x} - x^*}\leq\epsilon$.
% \begin{align*}
%     \norm{\widehat{x} - x^*}\leq\epsilon.
% \end{align*}
\end{definition}

Before we present the necessary and sufficient conditions for achieving {$(f, \, \epsilon)$-resilience} we present below a comparison between $(f, \, \epsilon)$-resilience and other notions of approximate fault-tolerance from prior works~\cite{diakonikolas2018sever, su2016fault}.

\subsection{Other notions of approximate fault-tolerance}
\label{sub:alt_approx}
% We first discuss a couple of approximation definitions inspired from existing works, and then present our proposed definition which not only generalizes the other existing definitions but is most suitable for.\\

As proposed by Su and Vaidya, 2016~\cite{su2016fault}, an alternate way of measuring approximation (or accuracy) in fault-tolerance is by use of scalar coefficients. To be precise, instead of a minimum point of the {\em uniformly weighted} aggregate of non-faulty agents' cost functions, a distributed optimization algorithm may output a minimum point of a {\em non-uniformly weighted} aggregate of non-faulty costs, i.e., $\sum_{i \in \H} \alpha_i \, Q_i(x)$,
where $\H$ denotes the set of non-faulty agents, and $\alpha_i \geq 0$ for all $i \in \H$. As is suggested in~\cite{su2016fault}, upon re-scaling the coefficients such that $\sum_{i \in \H} \alpha_i = 1$, we can measure approximation in fault-tolerance using two metrics; 1) the number of coefficients in $\{\alpha_i, \, i \in \H\}$ that are positive, and 2) the minimum positive value amongst the coefficients: $\min \left\{ \alpha_i; \, \alpha_i > 0, \, i \in \H \right\}$.  \\

An alternate way of measuring approximation is by the value of the non-faulty aggregate cost function, or its gradient, at the output. For instance, as discussed in~\cite{diakonikolas2018sever}, for
differential cost functions, a resilient distributed optimization algorithm may aim to output a point $x_\Pi \in \R^d$, such that each element of the aggregate non-faulty gradient $\sum_{i \in \H} \nabla Q_i(x_\Pi)$ has an absolute value upper bounded by $\epsilon$. As yet another alternative, a resilient algorithm $\Pi$ may aim to output a point $x_\Pi$
such that the non-faulty aggregate cost $\sum_{i \in \H} Q_i(x_\Pi)$ is within $\epsilon$ of the true minimum cost $\min_x \sum_{i \in \H} Q_i(x)$. However, these definitions of approximate resilience are sensitive to scaling of the cost functions. In particular, if the elements of $\sum_{i \in \H} \nabla Q_i(x_\Pi)$ are bounded by $\epsilon$ then the elements of $\sum_{i \in \H} \alpha \nabla Q_i(x_\Pi)$ are bounded by $\alpha \epsilon$, where $\alpha$ is a positive scalar value. On the other hand, both $\sum_{i \in \H} Q_i(x)$ and $\sum_{i \in \H} \alpha Q_i(x_\Pi)$ have identical minimum point regardless of the value of $\alpha$. Therefore, if our objective is to approximate a true minimum point $x^*$ then using function or gradient values to define approximation may not be the most appropriate choice in general.\\

% An alternate way of measuring approximation is by the value of the non-faulty aggregate cost function, or its gradient's elements, at the output. For instance, as discussed in~\cite{diakonikolas2018sever}, assuming that the cost functions are differentiable, a distributed optimization algorithm $\Pi$, that outputs a point $x_\Pi \in \R^d$, may be referred to as $(f, \, \epsilon)$-resilient if each element of the aggregate non-faulty gradient $\sum_{i \in \H} \nabla Q_i(x_\Pi)$ has an absolute value less than or equal to $\epsilon$. As yet another alternative, algorithm $\Pi$ may be referred to as $(f, \, \epsilon)$-resilient if the non-faulty aggregate cost $\sum_{i \in \H} Q_i(x_\Pi)$ is more than the minimum cost $\sum_{i \in \H} Q_i(x^*)$ by at most $\epsilon$. However, these definitions of approximate resilience are sensitive to scaling of the cost functions, i.e., if the elements of $\sum_{i \in \H} \nabla Q_i(x_\Pi)$ are bounded by $\epsilon$ then the elements of $\sum_{i \in \H} \alpha \nabla Q_i(x_\Pi)$ are bounded by $\alpha \epsilon$ where $\alpha$ is a positive scalar value. On the other hand, both $\sum_{i \in \H} Q_i(x)$ and $\sum_{i \in \H} \alpha Q_i(x_\Pi)$ have identical minimum point regardless of the value of $\alpha$. Therefore, if our objective is to approximate a true minimum point $x^*$ then using function or gradient values to define approximation may not be the most appropriate choice.\\

In this paper, we consider $(f, \, \epsilon)$-resilience as per Definition~\ref{def:approx_res}.
We next present the necessary and sufficient conditions for achieving $(f, \, \epsilon)$-resilience.




==> alt_approx_v2.tex <==
\section{Necessary and Sufficient Conditions for $(f, \, \epsilon)$-Resilience}
\label{sec:approx-fault-tolerance}
% In this section, we present necessary and sufficient conditions for $(f, \, \epsilon)$-resilience.
Throughout this paper we assume, as stated below, that the non-faulty agents' cost functions and their aggregates have well-defined minimum points. Otherwise, the problem of optimization is rendered vacuous. 
% Specifically, we assume the following by default.
\begin{assumption}
\label{asp:exists}
For every non-empty set of non-faulty agents $S$, we assume that the set $\arg \min_{x \in \R^d} \sum_{i \in S}Q_i(x)$ is non-empty and closed.
\end{assumption}








==> cwtm_proof.tex <==
\section{Appendix: Proof of Theorem~\ref{thm:conv-guarantee_cwtm}}
\label{app:proof_2}

In this section we present the proof of Theorem~\ref{thm:conv-guarantee_cwtm}.
Throughout this section we assume $f > 0$ to ignore the trivial case of $f = 0$. The proof closely follows that of Theorem~\ref{thm:conv-guarantee}, and we may borrow some notation and results directly from Appendix~\ref{app:proof_1}.\\

% Consider an arbitrary set $\H$ of non-faulty agents with $\mnorm{\H} = n-f$. Recall that under Assumption~\ref{assum:strongly-convex} the minimum point of the aggregate cost function $\sum_{i \in \H} Q_i(x)$, denoted by $x_{\H}$, is unique. Specifically, 
% \[x_{\H} = \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x).\]
% To prove the theorem we make use of the result stated in Theorem~\ref{thm:upper-bound-D}. Specifically, we show that the CWTM gradient-filter satisfies the conditions of Theorem~\ref{thm:upper-bound-D} for $\D^* = 4 \lambda \mu f \, \epsilon$, and $x^* = x_{\H}$. The rest follows easily from the convergence result stated in Theorem~\ref{thm:upper-bound-D}. 
Recall from~\eqref{eqn:cwtm_gf} that for CWTM gradient-filter, for all $l \in \{1, \ldots, \, d\}$,
\begin{align}
    \gf\left(g^t_1, \ldots, \, g^t_n \right)[l] = \frac{1}{n-2f} \, \sum_{j=f+1}^{n-f}g_{i_j[l]}^t [l], \quad \forall t. \label{eqn:gf_cwtm_proof}
\end{align}
~

First, we show that $\sum_{j=f+1}^{n-f}g_{i_j[l]}^t [l]$ is finite for all $l$ and $t$. From~\eqref{eqn:honest-bound-everywhere} in Appendix~\ref{app:proof_1}, we know that if the $(2f, \, \epsilon)$-redundancy property and Assumption~\ref{assum:lipschitz} hold true then for each non-faulty agent $i\in\H$, 
\begin{equation}
    \norm{\nabla Q_i(x)} \leq 2n\mu\epsilon+\mu\norm{x-x_{\H}}. \label{eqn:pf_2_lip}
\end{equation}
The above implies that for all $i \in \H$, $l \in \{1, \ldots, \, d\}$ and $x$,
\begin{equation}
    \mnorm{\nabla Q_i(x)[l]} \leq 2n\mu\epsilon+\mu\norm{x-x_{\H}}.
    \label{eqn:honest-bound-everywhere_l}
\end{equation}
% The last inequality in~\eqref{eqn:honest-bound-everywhere} follows from the fact that $f > 0$.\\
Recall that for all $l$ and $t$, 
\begin{equation*}
    g_{i_1[l]}^t[l] \leq \ldots \leq g_{i_{f + 1}[l]}^t[l] \leq \ldots \leq g_{i_{n-f}[l]}^t[l] \leq  \ldots \leq g_{i_n[l]}^t[l].
\end{equation*}
%With \eqref{eqn:update}, the construction of $\widehat{g_j^t}$, we have
%\begin{equation}
%    \norm{\widehat{g_j^t}}\leq\norm{g_{i_{n-f}}^t}, ~\forall j\in[n],~t\in\mathbb{Z}_{\geq0}.
%    \label{eqn:norm-upperbound}
%\end{equation}
As there are at most $f$ Byzantine agents and $\mnorm{\H} = n-f$, for all $l$ and $t$ there exists a pair of non-faulty agents $\sigma^1_t[l], \,  \sigma^2_t[l] \in \H$ such that
\begin{equation}
    g_{i_{n-f}[l]}^t[l] \leq g_{i_{\sigma^1_t[l]}}^t[l], \text{ and } g_{i_{f+1}[l]}^t[l] \geq g_{i_{\sigma^2_t[l]}}^t[l].
    \label{eqn:honest-bound_l}
\end{equation}
As $g_j^t=\nabla Q_j(x^t)$ for all $j\in\H$, from~\eqref{eqn:honest-bound_l} we obtain that for all $j \in \{f+1, \ldots, n-f\}$, $l$ and $t$,
\begin{equation*}
    \mnorm{g_{i_j[l]}^t[l]} \leq \max \left\{ \mnorm{\nabla Q_{\sigma^1_t[l]}(x^t)[l]}, \, \mnorm{\nabla Q_{\sigma^1_t[l]}(x^t)[l]} \right\}.
\end{equation*}
Substituting from~\eqref{eqn:honest-bound-everywhere_l} above we obtain that for all $j \in \{f+1, \ldots, n-f\}$, $l$ and $t$,
\begin{equation*}
    \mnorm{g_{i_j[l]}^t[l]} \leq  2n\mu\epsilon+\mu\norm{x^t-x_{\H}}.
\end{equation*}
Therefore, owing to the triangle inequality,
\begin{equation}
    \mnorm{\sum_{j=f+1}^{n-f}g_{i_j[l]}^t [l]} \leq \sum_{j=f+1}^{n-2f}\mnorm{g_{i_j[l]}^t [l]} \leq (n-f)\left(2n\mu\epsilon+\mu\norm{x^t-x_{\H}}\right). \label{eqn:filtered-upperbound_l}
\end{equation}
Let $\Gamma = \max_{x \in \W} \norm{x - x_{\H}}$. As $\W$ is a compact set, $\Gamma < \infty$. Recall from the update rule~\eqref{eqn:update} that $x^t \in \W$ for all $t$. Thus, $\norm{x^t - x_{\H}} \leq \max_{x \in \W} \norm{x - x_{\H}} = \Gamma < \infty$. Substituting this in~\eqref{eqn:filtered-upperbound_l} implies that for all $l \in \{1, \ldots, \, d\}$,
\begin{equation*}
    \mnorm{\sum_{j=f+1}^{n-f}g_{i_j[l]}^t [l]} \leq (n-2f) \left( 2n \mu \epsilon + \mu \Gamma\right) < \infty. 
\end{equation*}
Substituting from above in~\eqref{eqn:gf_cwtm_proof} we obtain that 
\begin{align}
    \norm{\gf \left(g^t_1, \ldots, \, g^t_n \right)} < \infty, \quad \forall t. \label{eqn:cwtm_bnd_grd}
\end{align}
~

% Recall from the update rule~\eqref{eqn:update} that, for all $t \geq 0$,
% \begin{align*}
%     \norm{x^{t+1}-x^*}^2 &= \norm{\left[x^t - \eta_t\sum_{j=1}^{n-f}g_{i_j}^t\right]_{\W} - x^*}^2.
% \end{align*}
% Due to the well-known non-expansion property of projection onto a convex set (see~\cite{boyd2004convex}) we obtain that
% \begin{align*}
%     \norm{x^{t+1}-x^*}^2 &\leq \norm{x^t - \eta_t\sum_{j=1}^{n-f}g_{i_j}^t - x^*}^2 \\
%     &=\norm{x^t-x^*}^2 - 2\eta_t\iprod{x^t-x^*}{\sum_{j=1}^{n-f}g_{i_j}^t}+\eta_t^2\norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2.
% \end{align*}
% Next, we show that 
% \begin{align}
%     \phi_t\triangleq\iprod{x^t-x_{\H}}{\gf\left(g^t_1, \ldots, \, g^t_n \right)} > 0 ~ \text{ when } ~ \norm{x^t-x_{\H}} > 4 \lambda \mu f \, \epsilon. \label{eqn:pf_2_phi_t}
% \end{align}
% Therefore, 
% \begin{equation}
%     \norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2\leq(n-f)^2\left(2n\mu\epsilon+\mu\norm{x^t-x^*}\right)^2. 
%     \label{eqn:square-filtered-gradients}
% \end{equation}
Now, consider an arbitrary iteration $t$ and $l \in \{1, \ldots, \, d\}$. From prior works on CWTM gradient-filter for the scalar case~\cite{su2016fault}, i.e., when $d = 1$, we know that trimmed mean of the $l$-th elements of the gradients lies in the convex hull of $l$-th elements of the non-faulty agents' gradients in set $\H$. Specifically,
\begin{align}
    \min_{i \in \H}g^t_{i}[l] \leq \gf\left(g^t_1, \ldots, \, g^t_n \right)[l] \leq \max_{i \in \H} g^t_{i}[l]. \label{eqn:cwtm_bnd_1}
\end{align}
Obviously,
\begin{align}
    \min_{i \in \H}g^t_{i}[l] \leq  \frac{1}{\mnorm{\H}} \sum_{i \in \H} g^t_{i}[l] \leq \max_{i \in \H} g^t_{i}[l]. \label{eqn:cwtm_bnd_2}
\end{align}
Therefore, from~\eqref{eqn:cwtm_bnd_1} and~\eqref{eqn:cwtm_bnd_2} we obtain that
\begin{align*}
    \mnorm{\gf\left(g^t_1, \ldots, \, g^t_n \right)[l] - \frac{1}{\mnorm{\H}} \sum_{i \in \H} g^t_{i}[l]} \leq \max_{i \in \H} g^t_{i}[l] - \min_{i \in \H} g^t_i[l]. 
\end{align*}
As $\max_{i \in \H} g^t_{i}[l] - \min_{i \in \H} g^t_i[l] = \max_{i, \, j \in \H} \mnorm{g^t_{i}[l] - g^t_{j}[l]}$, and $g^t_i = \nabla Q_i(x^t)$ for all $i \in \H$, the above can be re-written as follows.
\begin{align}
    \mnorm{\gf\left(g^t_1, \ldots, \, g^t_n \right)[l] - \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)[l]} \leq \max_{i, \, j \in \H} \mnorm{\nabla Q_i(x^t)[l] - \nabla Q_j(x^t)[l]}.  \label{eqn:cwtm-avg}
\end{align}
Note that for any two $i, \, j \in \H$,
\begin{align}
    \mnorm{\nabla Q_i(x^t)[l] - \nabla Q_j(x^t)[l]} \leq \norm{\nabla Q_i(x^t) - \nabla Q_j(x^t)}. \label{eqn:sep_bnd_1}
\end{align}
Substituting from Assumption~\ref{assum:corr_grad}, $\norm{\nabla Q_i(x) - \nabla Q_j(x)} \leq \lambda \max \left\{\norm{\nabla Q_i(x)}, \norm{\nabla Q_j(x)} \right\}$, in~\eqref{eqn:sep_bnd_1} we obtain that
\begin{align}
    \mnorm{\nabla Q_i(x^t)[l] - \nabla Q_j(x^t)[l]} \leq \lambda \max \left\{\norm{\nabla Q_i(x^t)}, \, \norm{\nabla Q_j(x^t)} \right\}. \label{eqn:sep_bnd_2}
\end{align}
Substituting from~\eqref{eqn:pf_2_lip} above we obtain that
\begin{align}
    \mnorm{\nabla Q_i(x^t)[l] - \nabla Q_j(x^t)[l]} \leq \lambda \left( 2n\mu \, \epsilon+\mu\norm{x^t-x_{\H}} \right). \label{eqn:sep_bnd_3}
\end{align}
Finally, substituting from~\eqref{eqn:sep_bnd_3} in~\eqref{eqn:cwtm-avg} we obtain that, for all $l$,
\begin{align*}
    \mnorm{\gf\left(g^t_1, \ldots, \, g^t_n \right)[l] - \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)[l]} \leq \lambda \left( 2n\mu \, \epsilon+\mu\norm{x^t-x_{\H}} \right). 
\end{align*}
As $\norm{x} = \sqrt{\sum_{l = 1}^d \mnorm{x[l]}^2}$ for $x \in \R^d$, the above implies that
\begin{align}
    \norm{\gf\left(g^t_1, \ldots, \, g^t_n \right) - \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)} \leq \sqrt{d} \lambda \left( 2n\mu \, \epsilon+\mu\norm{x^t-x_{\H}} \right). \label{eqn:cwtm-avg-2}
\end{align}
Now, note that
\begin{align}
    \gf\left(g^t_1, \ldots, \, g^t_n \right) & = \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)  \label{eqn:cwtm-cwtm-avg}\\
    & + \left( \gf\left(g^t_1, \ldots, \, g^t_n \right) - \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t) \right).  \nonumber
\end{align}
Recall from Theorem~\ref{thm:upper-bound-D} that $\phi_t$, for each $t$, is defined to be
\begin{align*}
    \phi_t = \iprod{x^t-x_{\H}}{\gf\left(g^t_1, \ldots, \, g^t_n \right)}.
\end{align*}
Substituting from~\eqref{eqn:cwtm-cwtm-avg} above we obtain that
\begin{align}
    \phi_t & = \iprod{x^t - x_{\H}}{\frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)} \label{eqn:phi_t_cwtm_1}\\
    & +  \iprod{x^t - x_{\H}}{\gf\left(g^t_1, \ldots, \, g^t_n \right) - \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)} .  \nonumber
\end{align}
~

Recall from Assumption~\ref{assum:strongly-convex} that $Q_{\H}(x) = (1/\mnorm{\H})\sum_{i \in \H}Q_i(x)$. Thus, the first term on the right-hand side of~\eqref{eqn:phi_t_cwtm_1}, 
\begin{align*}
    \iprod{x^t - x_{\H}}{\frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)} = \iprod{x^t - x_{\H}}{\nabla Q_{\H}(x^t)}.
\end{align*}
Substituting from the Assumption~\ref{assum:strongly-convex} above, and recalling that $\nabla Q_{\H}(x_{\H}) = 0$, we obtain that
\begin{align}
    \iprod{x^t - x_{\H}}{\frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)}  \geq \gamma \, \norm{x^t - x_{\H}}^2. \label{eqn:first_phi_cwtm}
\end{align}
Next, we consider the second term on the right-hand side of~\eqref{eqn:phi_t_cwtm_1}. From Cauchy-Schwartz inequality,
\begin{align*}
    & \iprod{x^t - x_{\H}}{\gf\left(g^t_1, \ldots, \, g^t_n \right) - \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)}  \\
    & \geq - \norm{x^t - x_{\H}} \norm{\gf\left(g^t_1, \ldots, \, g^t_n \right) - \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)}.
\end{align*}
Substituting from~\eqref{eqn:cwtm-avg-2} above we obtain that
\begin{align}
    & \iprod{x^t - x_{\H}}{\gf\left(g^t_1, \ldots, \, g^t_n \right) - \frac{1}{\mnorm{\H}} \sum_{i \in \H} \nabla Q_i(x^t)} \nonumber \\
    & \geq - \sqrt{d} \lambda \, \norm{x^t - x_{\H}}  \left( 2n\mu \, \epsilon+\mu\norm{x^t-x_{\H}} \right). \label{eqn:second_phi_cwtm}
\end{align}
Substituting from~\eqref{eqn:first_phi_cwtm} and~\eqref{eqn:second_phi_cwtm} in~\eqref{eqn:phi_t_cwtm_1} we obtain that
\begin{align}
\begin{split}
    \phi_t & \geq \gamma \, \norm{x^t - x_{\H}}^2 - \sqrt{d} \lambda \, \norm{x^t - x_{\H}}  \left( 2n\mu \, \epsilon+\mu\norm{x^t-x_{\H}} \right) \label{eqn:phi_t_cwtm_2} \\
    & = \left(\gamma -  \sqrt{d} \lambda \mu \right) \norm{x^t - x_{\H}} \left( \norm{x^t - x_{\H}} - \frac{2 \sqrt{d} n \mu \lambda}{(\gamma - \sqrt{d} \mu \lambda)} \, \epsilon \right).
\end{split}
\end{align}
% Upon substituting
% \[\alpha = \gamma -  \sqrt{d} \lambda \mu , ~ \text{ and } ~ \D = \frac{2 \sqrt{d} n \mu \lambda}{(\gamma - \sqrt{d} \mu \lambda)}\]
% in~\eqref{eqn:phi_t_cwtm_2} we obtain that
% \begin{align}
%     \phi_t \geq \alpha \left(\norm{x^t - x_{\H}} - \D \epsilon \right). \label{eqn:cwtm_final_phi_1}
% \end{align}
% Upon 
Therefore, if, for an arbitrary $\delta > 0$, 
\begin{align*}
    \norm{x^t - x_{\H}} \geq \frac{2 \sqrt{d} n \mu \lambda}{(\gamma - \sqrt{d} \mu \lambda)} \, \epsilon  + \delta
\end{align*}
then
\begin{align*}
    \phi_t \geq \left(\gamma -  \sqrt{d} \lambda \mu \right) \left( \frac{2 \sqrt{d} n \mu \lambda}{(\gamma - \sqrt{d} \mu \lambda)} \, \epsilon  + \delta \right) \, \delta = \left( 2 \sqrt{d} n \mu \lambda \, \epsilon +  \left(\gamma -  \sqrt{d} \lambda \mu \right) \, \delta \right) \, \delta.
\end{align*}
Hence, the proof.

==> experiment.tex <==
\section{Numerical experiments}
\label{sec:experiments}

In this section, we present simulation results to empirically compare the approximate fault-tolerance achieved by the aforementioned gradient-filters; CGE and CWTM. For the simulation, we consider the problem of distributed linear regression, which is a special distributed optimization problem with quadratic cost functions~\cite{gupta2019byzantine}. 

\subsection{Problem description}
We consider a synchronous server-based system, as shown in Figure~\ref{fig:sys}, wherein $n=6$, $d=2$, and $f=1$. Each agent $i\in \{1, \, \ldots, \, n\}$ has a data point represented by a triplet $(A_i, \, B_i, \, N_i)$ where $A_i$ is a $d$-dimensional row vector, $B_i \in \R$ as the response, and a noise value $N_i \in \R$. Specifically, for all $i \in \{1, \, \ldots, \, n\}$, 
\begin{equation}
    B_i=A_ix^*+N_i ~ \text{ where } ~x^*=\begin{pmatrix}1\\1\end{pmatrix}.
\end{equation}
The collective data is represented by a triplet of matrices $(A, \, B, \, N)$ where the $i$-th row of $A$, $B$, and $N$ are equal to $A_i$, $B_i$ and $N_i$, respectively. The specific values are as follows.
\begin{equation}
    A=\begin{pmatrix}
        1 & 0 \\
        0.8 & 0.5 \\
        0.5 & 0.8 \\
        0 & 1 \\
        -0.5 & 0.8 \\
        -0.8 & 0.5 
    \end{pmatrix}, ~ 
    B=\begin{pmatrix}
        %0.91078179 \\  1.33487616 \\ 1.33758823 \\ 1.00334385 \\ 0.21424485 \\ -0.36153888
        0.9108 \\  1.3349 \\ 1.3376 \\ 1.0033 \\ 0.2142 \\ -0.3615
    \end{pmatrix}, ~ \text{ and }
    N=\begin{pmatrix}
        %-0.08921821 \\0.03487616\\0.03758823\\0.00334385\\-0.08575515\\-0.06153888
        -0.0892 \\0.0349 \\0.0376\\0.0033\\-0.0858\\-0.0615
    \end{pmatrix}.
\end{equation}
It should be noted that
\begin{align}
    B = A x^{*} + N. \label{eqn:set_equations}
\end{align}
We let $A_S$, $B_S$ and $N_S$ represent matrices of dimensions $\mnorm{S} \times 2$, $\mnorm{S} \times 1$ and $\mnorm{S} \times 1$ obtained by stacking the rows $\{A_i, \, i \in S \}$, $\{B_i, \, i \in S \}$ and $\{N_i, \, i \in S\}$, respectively, in the increasing order. From~\eqref{eqn:set_equations}, observe that for every non-empty set $S$,
\begin{align}
    B_S = A_S x^{*} + N_S. \label{eqn:set_equations-2}
\end{align}
Recall from basic linear algebra that if $A_S$ is full-column rank, i.e., $\rank{A_S} = d = 2$ then $x^*$ is the unique solution of the set of equations in~\eqref{eqn:set_equations-2}. Note that for every set $S$ with $\mnorm{S} \geq n-2f = 6 - 2 = 4$, the matrix $A_S$ is full rank. Specifically,
\begin{align}
    \rank{A_S} = d = 2, \quad \forall S \subseteq \{1, \ldots, \, 6\}, ~ \mnorm{S} \geq 4. \label{eqn:exp_full_rank}
\end{align}
~

In this particular distributed optimization problem, each agent $i$ has a quadratic cost function defined to be 
\[Q_i(x)=(B_i-A_ix)^2, \quad \forall x \in \R^2.\] 
For an arbitrary non-empty set of agents $S$, we define 
\[Q_S(x) = \sum_{i\in S}Q_i(x) = \sum_{i \in S}\left(B_i-A_ix \right)^2, \quad \forall x \in \R^2.\]
 Therefore,
\begin{align}
    Q_S(x) = \sum_{i \in S}\left(B_i-A_ix \right)^2 = \norm{B_S-A_Sx}^2. \label{def:exp_Q_S}
\end{align}
As matrix $A_S$ is full rank for every $S$ with $\mnorm{S} \geq 4$,
\begin{align}
    \arg \min_{x \in \R^2} Q_S(x) = \arg \min_{x \in \R^2} \norm{B_S-A_Sx}^2 = \left(x ~ \vline ~ A_S x = B_S \right). \label{eqn:solve_Q_S}
\end{align}
Therefore, $Q_S(x)$ has a unique minimum point when $\mnorm{S} \geq 4$. Henceforth, we write notation $\arg \min_{x \in \R^2}$ simply as $\arg \min$, unless otherwise stated.
% Substituting $B_S$ from~\eqref{eqn:set_equations-2} above, we obtain that, for every $S$ with $\mnorm{S} \geq 4$,
% \begin{align}
%     \arg \min_{x \in \R^2} Q_S(x) = \left(x ~ \vline ~ A_S (x - x^*) = N_S \right). \label{eqn:solve_Q_S}
% \end{align}
% ~
% $Q_S(x)=\sum_{i\in S}Q_i(x)=\norm{B_S-A_Sx}^2$, where the notation $A_S$, $B_S$ refer to the row submatrices of $A$ and $B$ containing only the rows in $S$. \\
% Note that the matrix $A$ has the following property: for any set of at least $n-2f$ rows $S\subseteq\{1,\,\dots,\,n\}$, the submatrix $A_S$ is full-column rank, \emph{i.e.}, $\rank{A}=\rank{A_S}=d=2$. Therefore, for any $S$, $\mnorm{S}\geq n-2f$, $B_S=A_Sx$ has a unique solution: there exists $\widetilde{x}_S$ such that $N_S=A_S\widetilde{x}_S$. Therefore, $B_S=A_S(x^*+\widetilde{x}_S)$, and 
% \begin{equation}
%     x^*_S\triangleq x^*+\widetilde{x}_S=\arg\min Q_S(x).
% \end{equation}
% ~

\subsection{Properties of agents' cost functions}
Due to the rank condition~\eqref{eqn:exp_full_rank}, the agents' cost functions satisfy the {\em $(2f, \, \epsilon)$-redundancy} property, stated in Definition~\ref{def:approx_red}, with $\epsilon = 0.0890$. The steps for computing $\epsilon$ are described below.
% We can mathematically examine the value of the redundancy parameter $\epsilon$, and the fulfillment of the Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex}.
% The value of $\epsilon$ is calculated by the following steps, according to Definition~\ref{def:approx_red}:
\begin{enumerate}
\setlength{\itemsep}{0.3em}
    \item For each set $S \subset\{1, \ldots, \, 6\}$ with $\mnorm{S} = n-f = 5$, compute $x_S \in \R^2$ such that $B_S = A_S x_S$. Note that, due to~\eqref{eqn:solve_Q_S}, $x_S = \arg \min Q_S(x)$.
    
    \item For each set $S \subset\{1, \ldots, \, 6\}$ with $\mnorm{S} = n-f = 5$ do the following: 
    
    \begin{enumerate}
        \item For each set $\widehat{S} \subseteq S$ with $\mnorm{\widehat{S}} \geq n-2f = 4$, compute $x_{\widehat{S}}$ such that $B_{\widehat{S}} = A_{\widehat{S}} x_{\widehat{S}}$. Note that, due to~\eqref{eqn:solve_Q_S}, $x_{\widehat{S}} = \arg \min Q_{\widehat{S}}(x)$.
        
        \item Compute 
        \[\epsilon_S=\max\limits_{\widehat{S}\subseteq S,\,\mnorm{\widehat{S}}\geq 4} \norm{x_S - x_{\widehat{S}}}.\]
        In this particular case, both the sets of minimum points $\arg \min Q_S(x)$ and $\arg \min Q_{\widehat{S}}(x)$ are singleton with points $x_S$ and $x_{\widehat{S}}$, respectively. Therefore, 
        \[\norm{x_S - x_{\widehat{S}}} = \dist{\arg \min Q_S(x)}{ \arg \min Q_{\widehat{S}}(x)}.\]
    \end{enumerate}
    % $B_{\widehat{S}}=A_{\widehat{S}}x_{\widehat{S}}$ for each ${\widehat{S}}$ with $\mnorm{\widehat{S}}\geq n-2f=4$, $\widehat{S}\subseteq S$.
    
    % \item Calculate $\epsilon_S=\max\limits_{\widehat{S}\subseteq S,\,\mnorm{\widehat{S}}\geq n-2f}\left\{\dist{x_S}{x_{\widehat{S}}}\right\}$ for each $S$, and
    \item In the final step, we compute 
    \[\epsilon=\max\limits_{\mnorm{S}=n-f}\epsilon_S.\]
\end{enumerate}
~

For each agent $i$, its cost function $Q_i(x)$ has Lipschitz continuous gradients, i.e., satisfy Assumption~\ref{assum:lipschitz}, with Lipschitz coefficient
\begin{align}
    \mu = \max_{i\in\H}2\,\overline{v}_i \label{eqn:exp_lip}
\end{align}
where $\overline{v}_i$ denotes the largest eigenvalue of $A_i^TA_i$, and $\H$ is the set of non-faulty agents. Also, for %every set of agents $S$ with $\mnorm{S} = n-f = 5$, 
agents in the set $\H$, their average cost function $(1/\mnorm{\H}) Q_\H(x)$ is strongly convex, i.e., satisfy Assumption~\ref{assum:strongly-convex}, with the strong convexity coefficient
\begin{align}
    \gamma = \frac{2}{\mnorm{\H}}\underline{v}_\H \label{eqn:exp_str}
\end{align}
where $\underline{\H}_S$ is the smallest eigenvalue of $A_\H^TA_\H$. Derivations of~\eqref{eqn:exp_lip} and~\eqref{eqn:exp_str} can found in \cite[Section 10]{gupta2019byzantine}.

% Also, the agents' cost functions also satisfy both Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex}.
% Suppose $\H$ is the set of honest agents in the system, $\mnorm{\H}=n-f$. For Assumption~\ref{assum:lipschitz}, the value of $\mu$, the Lipschitz constant, can be obtained by 
% \begin{equation}
%     \mu=\max_{i\in\H}\overline{v}_i, 
% \end{equation}
% where $\overline{v}_i$ is the largest eigenvalue of $A_i^TA_i$. For Assumption~\ref{assum:strongly-convex}, the value of $\gamma$, the strong convexity parameter can be obtained by 
% \begin{equation}
%     \gamma=\frac{1}{\mnorm{\H}}\underline{v}_\H,
% \end{equation}
% where $\underline{v}_\H$ is the smallest eigenvalue of $A_\H^TA_\H$. The derivation can be found in \cite{gupta2019byzantine}.\\

% For $f=1$, the dataset satisfies $(2f,\epsilon)$-redundancy with $\epsilon=0.0890$. %0.08896977000047095
\subsection{Simulation}
In our experiments, we simulate the following fault behaviors for the faulty agent.
\begin{itemize}
\setlength{\itemsep}{0.3em}
    \item \textit{gradient-reverse}: the faulty agent \textit{reverses} its true gradient. Suppose the correct gradient of a faulty agent $i$ at step $t$ is $s_i^t$, the agent $i$ will send the incorrect gradient $g_i^t=-s_i^t$ to the server.
    \item \textit{random}: the faulty agent sends a randomly chosen vector in $\mathbb{R}^d$. In our experiments, the faulty agent in each step chooses i.i.d. Gaussian random vector with mean 0 and a isotropic covariance matrix with standard deviation of 200.
\end{itemize}
~

We simulate the distributed gradient-descent algorithm described in Section~\ref{sub:steps} by assuming agent $1$ to be Byzantine faulty. It should be noted that the identity of the faulty agent is not used in any way during the simulations. Here, the set of non-faulty agents is $\H = \{2, \ldots, \, 6\}$ and $\mnorm{\H} = n-f = 5$. Therefore, in this particular case $\H$ is the only set of $n-f$ non-faulty agents. From~\eqref{eqn:solve_Q_S}, we obtain that the minimum point of the aggregate cost function $\sum_{i \in \H}Q_i(x)$, denoted by $x_{\H}$, is equal to the solution of the following set of linear equations: 
$$B_\H=A_\H x_\H.$$
Specifically, $x_\H=\begin{pmatrix}1.0780\\ 0.9825\end{pmatrix}$. Also, note from our earlier deductions in~\eqref{eqn:exp_lip} and~\eqref{eqn:exp_str} that in this particular case, the non-faulty agents' cost functions satisfy Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex} with $\mu=2$ and $\gamma=0.712$, respectively.\\

{\bf Parameters:} We use the following parameters for implementing the algorithm. In the update rule~\eqref{eqn:update}, we use step size $\eta_t=1.5/(t+1)$ for iteration $t = 0, \, 1, \ldots$. Note that this particular step-size is diminishing and satisfies the conditions: $\sum_{t=0}^\infty\eta_t=\infty$ and $\sum_{t=0}^\infty\eta_t^2=3\pi^2/8<\infty$ (see~\cite{rudin1964principles}). We assume the convex compact $\W \subset \R^d$ to be a 2-dimensional hypercube $[-1000,1000]^2$. Note that $x_{\H} \in \W$, i.e., Assumption~\ref{assum:compact} holds true. In all the simulation results presented below, the initial estimate $x^0 = (-0.0085,-0.5643)$. \\

In every execution, we observe that the iterative estimates produced by the algorithm practically converge after $400$ iterations. Thus, to measure the approximate fault-tolerance achieved by the different gradient-filter, i.e., CGE and CWTM, we define the output of the algorithm to be $x_{\textrm{out}} = x^{500}$. The outputs for the two gradient-filters, under different faulty behaviors, are shown in Table~\ref{tab:results}. Note that $\dist{x_\H}{x_{\mathrm{out}}}=\norm{x_\H-x_{\mathrm{out}}}$. The results for the case when the faulty agent sends {\em random} faulty gradients are only shown for a randomly chosen execution. \\

{\bf Conclusion:} As shown in Table~\ref{tab:results}, in all executions, the distances between $x_\H$ the output of the algorithm $x_{\textrm{out}}$ in case of both CGE and CWTM gradient-filters are smaller than $\epsilon = 0.0890$. For the said executions, we plot in Figure~\ref{fig:fault-comparison} the values of the aggregate cost function $\sum_{i \in \H}Q_i(x^t)$ (referred as {\em loss}) and the approximation error $\norm{x^t - x_{\H}}$ (referred as {\em distance}) for iteration $t$ ranging from $0$ to $500$. We also show the plots of the fault-free distributed gradient-descent (DGD) method when all agents are free from faults, and the DGD method without any gradient-filter when agent $1$ is Byzantine faulty. The details for iteration $t$ ranging from 0 to 80 are also highlighted in Figure~\ref{fig:fault-comparison-detail}. \\
% The plots for CWTM gradient-filter are colored yellow, 
% The trends of losses and distances between the estimate $x^t$ and the true minimum $x_\H$ point is shown in Figure~\ref{fig:fault-comparison}, CWTM by the yellow plots, and CGE by the green plots. In the fault-free case, gradient descent (GD) solves the problem with negligible numerical error, as is shown by the blue plots, while if the faulty agent is present in the system, plain gradient descent cannot solve the problem at all, as is shown by the red plots.

\begin{table}[tb!]
    \centering
    \caption{\footnotesize{\it Algorithm's outputs with gradient-filters CGE and CWTM, and the approximation errors, corresponging to executions when the faulty agent $1$ exhibits two different types of Byzantine faults; \textit{gradient-reverse} and \textit{random}. Recall that $x_{\mathrm{out}} = x^{500}$ and $\dist{x_\H}{x_{\mathrm{out}}}=\norm{x_\H-x_{\mathrm{out}}}$.}}
    \begin{tabular}{c|cc|cc}
         & \multicolumn{2}{c}{{\bf gradient-reverse}} & \multicolumn{2}{c}{{\bf random}} \\
         & $x_{\mathrm{out}}$ & $\dist{x_\H}{x_{\mathrm{out}}}$ & $x_{\mathrm{out}}$ & $\dist{x_\H}{x_{\mathrm{out}}}$ \\
        \hline
        {\bf CGE} & $\begin{pmatrix}1.0541\\0.9826\end{pmatrix}$ & 0.0239& $\begin{pmatrix}1.0779\\0.9826\end{pmatrix}$ & $4.72\times10^{-5}$ \\
        {\bf CWTM} & $\begin{pmatrix}1.0645\\0.9924\end{pmatrix}$ & 0.0167 & $\begin{pmatrix}1.0775\\0.9840\end{pmatrix}$ & $1.51\times10^{-3}$ \\
    \end{tabular}
\label{tab:results}
\end{table}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{imgs/comparison-8.pdf}
    %\includegraphics[width=.8\linewidth]{imgs/comparison-8.2.pdf}
    \caption{\footnotesize{\it The losses, i.e., $\sum_{i \in \H}Q_i(x^t)$, and distances, i.e., $\norm{x^t - x_{\H}}$, versus the number of iterations in the algorithm. The final approximation errors, i.e., $\norm{x^{500} - x_{\H}}$, are annotated in the same colors of their corresponding plots. For the executions shown, agent $1$ is assumed to be Byzantine faulty. The different columns show the results when the faulty agent exhibits the different types of faults: \emph{(a)}~gradient-reverse, and \emph{(b)}~random. Apart from the plots with CGE (in {\em green}) and CWTM (in {\em yellow}) gradient-filters, we also plot the fault-free distributed gradient-descent (DGD) method when all agents are free from faults (in {\em blue}), and the DGD method without any gradient-filters when agent $1$ is Byzantine faulty (in {\em red}).
    % The performance of CGE and CWTM gradient-filters are shown in the figures, comparing with the fault-free case where there is no faulty agent (blue plot), and 1 faulty agent but solved by plain gradient descent with no filter applied (red plot). 
    %Also, the first group of four figures shows the whole training process while the second group magnifies the first 80 steps, note that it is not converged at the 80th step for any GD procedures shown in the figures.
    }}
    \label{fig:fault-comparison}
\end{figure}

\begin{figure}[tb!]
    \centering
    %\includegraphics[width=\linewidth]{imgs/comparison-8.pdf}
    \includegraphics[width=\linewidth]{imgs/comparison-8.2.pdf}
    \caption{\footnotesize{\it The losses, i.e., $\sum_{i \in \H}Q_i(x^t)$, and distances, i.e., $\norm{x^t - x_{\H}}$, versus the number of iterations in the algorithm, magnified for the initial 80 iterations in the training process. The meaning of plots are the same as in Figure~\ref{fig:fault-comparison}.
    %For the executions shown, agent $1$ is assumed to be Byzantine faulty. The different columns show the results when the faulty agent exhibits the different types of faults: \emph{(a)}~gradient-reverse, and \emph{(b)}~random. Apart from the plots with CGE (in {\em green}) and CWTM (in {\em yellow}) gradient-filters, we also plot the fault-free distributed gradient-descent (DGD) method when all agents are free from faults (in {\em blue}), and the DGD method without any gradient-filters when agent $1$ is Byzantine faulty (in {\em red}).
    % The performance of CGE and CWTM gradient-filters are shown in the figures, comparing with the fault-free case where there is no faulty agent (blue plot), and 1 faulty agent but solved by plain gradient descent with no filter applied (red plot). 
    %Also, the first group of four figures shows the whole training process while the second group magnifies the first 80 steps, note that it is not converged at the 80th step for any GD procedures shown in the figures.
    }}
    \label{fig:fault-comparison-detail}
\end{figure}


==> gradient_proof-podc.old.2.tex <==
\section{Appendix: Lemma~\ref{lemma:upbd-vector}} % on the upper bound of the norm of vectors knowing the upper bound of the norm of the sum of these vectors}
\label{app:lemma}

\begin{lemma}
    \label{lemma:upbd-vector}
    For $n$ vectors $a_1,...,a_n$ and a positive number $f\leq n/2$, if there exists some real number $r\geq0$, such that for any set $S\subset[n]$ with $\mnorm{S}=f$ we have
    \begin{align}
        \norm{\sum_{i\in S}a_i}\leq r,
        \label{eqn:lemma-condition}
    \end{align}
    then for all $i\in[n]$ we also have
    \begin{align}
        \norm{a_i}\leq 2r.
    \end{align}
\end{lemma}
Let us first introduce some notations. For two vectors $a,b$, denote by $[a]_b$ the vector projection of $a$ onto $b$. Also, denote by $\boldsymbol{e}_b$ the unit vector on the direction of $b$.
\begin{proof}
    The proof is by contradiction. Suppose for some $k$, $s\triangleq\norm{a_k}>2r$. By \eqref{eqn:lemma-condition}, for any set $S'\subset[n]$ with $\mnorm{S'}=f-1$, we have
    \begin{align}
        \norm{\sum_{i\in S'}a_i + a_{k}}\leq r.
    \end{align}
    Due to the additivity and the non-expansion property of vector projection, 
    \begin{align}
        \norm{\left[\sum_{i\in S'}a_i + a_{k}\right]_{a_{k}}}=\norm{\left[\sum_{i\in S'}a_i\right]_{a_{k}}+a_{k}} \leq \norm{\sum_{i\in S'}a_i+a_{k}}\leq r.
    \end{align}
    Let $t$ be a real value such that $\left[\sum_{i\in S'}a_i\right]_{a_{k}} = t\cdot \boldsymbol{e}_{a_k}$. It follows that 
    \begin{align}
        \norm{\left[\sum_{i\in S'}a_i\right]_{a_{k}}+a_{k}} = \norm{(t + s)\boldsymbol{e}_{a_k}} = \mnorm{t+s} \leq r.
    \end{align}
    Therefore, $t+s\leq r$. So $t\leq r-s<r-2r=-r$.

    On the other hand, for any $j\in[n]$, $j\neq k$, by \eqref{eqn:lemma-condition}, we also have
    \begin{align}
        \norm{\sum_{i\in S'}a_i + a_j}\leq r.
    \end{align}
    Similarly, due to the non-expansion property of vector projection,
    \begin{align}
        \norm{\left[\sum_{i\in S'}a_i + a_j\right]_{a_{k}}}\leq \norm{\sum_{i\in S'}a_i+a_j}\leq r.
    \end{align}
    Let $t'$ be a real value such that ${\left[a_j\right]_{a_{k}}} = t'\cdot \boldsymbol{e}_{a_k}$. It follows that 
    \begin{align}
        \norm{\left[\sum_{i\in S'}a_i + a_j\right]_{a_{k}}} = \norm{(t'+t)\boldsymbol{e}_{a_k}} = \norm{t'+t}\leq r.
    \end{align}
    Since $t<-r$, we have $t'>0$.

    Since $f\leq n/2$, there are at least $f$ different element that is in $[n]$ but not in $S'\cup\{k\}$. Let $f-1$ of them be a set $S''$. We have
    \begin{align}
        \norm{\sum_{i\in S''}a_i+a_{k}}&\geq \norm{\left[\sum_{i\in S''}a_i+a_{k}\right]_{a_{k}}}\geq \norm{\sum_{i\in S''}\left[a_i\right]_{a_{k}}+a_{k}} \nonumber \\
        &\geq\norm{(\mnorm{S}t'+2r)\cdot\boldsymbol{e}_{a_{k}}} = \mnorm{\mnorm{S}t' + 2r} = \mnorm{S}t'+2r>2r.
    \end{align}
    However, since $\mnorm{S''\cup\{k\}}=f$, by \eqref{eqn:lemma-condition}, 
    \begin{align}
        \norm{\sum_{i\in S''}a_i+a_{k}}<r.
    \end{align}
    Contradiction. Hence the proof.
\end{proof}

\section{Appendix: Lemma~\ref{lemma:bounding-gradients-at-xH} on the upper bound of the norm of gradients with $(2f,\epsilon)$-redundancy}

We assume $f > 0$ to ignore the trivial case of $f = 0$. We also assume $f\leq n/2$. 

Consider an arbitrary set $\H$ of non-faulty agents with $\mnorm{\H} = n-f$. Recall that under Assumptions~\ref{assum:strongly-convex} and~\ref{assum:compact}, the aggregate cost function $\sum_{i \in \H} Q_i(x)$ has a unique minimum point in set $\W$, which we denote by $x_{\H}$. Specifically, 
\begin{align}
    \left\{x_{\H} \right\} = \W \cap \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x). \label{eqn:x_H_W}
\end{align}

\begin{lemma}
    \label{lemma:bounding-gradients-at-xH}
    Suppose a group of $n$ cost functions $Q_i(x)$'s satisfies $(2f,\epsilon)$-redundancy, and Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex} hold. 
    % Suppose $x_{\H}\in\arg\min_x\sum_{i\in\H}Q_i(x)$ of any set $\H\subset[n]$ with $\mnorm{\H}=n-f$. 
    Then for any $j\in[n]$ and any set $\H\subset[n]$ with $\mnorm{\H}=n-f$, we have
    \begin{align}
        \norm{\nabla Q_j(x_\H)} \leq 2(n-2f)\mu\epsilon.
    \label{eqn:honest-norm-bound}
    \end{align}
\end{lemma}

\begin{proof}
    Consider any subset $S_1 \subset \H$ with $\mnorm{S_1} = n-2f$. From triangle inequality, $\forall x \in \R^d$,
\begin{align*}
    \norm{\sum_{j\in S_1}\nabla Q_j(x)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \sum_{j \in S_1}\norm{\nabla Q_j(x) - \nabla Q_j(x_{\H})}.
\end{align*}
Under Assumption~\ref{assum:lipschitz}, i.e., Lipschitz continuity of non-faulty gradients, for each non-faulty agent $j$, $\norm{\nabla Q_j(x) - \nabla Q_j(x_{\H})} \leq \mu \norm{x - x_{\H}}$. Substituting this above implies that 
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \, \norm{x-x_{\H}}.
    \label{eqn:lipschitz-distance}
\end{equation}
As $\mnorm{S_1} = n-2f$, the $(2f,\epsilon)$-redundancy property defined in Definition~\ref{def:approx_red} implies that for all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$,
\[\norm{x_1-x_{\H}} \leq \epsilon.\]
Substituting from above in~\eqref{eqn:lipschitz-distance} implies that, for all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$,
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x_1)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \, \norm{x_1-x_{\H}} \leq \mnorm{S_1} \mu \epsilon.
    \label{eqn:lipschitz-distance-2}
\end{equation}
For all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$, $\sum_{j\in S_1}\nabla Q_j(x_1) = 0$. Thus,~\eqref{eqn:lipschitz-distance-2} implies that
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \epsilon.
    \label{eqn:lipschitz-distance-S1}
\end{equation}
For all $x_{\H}\in\arg\min_x\sum_{j\in\H}Q_j(x)$, $\sum_{j\in\H}\nabla Q_j(x_{\H})=0$. Thus, with $\mnorm{S_1}=n-2f$, \eqref{eqn:lipschitz-distance-S1} implies that 
\begin{align}
    \norm{\sum_{j\in\H\backslash S_1}\nabla Q_j(x_{\H})} = \norm{\sum_{j\in\H}\nabla Q_j(x_{\H}) - \sum_{j\in S_1}\nabla Q_j(x_{\H})} = \norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq (n-2f)\mu\epsilon.
\end{align}
Note that $\mnorm{\H\backslash S_1}=f$. Since the choices of $\H$ and $S_1$ are arbitrary, the above implies that for any subset of agents $T\subset[n]$ with $\mnorm{T}=f$, we have
\begin{align}
    \norm{\sum_{j\in T}\nabla Q_j(x_{\H})} \leq (n-2f)\mu\epsilon.
\end{align}
Since we assumed that $f\leq n/2$, by Lemma~\ref{lemma:upbd-vector}, from above we have for all $j\in[n]$,
\begin{align*}
    \norm{\nabla Q_j(x_{\H})} \leq 2(n-2f)\mu\epsilon.
    % \label{eqn:honest-norm-bound}
\end{align*}
\end{proof}

\section{Appendix: Proof of Theorem~\ref{thm:conv-guarantee}}
\label{app:proof_1}

% In this section, we present the proof of Theorem~\ref{thm:conv-guarantee}.
Throughout, we assume $f > 0$ to ignore the trivial case of $f = 0$.\\
% % Throughout this section we denote the set of non-faulty agents by $\H$. Recall that $\mnorm{\H} \geq n-f$. Recall that $x^*$ denotes the true minimum point of the non-faulty agents' aggregate cost function $\sum_{i \in \H} Q_i(x)$. We 

% \subsection{Proof of Theorem~\ref{thm:conv-guarantee}}
% \label{sub:proof_1}
Consider an arbitrary set $\H$ of non-faulty agents with $\mnorm{\H} = n-f$. Recall that under Assumptions~\ref{assum:strongly-convex} and~\ref{assum:compact}, the aggregate cost function $\sum_{i \in \H} Q_i(x)$ has a unique minimum point in set $\W$, which we denote by $x_{\H}$. Specifically, 
\begin{align}
    \left\{x_{\H} \right\} = \W \cap \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x). \label{eqn:x_H_W}
\end{align}
% \[x_{\H} = \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x).\]
% To prove the theorem we make use of the result stated in Theorem~\ref{thm:upper-bound-D}. Specifically, we show is that the CGE gradient-filter satisfies the conditions of Theorem~\ref{thm:upper-bound-D} for $\D^* = \D \, \epsilon$, and $x^* = x_{\H}$. The rest follows easily from the convergence result stated in Theorem~\ref{thm:upper-bound-D}. 
Recall from~\eqref{eqn:cge_gf} that for CGE gradient-filter, in update rule~\eqref{eqn:update},
\begin{align}
    \gf\left(g^t_1, \ldots, \, g^t_n \right) = \sum_{j=1}^{n-f}g_{i_j}^t, \quad \forall t. \label{eqn:cge_grad_filter_proof}
\end{align}
~

First, we show that $\norm{\sum_{j=1}^{n-f}g_{i_j}^t} < \infty, ~ \forall t$. 
% Now, consider an arbitrary non-faulty agent $i \in \H\setminus S_1$. Let $S_2=S_1\cup\{i\}$. 
% % Also suppose $i\in\H\backslash S_1$, and $S_2=S_1\cup\{i\}$. By Assumption \ref{assum:lipschitz}, there exists some $\mu$, such that %$(2f,\epsilon)$-redundancy, 
% % For any $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$, by $(2f,\epsilon)$-redundancy, $\norm{x_1-x^*}\leq\epsilon$. Combining with \eqref{eqn:lipschitz-distance}
% % \begin{equation}
% %     \norm{\sum_{j\in S_1}\nabla Q_j(x^*)}=\norm{\sum_{j\in S_1}\nabla Q_j(x_1)-\sum_{j\in S_1}\nabla Q_j(x^*)}\leq\mu\epsilon.
% % \end{equation}
% Using similar arguments as above we obtain that under the $(2f, \, \epsilon)$-redundancy property and Assumption~\ref{assum:lipschitz}, for all $x_2\in\arg\min_x\sum_{j\in S_2}Q_j(x)$,
% \begin{align}
%     \norm{\sum_{j\in S_2}\nabla Q_j(x_{\H})}=\norm{\sum_{j\in S_2}\nabla Q_j(x_2)-\sum_{j\in S_2}\nabla Q_j(x_{\H})}\leq\mnorm{S_2}\mu\epsilon.
% \end{align}
% Note that $\sum_{j\in S_2}\nabla Q_j(x)=\sum_{j\in S_1}\nabla Q_j(x)+\nabla Q_i(x)$. From triangle inequality,
% \begin{equation}
%     \norm{\nabla Q_i(x_{\H})}-\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})}\leq\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})+\nabla Q_i(x_{\H})}.
% \end{equation}
% Therefore, for each non-faulty agent $i\in\H$, 
% \begin{align}
%     \norm{\nabla Q_i(x_{\H})}&\leq\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})+\nabla Q_i(x_{\H})}+\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq\mnorm{S_2}\mu\epsilon+\mnorm{S_1}\mu\epsilon \nonumber\\
%     & = (n-2f+1)\mu \epsilon + (n-2f) \mu \epsilon = (2n-4f+1)\mu\epsilon.
%     \label{eqn:honest-norm-bound}
% \end{align}
For all $x$ and $i\in\H$, by Assumption \ref{assum:lipschitz},
\begin{equation*}
    \norm{\nabla Q_i(x)-\nabla Q_i(x_{\H})}\leq\mu\norm{x-x_{\H}}.
\end{equation*}
By triangle inequality,
\begin{equation*}
    \norm{\nabla Q_i(x)}\leq\norm{\nabla Q_i(x_{\H})}+\mu\norm{x-x_{\H}}.
\end{equation*}
Substituting from~\eqref{eqn:honest-norm-bound} in Lemma~\ref{lemma:bounding-gradients-at-xH} above, we obtain that
\begin{equation}
    \norm{\nabla Q_i(x)}\leq2(n-2f)\mu\epsilon+\mu\norm{x-x_{\H}}\leq2n\mu\epsilon+\mu\norm{x-x_{\H}}.
    \label{eqn:honest-bound-everywhere}
\end{equation}
% The last inequality in~\eqref{eqn:honest-bound-everywhere} follows from the fact that $f > 0$.\\
We use the above inequality~\eqref{eqn:honest-bound-everywhere} to show below that $\norm{\sum_{j=1}^{n-f}g_{i_j}^t}$ is bounded for all $t$. Recall that for each iteration $t$, 
\begin{equation*}
    \norm{g_{i_1}^t}\leq...\leq\norm{g_{i_{n-f}}^t}\leq\norm{g_{i_{n-f+1}}^t}\leq...\leq\norm{g_{i_n}^t}.
\end{equation*}
%With \eqref{eqn:update}, the construction of $\widehat{g_j^t}$, we have
%\begin{equation}
%    \norm{\widehat{g_j^t}}\leq\norm{g_{i_{n-f}}^t}, ~\forall j\in[n],~t\in\mathbb{Z}_{\geq0}.
%    \label{eqn:norm-upperbound}
%\end{equation}
As there are at most $f$ Byzantine agents, for each $t$ there exists $\sigma_t\in\H$ such that
\begin{equation}
    \norm{g_{i_{n-f}}^t}\leq\norm{g_{i_{\sigma_t}}^t}.
    \label{eqn:honest-bound}
\end{equation}
As $g_j^t=\nabla Q_j(x^t)$ for all $j\in\H$, from~\eqref{eqn:honest-bound} we obtain that
\begin{equation*}
    \norm{g_{i_j}^t}\leq\norm{\nabla Q_{\sigma_t}(x^t)}, \quad \forall j \in \{1, \ldots, n-f\}, ~ t.
\end{equation*}
Substituting from~\eqref{eqn:honest-bound-everywhere} above we obtain that for every $j \in \{1, \ldots, n-f\}$,
\begin{equation*}
    \norm{g_{i_j}^t}\leq\norm{g_{i_{n-f}}^t}\leq2n\mu\epsilon+\mu\norm{x^t-x_{\H}}.
\end{equation*}
Therefore, from triangle inequality,
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t}\leq\sum_{j=1}^{n-f}\norm{g_{i_j}^t}\leq(n-f)\left(2n\mu\epsilon+\mu\norm{x^t-x_{\H}}\right). \label{eqn:filtered-upperbound}
\end{equation}
Recall from~\eqref{eqn:x_H_W} that $x_{\H} \in \W$. Let $\Gamma = \max_{x \in \W} \norm{x - x_{\H}}$. As $\W$ is a compact set, $\Gamma < \infty$. Recall from the update rule~\eqref{eqn:update} that $x^t \in \W$ for all $t$. Thus, $\norm{x^t - x_{\H}} \leq \max_{x \in \W} \norm{x - x_{\H}} = \Gamma < \infty$. Substituting this in~\eqref{eqn:filtered-upperbound} implies that
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t} \leq (n-f) \left( 2n \mu \epsilon + \mu \Gamma\right) < \infty. 
\end{equation}
Recall that in this particular case, $\sum_{j=1}^{n-f}g_{i_j}^t = \gf\left(g^t_1, \ldots, \, g^t_n \right)$ (see~\eqref{eqn:cge_grad_filter_proof}). Therefore, from above we obtain that
\begin{align}
    \norm{\gf\left(g^t_1, \ldots, \, g^t_n \right)} < \infty, \quad \forall t. \label{eqn:cge_bnd_grd}
\end{align}
~

% Recall from the update rule~\eqref{eqn:update} that, for all $t \geq 0$,
% \begin{align*}
%     \norm{x^{t+1}-x^*}^2 &= \norm{\left[x^t - \eta_t\sum_{j=1}^{n-f}g_{i_j}^t\right]_{\W} - x^*}^2.
% \end{align*}
% Due to the well-known non-expansion property of projection onto a convex set (see~\cite{boyd2004convex}) we obtain that
% \begin{align*}
%     \norm{x^{t+1}-x^*}^2 &\leq \norm{x^t - \eta_t\sum_{j=1}^{n-f}g_{i_j}^t - x^*}^2 \\
%     &=\norm{x^t-x^*}^2 - 2\eta_t\iprod{x^t-x^*}{\sum_{j=1}^{n-f}g_{i_j}^t}+\eta_t^2\norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2.
% \end{align*}

% Recall that we defined in \eqref{eqn:D_cge} that 
% \begin{align}
%     \D\triangleq\cfrac{4\mu f}{\alpha\gamma}.
%     \label{eqn:D_cge_appdx}
% \end{align}
Next, we show that for an arbitrary $\delta>0$, %$\delta > 0$ there exists $\xi > 0$ such that
\begin{align}
    \phi_t\triangleq\iprod{x^t-x_{\H}}{\sum_{j=1}^{n-f}g_{i_j}^t} \geq \alpha n\gamma\delta\left(\cfrac{4\mu f}{\alpha\gamma}\epsilon+\delta\right)>0 ~ \text{ when } ~ \norm{x^t-x_{\H}} \geq \cfrac{4\mu f}{\alpha\gamma}\epsilon + \delta, \nonumber
\end{align}
where $\alpha$ is defined by \eqref{eqn:alpha}.

% Therefore, 
% \begin{equation}
%     \norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2\leq(n-f)^2\left(2n\mu\epsilon+\mu\norm{x^t-x^*}\right)^2. 
%     \label{eqn:square-filtered-gradients}
% \end{equation}


Consider an arbitrary iteration $t$. Note that, as $\mnorm{\H} = n-f$, there are at least $n-2f$ agents that are common to both sets $\H$ and $\{i_1,...,i_{n-f}\}$. We let $\H^t$ be an arbitrary set such that $\H^t \subset \{i_1,...,i_{n-f}\} \cap \H$ with $\mnorm{\H^t}=n-2f$. The remaining set of agents $\B^t = \{i_1,...,i_{n-f}\} \setminus \H^t$ may contain up to $f$ Byzantine agents. Note that $\mnorm{\H^t} = n-2f $ and $\mnorm{\B^t} =f$. We have
\begin{equation}
    \phi_t=\iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t}+\iprod{x^t-x_{\H}}{\sum_{k\in\B^t}g_k^t}.
    \label{eqn:phi-t-two-parts}
\end{equation}
Consider the first term on the right-hand side of~\eqref{eqn:phi-t-two-parts}. Recall that $g_j^t=\nabla Q_j(x^t)$ for all $j\in\H$. Therefore, 
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t} &= \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}\nabla Q_j(x^t)} - \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}\nabla Q_j(x_{\H})} + \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}\nabla Q_j(x_{\H})} \nonumber \\
    &= \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}\nabla Q_j(x^t)-\sum_{j\in\H^t}\nabla Q_j(x_{\H})} + \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}\nabla Q_j(x_{\H})}
    \label{eqn:phi_t_1}
\end{align}
For the first term in \eqref{eqn:phi_t_1}, by Assumption~\ref{assum:strongly-convex} of strong convexity, since $\mnorm{\H^t}=n-2f$, 

\comment{need to update Assumption~\ref{assum:strongly-convex} to size $n-2f$ sets}
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}\nabla Q_j(x^t)-\sum_{j\in\H^t}\nabla Q_j(x_{\H})}\geq \mnorm{\H^t}\gamma\norm{x^t-x_{\H}}^2.
    \label{eqn:phi_t_1_1}
\end{align}
For the second term in \eqref{eqn:phi_t_1}, by Cauchy-Schwarz inequality, 
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}\nabla Q_j(x_{\H})}\geq -\norm{x^t-x_{\H}}\cdot\norm{\sum_{j\in\H^t}\nabla Q_j(x_{\H})}.
\end{align}
Substituting from \eqref{eqn:lipschitz-distance-S1} in above, we further have
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}\nabla Q_j(x_{\H})}\geq-\norm{x^t-x_{\H}}\cdot \mnorm{\H^t}\mu\epsilon.
    \label{eqn:phi_t_1_2}
\end{align}
Substituting from \eqref{eqn:phi_t_1_1} and \eqref{eqn:phi_t_1_2} in \eqref{eqn:phi_t_1}, we have
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t} &\geq \mnorm{\H^t}\gamma\norm{x^t-x_{\H}}^2 - \norm{x^t-x_{\H}}\cdot \mnorm{\H^t}\mu\epsilon
    \label{eqn:phi_t_1-result}
\end{align}

Next, for the second term on the right-hand side of~\eqref{eqn:phi-t-two-parts}, we have
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{k\in\B^t}g_k^t} = \sum_{k\in\B^t}\iprod{x^t-x_{\H}}{g_k^t}.
    \label{eqn:phi-t-2}
\end{align}
From the Cauchy-Schwartz inequality, 
\begin{equation}
    \iprod{x^t-x_{\H}}{g_k^t}\geq-\norm{x^t-x_{\H}}\, \norm{g_k^t}.
    \label{eqn:iprod-single}
\end{equation}
Also, note that due to the Cauchy-Schwartz inequality, 
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H\backslash\H^t}\nabla Q_j(x^t)}&=\sum_{j\in\H\backslash\H^t}\iprod{x^t-x_{\H}}{\nabla Q_j(x^t)} \leq\sum_{j\in\H\backslash\H^t}\norm{x^t-x_{\H}}\, \norm{\nabla Q_j(x^t)}.
    \label{eqn:inner-prod-h-ht}
\end{align}
Suppose the number of Byzantine agents in $\B^t$ is $f'\leq f$. Since $\H^t + \B^t = \{i_1,...,i_{n-f}\}$ and $\mnorm{\H}=n-f$, there are at least $f'$ non-faulty agents in $\H\backslash\{i_1,...,i_{n-f}\} = \{i_{n-f+1},...,i_n\}$. Therefore, due to the sorting of the gradients, for each Byzantine agent $k \in \B^t$, there is a unique non-faulty agent $\sigma_k \in \{i_{n-f+1},...,i_n\}$,
% for each $k \in \B^t$ there exists $j \in \H\backslash\H^t$ such that 
such that
\begin{equation}
    \norm{g_k^t}\leq\norm{g_{\sigma_k}^t}=\norm{\nabla Q_{\sigma_k}(x^t)}. \label{eqn:k_B_j_H}
\end{equation}
Let us also designate $\sigma_k = k$ for every non-faulty agent $k\in\B^t$. For each non-faulty $k\in\B^t$, we also have
\begin{equation}
    \norm{g_k^t}=\norm{g_{\sigma_k}^t}=\norm{\nabla Q_{\sigma_k}(x^t)}. \label{eqn:k_B_j_H_2}
\end{equation}
Consider the set of agents $\H'_t = \{\sigma_k \textrm{ for all }k\in\B^t\}$. It follows that $\H'_t$ is a set of non-faulty agents with $\mnorm{\H'_t}=f$.
Therefore,~\eqref{eqn:k_B_j_H} and~\eqref{eqn:k_B_j_H_2} imply that
\begin{align}
    \sum_{k \in \B^t} \norm{g_k^t} \leq \sum_{j \in \H'_t} \norm{\nabla Q_j(x^t)}.
    \label{eqn:bound-good-bad}
\end{align}
Combining \eqref{eqn:phi-t-2}, \eqref{eqn:iprod-single}, \eqref{eqn:inner-prod-h-ht} and~\eqref{eqn:bound-good-bad}, we have
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{k\in\B^t}g_k^t}\geq-\sum_{i\in\B^t}\norm{x^t-x_{\H}}\norm{g_k^t}\geq-\norm{x^t-x_{\H}}\sum_{i\in\H'_t}\norm{\nabla Q_i(x^t)}.
\end{align}
Substituting from \eqref{eqn:honest-bound-everywhere}, i.e., $\norm{\nabla Q_i(x)}\leq2(n-2f)\mu\epsilon+\mu\norm{x-x_{\H}}$, above we obtain that
% . With \eqref{eqn:honest-bound-everywhere}, 
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{k\in\B^t}g_k^t}\geq-\norm{x^t-x_{\H}}\cdot \mnorm{\H'_t}(2(n-2f)\mu\epsilon + \mu\norm{x^t-x_{\H}}).
    \label{eqn:phi_t_2-result}
\end{align}

Substituting from \eqref{eqn:phi-t-two-parts} in \eqref{eqn:phi_t_1-result} and \eqref{eqn:phi_t_2-result}, we have
\begin{align}
    \phi_t\geq \mnorm{\H^t}\gamma\norm{x^t-x_{\H}}^2 - \norm{x^t-x_{\H}}\cdot \mnorm{\H^t}\mu\epsilon -\norm{x^t-x_{\H}}\cdot \mnorm{\H'_t}(2(n-2f)\mu\epsilon + \mu\norm{x^t-x_{\H}}).
\end{align}
As $\mnorm{\H^t}=n-2f$ and $\mnorm{\H'_t}=f$, the above implies that
\begin{align}
    \phi_t &\geq (n-2f)\gamma\norm{x^t-x_{\H}}^2 - \norm{x^t-x_{\H}}\cdot(n-2f)\mu\epsilon -\norm{x^t-x_{\H}}\cdot f(2(n-2f)\mu\epsilon + \mu\norm{x^t-x_{\H}})  \nonumber \\
    &=(\gamma(n-2f)-\mu f)\norm{x^t-x_{\H}}\left(\norm{x^t-x_{\H}} - \frac{(1 + 2f)(n-2f)\mu\epsilon}{\gamma(n-2f)-\mu f}\right) \nonumber \\
    &=n\gamma\left(1-\frac{f}{n}\left(\frac{2\gamma+\mu}{\gamma}\right)\right)\norm{x^t-x_{\H}}\left(\norm{x^t-x_{\H}}-\frac{(1 + 2f)(n-2f)\mu\epsilon}{n\gamma\left(1-\frac{f}{n}\left(\frac{2\gamma+\mu}{\gamma}\right)\right)}\right)
    \label{eqn:phi-t-pre-final}
\end{align}

Recall from~\eqref{eqn:alpha} that

\comment{
need to update \eqref{eqn:alpha}
}
$$\alpha = 1-\frac{f}{n}\left(\frac{2\gamma+\mu}{\gamma}\right). $$
Substituting from above in~\eqref{eqn:phi-t-pre-final} we obtain that
% \[\D = \frac{4\mu f}{\alpha\gamma}\]
% and 
% $$\D = \dfrac{4n\mu f}{n\gamma\left(1-\dfrac{f}{n}\left(1+\dfrac{2\mu}{\gamma}\right)\right)}=\frac{4\mu f}{\alpha\gamma}.$$
% We have
\begin{align}
    \phi_t \geq \alpha \, n \gamma \,\norm{x^t-x_{\H}}\, \left(\norm{x^t-x_{\H}}- \frac{(1+2f)(n-2f)\mu}{\alpha n\gamma} \epsilon \right).
    \label{eqn:phi-t-final}
\end{align}
% Recall that in \eqref{eqn:D_cge_appdx} we defined $\D=\cfrac{4\mu f}{\alpha\gamma}$. 
As it is assumed that $\alpha > 0$,~\eqref{eqn:phi-t-final} implies that for an arbitrary $\delta>0$,
\begin{align}
    \phi_t \geq \alpha n \gamma \delta\left(\frac{(1+2f)(n-2f)\mu}{\alpha n\gamma} \epsilon+\delta\right) > 0 ~ \text{ when } \norm{x^t-x_{\H}} \geq \frac{(1+2f)(n-2f)\mu}{\alpha n\gamma} \epsilon+\delta.
    \label{eqn:test}
\end{align}
\comment{
The above bound is roughly:
\begin{align*}
    \frac{(1+2f)(n-2f)\mu}{\alpha n\gamma} \epsilon \geq \frac{(1+2f)\mu}{\alpha\gamma} \epsilon.
\end{align*}
For comparison, the old bound is provided by the inequality below: (replaced by \eqref{eqn:test})
\begin{align*}
    \phi_t \geq \alpha n \gamma \delta\left(\cfrac{4\mu f}{\alpha\gamma}\epsilon+\delta\right) > 0 ~ \text{ when } \norm{x^t-x_{\H}} \geq \cfrac{4\mu f}{\alpha\gamma}\epsilon+\delta.
\end{align*}}
Hence, the proof.
% $\lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \not> \D \, \epsilon$. Hence, and therefore, $\lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \leq \D \, \epsilon$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{Proof of Theorem~\ref{thm:conv-rate}}
\label{sub:proof_2}
From the update rule~\eqref{eqn:update}, and the non-expansion property of projection onto a convex set, we obtain that for all $t \geq 0$,
\begin{align}
    \norm{x^{t+1}-x_{\H}}^2 \leq \norm{x^t-x_{\H}}^2-2\eta_t\phi_t+\eta_t^2\norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2 \label{eqn:conv_exp_1}
\end{align}
where $\phi_t\triangleq\iprod{x^t-x_{\H}}{\sum_{j=1}^{n-f}g_{i_j}^t}$. From~\eqref{eqn:filtered-upperbound}, we obtain that
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2\leq(n-f)^2\left(2n\mu\epsilon+\mu\norm{x^t-x_{\H}}\right)^2. 
    \label{eqn:square-filtered-gradients}
\end{equation}
Substituting from~\eqref{eqn:square-filtered-gradients} and~\eqref{eqn:phi-t-final} in~\eqref{eqn:conv_exp_1} we obtain that
\begin{align*}
    \norm{x^{t+1}-x_{\H}}^2 &\leq (1-2\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+2\eta_t\alpha n \gamma\D\epsilon\norm{x^t-x_{\H}} \nonumber \\
        & + \eta_t^2\mu^2(n-f)^2 \left(\norm{x^t-x_{\H}}+2n\epsilon \right)^2 \\
        & \leq(1-2\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+2\eta_t\alpha n \gamma\D\epsilon\norm{x^t-x_{\H}} \nonumber \\
        & + \eta_t^2\mu^2n^2 \left(\norm{x^t-x_{\H}}+2n\epsilon \right)^2.
\end{align*}
As $2\D\epsilon\norm{x^t-x_{\H}}\leq\norm{x^t-x_{\H}}^2+\D^2\epsilon^2$ and $\norm{x^t - x_{\H}} \leq \Gamma$ for all $t$ (due to the projection of the estimates onto the hypercube $\W$), the above implies that
\begin{align}
    \norm{x^{t+1}-x_{\H}}^2&\leq(1-\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+\eta_t\alpha n\gamma\D^2\epsilon^2+\eta_t^2\mu^2n^2(\Gamma+2n\epsilon)^2. \label{eqn:before_step-size}
\end{align}
Upon substituting the step size $\eta_t=\left(\frac{2}{\alpha n\gamma}\right)\frac{1}{t+1}$ for all $t$ in~\eqref{eqn:before_step-size} we obtain that
\begin{equation*}
    \norm{x^{t+1}-x_{\H}}^2\leq\left(1-\dfrac{2}{t+1}\right)\norm{x^t-x_{\H}}^2+\dfrac{2}{t+1}\D^2\epsilon^2+\left(\dfrac{1}{t+1}\right)^2\dfrac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2.
\end{equation*}
We let
\begin{equation}
    \L = \dfrac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2.
\end{equation}
Thus, for all $t \geq 0$,
\begin{equation}
    \norm{x^{t+1}-x_{\H}}^2\leq\left(\dfrac{t-1}{t+1}\right)\norm{x^t-x_{\H}}^2+\dfrac{2}{t+1}\D^2\epsilon^2+\left(\dfrac{1}{t+1}\right)^2\L.
    \label{eqn:distance-recursive}
\end{equation}
Note that, as $\alpha < 1$ and $\mu \geq \gamma$ (under Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex}), 
\begin{equation*}
    \L \geq 4\Gamma^2.
\end{equation*}
Therefore, as $x^1 \in \W$,
\begin{align}
    \norm{x^1-x_{\H}}^2 \leq \Gamma^2 \leq \frac{\L}{4} \leq \frac{\L}{4} + \D^2\epsilon^2. \label{eqn:ind_1}
\end{align}
~

Next, we reason by induction that for all $t \geq 1$,
\begin{equation}
    \norm{x^t-x_{\H}}^2 \leq \dfrac{1}{t+1}\L + \D^2\epsilon^2. \label{eqn:main_conv}
\end{equation}
The above inequality holds true for $t = 1$ as shown above in~\eqref{eqn:ind_1}. Now, suppose that~\eqref{eqn:main_conv} is true for $t = \tau$ where $\tau$ is an arbitrary integer greater than $1$, i.e., 
\begin{equation*}
    \norm{x^\tau - x_{\H}} \leq \dfrac{1}{\tau+1}\L + \D^2\epsilon^2.
\end{equation*}
We show below that~\eqref{eqn:main_conv} also holds true for $t = \tau + 1$. Substituting from above in~\eqref{eqn:distance-recursive} for $t = \tau $ we obtain that
\begin{align}
    \norm{x^{\tau+1}-x_{\H}} &\leq \left( \dfrac{\tau-1}{\tau+1}\right) \left(\dfrac{\L}{\tau+1}+ \D^2\epsilon^2 \right) + \dfrac{2}{\tau+1} \D^2 + \left(\dfrac{1}{\tau+1}\right)^2 \L \nonumber \\
    &=\dfrac{\tau}{(\tau+1)^2}\L. \label{eqn:ind_last}%+\D^2\leq\dfrac{1}{t+2}\L(f,\epsilon)+\D^2.
\end{align}
Note that for $\tau \geq 0$, $\tau (\tau + 2) \leq (\tau +1)^2$, or
\begin{equation*}
    \dfrac{\tau}{(\tau+1)^2}\leq\dfrac{1}{\tau+2}.
\end{equation*}
Therefore,~\eqref{eqn:ind_last} implies that
\begin{equation}
    \norm{x^{\tau+1}-x_{\H}}=\dfrac{\tau}{(\tau+1)^2}\L + \D^2 \epsilon^2 \leq \dfrac{1}{\tau+2} \L + \D^2\epsilon^2. \label{eqn:last}
\end{equation}
As $\L = \frac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2 = \left(\frac{2 \mu (\Gamma + 2n\epsilon)}{\alpha \gamma} \right)^2$,~\eqref{eqn:last} proves the theorem.

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> gradient_proof-podc.tex <==
\section{Appendix: Lemma~\ref{lemma:upbd-vector}} % on the upper bound of the norm of vectors knowing the upper bound of the norm of the sum of these vectors}
\label{app:lemma}

\begin{lemma}
    \label{lemma:upbd-vector}
    For $n$ vectors $a_1,...,a_n$ and a positive number $f\leq n/2$, if there exists some real number $r\geq0$, such that for any set $S\subset[n]$ with $\mnorm{S}=f$ we have
    \begin{align}
        \norm{\sum_{i\in S}a_i}\leq r,
        \label{eqn:lemma-condition}
    \end{align}
    then for all $i\in[n]$ we also have
    \begin{align}
        \norm{a_i}\leq 2r.
    \end{align}
\end{lemma}
Let us first introduce some notations. For two vectors $a,b$, denote by $[a]_b$ the vector projection of $a$ onto $b$. Also, denote by $\boldsymbol{e}_b$ the unit vector on the direction of $b$.
\begin{proof}
    The proof is by contradiction. Suppose for some $k$, $s\triangleq\norm{a_k}>2r$. By \eqref{eqn:lemma-condition}, for any set $S'\subset[n]$ with $\mnorm{S'}=f-1$, we have
    \begin{align}
        \norm{\sum_{i\in S'}a_i + a_{k}}\leq r.
    \end{align}
    Due to the additivity and the non-expansion property of vector projection, 
    \begin{align}
        \norm{\left[\sum_{i\in S'}a_i + a_{k}\right]_{a_{k}}}=\norm{\left[\sum_{i\in S'}a_i\right]_{a_{k}}+a_{k}} \leq \norm{\sum_{i\in S'}a_i+a_{k}}\leq r.
    \end{align}
    Let $t$ be a real value such that $\left[\sum_{i\in S'}a_i\right]_{a_{k}} = t\cdot \boldsymbol{e}_{a_k}$. It follows that 
    \begin{align}
        \norm{\left[\sum_{i\in S'}a_i\right]_{a_{k}}+a_{k}} = \norm{(t + s)\boldsymbol{e}_{a_k}} = \mnorm{t+s} \leq r.
    \end{align}
    Therefore, $t+s\leq r$. So $t\leq r-s<r-2r=-r$.

    On the other hand, for any $j\in[n]$, $j\neq k$, by \eqref{eqn:lemma-condition}, we also have
    \begin{align}
        \norm{\sum_{i\in S'}a_i + a_j}\leq r.
    \end{align}
    Similarly, due to the non-expansion property of vector projection,
    \begin{align}
        \norm{\left[\sum_{i\in S'}a_i + a_j\right]_{a_{k}}}\leq \norm{\sum_{i\in S'}a_i+a_j}\leq r.
    \end{align}
    Let $t'$ be a real value such that ${\left[a_j\right]_{a_{k}}} = t'\cdot \boldsymbol{e}_{a_k}$. It follows that 
    \begin{align}
        \norm{\left[\sum_{i\in S'}a_i + a_j\right]_{a_{k}}} = \norm{(t'+t)\boldsymbol{e}_{a_k}} = \norm{t'+t}\leq r.
    \end{align}
    Since $t<-r$, we have $t'>0$.

    Since $f\leq n/2$, there are at least $f$ different element that is in $[n]$ but not in $S'\cup\{k\}$. Let $f-1$ of them be a set $S''$. We have
    \begin{align}
        \norm{\sum_{i\in S''}a_i+a_{k}}&\geq \norm{\left[\sum_{i\in S''}a_i+a_{k}\right]_{a_{k}}}\geq \norm{\sum_{i\in S''}\left[a_i\right]_{a_{k}}+a_{k}} \nonumber \\
        &\geq\norm{(\mnorm{S}t'+2r)\cdot\boldsymbol{e}_{a_{k}}} = \mnorm{\mnorm{S}t' + 2r} = \mnorm{S}t'+2r>2r.
    \end{align}
    However, since $\mnorm{S''\cup\{k\}}=f$, by \eqref{eqn:lemma-condition}, 
    \begin{align}
        \norm{\sum_{i\in S''}a_i+a_{k}}<r.
    \end{align}
    Contradiction. Hence the proof.
\end{proof}

\section{Appendix: Lemma~\ref{lemma:bounding-gradients-at-xH} on the upper bound of the norm of gradients with $(2f,\epsilon)$-redundancy}

We assume $f > 0$ to ignore the trivial case of $f = 0$. We also assume $f\leq n/2$. 

Consider an arbitrary set $\H$ of non-faulty agents with $\mnorm{\H} = n-f$. Recall that under Assumptions~\ref{assum:strongly-convex} and~\ref{assum:compact}, the aggregate cost function $\sum_{i \in \H} Q_i(x)$ has a unique minimum point in set $\W$, which we denote by $x_{\H}$. Specifically, 
\begin{align}
    \left\{x_{\H} \right\} = \W \cap \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x). \label{eqn:x_H_W}
\end{align}

\begin{lemma}
    \label{lemma:bounding-gradients-at-xH}
    Suppose a group of $n$ cost functions $Q_i(x)$'s satisfies $(2f,\epsilon)$-redundancy, and Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex} hold. 
    % Suppose $x_{\H}\in\arg\min_x\sum_{i\in\H}Q_i(x)$ of any set $\H\subset[n]$ with $\mnorm{\H}=n-f$. 
    Then for any $j\in[n]$ and any set $\H\subset[n]$ with $\mnorm{\H}=n-f$, we have
    \begin{align}
        \norm{\nabla Q_j(x_\H)} \leq 2(n-2f)\mu\epsilon.
    \label{eqn:honest-norm-bound}
    \end{align}
\end{lemma}

\begin{proof}
    Consider any subset $S_1 \subset \H$ with $\mnorm{S_1} = n-2f$. From triangle inequality, $\forall x \in \R^d$,
\begin{align*}
    \norm{\sum_{j\in S_1}\nabla Q_j(x)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \sum_{j \in S_1}\norm{\nabla Q_j(x) - \nabla Q_j(x_{\H})}.
\end{align*}
Under Assumption~\ref{assum:lipschitz}, i.e., Lipschitz continuity of non-faulty gradients, for each non-faulty agent $j$, $\norm{\nabla Q_j(x) - \nabla Q_j(x_{\H})} \leq \mu \norm{x - x_{\H}}$. Substituting this above implies that 
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \, \norm{x-x_{\H}}.
    \label{eqn:lipschitz-distance}
\end{equation}
As $\mnorm{S_1} = n-2f$, the $(2f,\epsilon)$-redundancy property defined in Definition~\ref{def:approx_red} implies that for all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$,
\[\norm{x_1-x_{\H}} \leq \epsilon.\]
Substituting from above in~\eqref{eqn:lipschitz-distance} implies that, for all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$,
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x_1)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \, \norm{x_1-x_{\H}} \leq \mnorm{S_1} \mu \epsilon.
    \label{eqn:lipschitz-distance-2}
\end{equation}
For all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$, $\sum_{j\in S_1}\nabla Q_j(x_1) = 0$. Thus,~\eqref{eqn:lipschitz-distance-2} implies that
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \epsilon.
    \label{eqn:lipschitz-distance-S1}
\end{equation}
For all $x_{\H}\in\arg\min_x\sum_{j\in\H}Q_j(x)$, $\sum_{j\in\H}\nabla Q_j(x_{\H})=0$. Thus, with $\mnorm{S_1}=n-2f$, \eqref{eqn:lipschitz-distance-S1} implies that 
\begin{align}
    \norm{\sum_{j\in\H\backslash S_1}\nabla Q_j(x_{\H})} = \norm{\sum_{j\in\H}\nabla Q_j(x_{\H}) - \sum_{j\in S_1}\nabla Q_j(x_{\H})} = \norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq (n-2f)\mu\epsilon.
\end{align}
Note that $\mnorm{\H\backslash S_1}=f$. Since the choices of $\H$ and $S_1$ are arbitrary, the above implies that for any subset of agents $T\subset[n]$ with $\mnorm{T}=f$, we have
\begin{align}
    \norm{\sum_{j\in T}\nabla Q_j(x_{\H})} \leq (n-2f)\mu\epsilon.
    \label{eqn:lipschitz-distance-S1-complement}
\end{align}
Since we assumed that $f\leq n/2$, by Lemma~\ref{lemma:upbd-vector}, from above we have for all $j\in[n]$,
\begin{align*}
    \norm{\nabla Q_j(x_{\H})} \leq 2(n-2f)\mu\epsilon.
    % \label{eqn:honest-norm-bound}
\end{align*}
\end{proof}

\section{Appendix: Proof of Theorem~\ref{thm:conv-guarantee}}
\label{app:proof_1}

% In this section, we present the proof of Theorem~\ref{thm:conv-guarantee}.
Throughout, we assume $f > 0$ to ignore the trivial case of $f = 0$.\\
% % Throughout this section we denote the set of non-faulty agents by $\H$. Recall that $\mnorm{\H} \geq n-f$. Recall that $x^*$ denotes the true minimum point of the non-faulty agents' aggregate cost function $\sum_{i \in \H} Q_i(x)$. We 

% \subsection{Proof of Theorem~\ref{thm:conv-guarantee}}
% \label{sub:proof_1}
Consider an arbitrary set $\H$ of non-faulty agents with $\mnorm{\H} = n-f$. Recall that under Assumptions~\ref{assum:strongly-convex} and~\ref{assum:compact}, the aggregate cost function $\sum_{i \in \H} Q_i(x)$ has a unique minimum point in set $\W$, which we denote by $x_{\H}$. Specifically, 
\begin{align}
    \left\{x_{\H} \right\} = \W \cap \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x). \label{eqn:x_H_W}
\end{align}
% \[x_{\H} = \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x).\]
% To prove the theorem we make use of the result stated in Theorem~\ref{thm:upper-bound-D}. Specifically, we show is that the CGE gradient-filter satisfies the conditions of Theorem~\ref{thm:upper-bound-D} for $\D^* = \D \, \epsilon$, and $x^* = x_{\H}$. The rest follows easily from the convergence result stated in Theorem~\ref{thm:upper-bound-D}. 
Recall from~\eqref{eqn:cge_gf} that for CGE gradient-filter, in update rule~\eqref{eqn:update},
\begin{align}
    \gf\left(g^t_1, \ldots, \, g^t_n \right) = \sum_{j=1}^{n-f}g_{i_j}^t, \quad \forall t. \label{eqn:cge_grad_filter_proof}
\end{align}
~

First, we show that $\norm{\sum_{j=1}^{n-f}g_{i_j}^t} < \infty, ~ \forall t$. 
% Now, consider an arbitrary non-faulty agent $i \in \H\setminus S_1$. Let $S_2=S_1\cup\{i\}$. 
% % Also suppose $i\in\H\backslash S_1$, and $S_2=S_1\cup\{i\}$. By Assumption \ref{assum:lipschitz}, there exists some $\mu$, such that %$(2f,\epsilon)$-redundancy, 
% % For any $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$, by $(2f,\epsilon)$-redundancy, $\norm{x_1-x^*}\leq\epsilon$. Combining with \eqref{eqn:lipschitz-distance}
% % \begin{equation}
% %     \norm{\sum_{j\in S_1}\nabla Q_j(x^*)}=\norm{\sum_{j\in S_1}\nabla Q_j(x_1)-\sum_{j\in S_1}\nabla Q_j(x^*)}\leq\mu\epsilon.
% % \end{equation}
% Using similar arguments as above we obtain that under the $(2f, \, \epsilon)$-redundancy property and Assumption~\ref{assum:lipschitz}, for all $x_2\in\arg\min_x\sum_{j\in S_2}Q_j(x)$,
% \begin{align}
%     \norm{\sum_{j\in S_2}\nabla Q_j(x_{\H})}=\norm{\sum_{j\in S_2}\nabla Q_j(x_2)-\sum_{j\in S_2}\nabla Q_j(x_{\H})}\leq\mnorm{S_2}\mu\epsilon.
% \end{align}
% Note that $\sum_{j\in S_2}\nabla Q_j(x)=\sum_{j\in S_1}\nabla Q_j(x)+\nabla Q_i(x)$. From triangle inequality,
% \begin{equation}
%     \norm{\nabla Q_i(x_{\H})}-\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})}\leq\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})+\nabla Q_i(x_{\H})}.
% \end{equation}
% Therefore, for each non-faulty agent $i\in\H$, 
% \begin{align}
%     \norm{\nabla Q_i(x_{\H})}&\leq\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})+\nabla Q_i(x_{\H})}+\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq\mnorm{S_2}\mu\epsilon+\mnorm{S_1}\mu\epsilon \nonumber\\
%     & = (n-2f+1)\mu \epsilon + (n-2f) \mu \epsilon = (2n-4f+1)\mu\epsilon.
%     \label{eqn:honest-norm-bound}
% \end{align}
For all $x$ and $i\in\H$, by Assumption \ref{assum:lipschitz},
\begin{equation*}
    \norm{\nabla Q_i(x)-\nabla Q_i(x_{\H})}\leq\mu\norm{x-x_{\H}}.
\end{equation*}
By triangle inequality,
\begin{equation*}
    \norm{\nabla Q_i(x)}\leq\norm{\nabla Q_i(x_{\H})}+\mu\norm{x-x_{\H}}.
\end{equation*}
Substituting from~\eqref{eqn:honest-norm-bound} in Lemma~\ref{lemma:bounding-gradients-at-xH} above, we obtain that
\begin{equation}
    \norm{\nabla Q_i(x)}\leq2(n-2f)\mu\epsilon+\mu\norm{x-x_{\H}}\leq2n\mu\epsilon+\mu\norm{x-x_{\H}}.
    \label{eqn:honest-bound-everywhere}
\end{equation}
% The last inequality in~\eqref{eqn:honest-bound-everywhere} follows from the fact that $f > 0$.\\
We use the above inequality~\eqref{eqn:honest-bound-everywhere} to show below that $\norm{\sum_{j=1}^{n-f}g_{i_j}^t}$ is bounded for all $t$. Recall that for each iteration $t$, 
\begin{equation*}
    \norm{g_{i_1}^t}\leq...\leq\norm{g_{i_{n-f}}^t}\leq\norm{g_{i_{n-f+1}}^t}\leq...\leq\norm{g_{i_n}^t}.
\end{equation*}
%With \eqref{eqn:update}, the construction of $\widehat{g_j^t}$, we have
%\begin{equation}
%    \norm{\widehat{g_j^t}}\leq\norm{g_{i_{n-f}}^t}, ~\forall j\in[n],~t\in\mathbb{Z}_{\geq0}.
%    \label{eqn:norm-upperbound}
%\end{equation}
As there are at most $f$ Byzantine agents, for each $t$ there exists $\sigma_t\in\H$ such that
\begin{equation}
    \norm{g_{i_{n-f}}^t}\leq\norm{g_{i_{\sigma_t}}^t}.
    \label{eqn:honest-bound}
\end{equation}
As $g_j^t=\nabla Q_j(x^t)$ for all $j\in\H$, from~\eqref{eqn:honest-bound} we obtain that
\begin{equation*}
    \norm{g_{i_j}^t}\leq\norm{\nabla Q_{\sigma_t}(x^t)}, \quad \forall j \in \{1, \ldots, n-f\}, ~ t.
\end{equation*}
Substituting from~\eqref{eqn:honest-bound-everywhere} above we obtain that for every $j \in \{1, \ldots, n-f\}$,
\begin{equation*}
    \norm{g_{i_j}^t}\leq\norm{g_{i_{n-f}}^t}\leq2n\mu\epsilon+\mu\norm{x^t-x_{\H}}.
\end{equation*}
Therefore, from triangle inequality,
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t}\leq\sum_{j=1}^{n-f}\norm{g_{i_j}^t}\leq(n-f)\left(2n\mu\epsilon+\mu\norm{x^t-x_{\H}}\right). \label{eqn:filtered-upperbound}
\end{equation}
Recall from~\eqref{eqn:x_H_W} that $x_{\H} \in \W$. Let $\Gamma = \max_{x \in \W} \norm{x - x_{\H}}$. As $\W$ is a compact set, $\Gamma < \infty$. Recall from the update rule~\eqref{eqn:update} that $x^t \in \W$ for all $t$. Thus, $\norm{x^t - x_{\H}} \leq \max_{x \in \W} \norm{x - x_{\H}} = \Gamma < \infty$. Substituting this in~\eqref{eqn:filtered-upperbound} implies that
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t} \leq (n-f) \left( 2n \mu \epsilon + \mu \Gamma\right) < \infty. 
\end{equation}
Recall that in this particular case, $\sum_{j=1}^{n-f}g_{i_j}^t = \gf\left(g^t_1, \ldots, \, g^t_n \right)$ (see~\eqref{eqn:cge_grad_filter_proof}). Therefore, from above we obtain that
\begin{align}
    \norm{\gf\left(g^t_1, \ldots, \, g^t_n \right)} < \infty, \quad \forall t. \label{eqn:cge_bnd_grd}
\end{align}
~

% Recall from the update rule~\eqref{eqn:update} that, for all $t \geq 0$,
% \begin{align*}
%     \norm{x^{t+1}-x^*}^2 &= \norm{\left[x^t - \eta_t\sum_{j=1}^{n-f}g_{i_j}^t\right]_{\W} - x^*}^2.
% \end{align*}
% Due to the well-known non-expansion property of projection onto a convex set (see~\cite{boyd2004convex}) we obtain that
% \begin{align*}
%     \norm{x^{t+1}-x^*}^2 &\leq \norm{x^t - \eta_t\sum_{j=1}^{n-f}g_{i_j}^t - x^*}^2 \\
%     &=\norm{x^t-x^*}^2 - 2\eta_t\iprod{x^t-x^*}{\sum_{j=1}^{n-f}g_{i_j}^t}+\eta_t^2\norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2.
% \end{align*}

% Recall that we defined in \eqref{eqn:D_cge} that 
% \begin{align}
%     \D\triangleq\cfrac{4\mu f}{\alpha\gamma}.
%     \label{eqn:D_cge_appdx}
% \end{align}
Next, we show that for an arbitrary $\delta>0$, %$\delta > 0$ there exists $\xi > 0$ such that
\begin{align}
    \phi_t\triangleq\iprod{x^t-x_{\H}}{\sum_{j=1}^{n-f}g_{i_j}^t} \geq \alpha n\gamma\delta\left(\cfrac{4\mu f}{\alpha\gamma}\epsilon+\delta\right)>0 ~ \text{ when } ~ \norm{x^t-x_{\H}} \geq \cfrac{4\mu f}{\alpha\gamma}\epsilon + \delta, \nonumber
\end{align}
where $\alpha$ is defined by \eqref{eqn:alpha}.

% Therefore, 
% \begin{equation}
%     \norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2\leq(n-f)^2\left(2n\mu\epsilon+\mu\norm{x^t-x^*}\right)^2. 
%     \label{eqn:square-filtered-gradients}
% \end{equation}


Consider an arbitrary iteration $t$. Note that, as $\mnorm{\H} = n-f$, there are at least $n-2f$ agents that are common to both sets $\H$ and $\{i_1,...,i_{n-f}\}$. We let $\H^t = \{i_1,...,i_{n-f}\} \cap \H$. The remaining set of agents $\B^t = \{i_1,...,i_{n-f}\} \setminus \H^t$ comprises of only faulty agents. Note that $\mnorm{\H^t} \geq n-2f $ and $\mnorm{\B^t} \leq f$. Therefore,
\begin{equation}
    \phi_t=\iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t}+\iprod{x^t-x_{\H}}{\sum_{k\in\B^t}g_k^t}.
    \label{eqn:phi-t-two-parts}
\end{equation}
Consider the first term in the right-hand side of~\eqref{eqn:phi-t-two-parts}. Note that
\begin{align*}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t}&=\iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t+\sum_{j\in\H\backslash\H^t}g_j^t-\sum_{j\in\H\backslash\H^t}g_j^t} \nonumber \\
    &=\iprod{x^t-x_{\H}}{\sum_{j\in\H}g_j^t}-\iprod{x^t-x_{\H}}{\sum_{j\in\H\backslash\H^t}g_j^t}.
\end{align*}
Recall that $g_j^t=\nabla Q_j(x^t)$, $\forall j\in\H$. Therefore,
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t}=&\iprod{x^t-x_{\H}}{\sum_{j\in\H}\nabla Q_j(x^t)} -\iprod{x^t-x_{\H}}{\sum_{j\in\H\backslash\H^t}\nabla Q_j(x^t)}. \label{eqn:first_phi_1}
\end{align}
~

\noindent Due to the strong convexity assumption (i.e., Assumption~\ref{assum:strongly-convex}), for all $x, \, y \in \W$,
\begin{equation}
    \iprod{x- y}{\nabla \sum_{j\in\H}Q_j(x)-\nabla\sum_{j\in\H} Q_j(y)} \geq \mnorm{\H}\, \gamma\norm{x-y}^2.
    \label{eqn:assum-strong-convex-restate}
\end{equation}
By the projection on $\W$ in update rule \eqref{eqn:update}, $x^t\in\W$ for all $t$. By \eqref{eqn:x_H_W}, $x_{\H}$ is also in $\W$. As $x_{\H}$ is minimum point of $\sum_{j \in \H}Q_j(x)$, $\nabla \sum_{j \in \H} Q_j(x_{\H}) = 0$. Thus, by \eqref{eqn:assum-strong-convex-restate} it follows that
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H}\nabla Q_j(x^t)} & = \iprod{x^t-x_{\H}}{\nabla\sum_{j\in\H}Q_j(x^t)-\nabla\sum_{j\in\H}Q_j(x_{\H})} \geq \mnorm{\H} \, \gamma\norm{x^t-x_{\H}}^2.
    \label{eqn:inner-prod-h}
\end{align}
Now, due to the Cauchy-Schwartz inequality, by \eqref{eqn:lipschitz-distance-S1-complement} we have
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H\backslash\H^t}\nabla Q_j(x^t)}& \leq\norm{x^t-x_{\H}}\cdot\norm{\sum_{j\in\H\backslash\H^t}\nabla Q_j(x^t)}\leq\norm{x^t-x_{\H}}\cdot(n-2f)\mu\epsilon.
    \label{eqn:inner-prod-h-ht-1}
\end{align}
Also, due to Cauchy-Schwarz inequality, 
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H\backslash\H^t}\nabla Q_j(x^t)}& \leq\norm{x^t-x_{\H}}\cdot\norm{\sum_{j\in\H\backslash\H^t}\nabla Q_j(x^t)}\leq\norm{x^t-x_{\H}}\cdot\sum_{j\in\H\backslash\H^t}\norm{\nabla Q_j(x^t)}
    \label{eqn:inner-prod-h-ht}
\end{align}
Substituting from~\eqref{eqn:inner-prod-h} and~\eqref{eqn:inner-prod-h-ht-1} in~\eqref{eqn:first_phi_1} we obtain that
\begin{equation}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t} \geq \gamma\mnorm{\H}\, \norm{x^t-x_{\H}}^2-(n-2f)\mu\epsilon\norm{x^t-x_{\H}}.
    \label{eqn:phi-t-first-part}
\end{equation}
~

Next, we consider the second term in the right-hand side of~\eqref{eqn:phi-t-two-parts}. From the Cauchy-Schwartz inequality, 
\begin{equation*}
    \iprod{x^t-x_{\H}}{g_k^t}\geq-\norm{x^t-x_{\H}}\, \norm{g_k^t}.
\end{equation*}
Substituting from~\eqref{eqn:phi-t-first-part} and above in~\eqref{eqn:phi-t-two-parts} we obtain that
\begin{equation}
    \phi_t\geq\gamma\mnorm{\H}\, \norm{x^t-x_{\H}}^2-\mnorm{\H\backslash\H^t}\mu\epsilon\norm{x^t-x_{\H}}-\sum_{k\in\B^t}\norm{x^t-x_{\H}}\, \norm{g_k^t}.
    \label{eqn:phi-t-2}
\end{equation}

Recall that, due to the sorting of the gradients, for an arbitrary $k \in \B^t$ and an arbitrary $j \in \H\backslash\H^t$,
% for each $k \in \B^t$ there exists $j \in \H\backslash\H^t$ such that 
\begin{equation}
    \norm{g_k^t}\leq\norm{g_j^t}=\norm{\nabla Q_j(x^t)}. \label{eqn:k_B_j_H}
\end{equation}
Recall that $\B^t = \{i_1, \ldots, \, i_{n-f}\} \setminus \H^t$. Thus, $\mnorm{\B^t} = n-f-\mnorm{\H^t}$. Also, as $\mnorm{\H} = n-f$, $\mnorm{\H\backslash\H^t} = n- f - \mnorm{\H^t}$. That is, $\mnorm{\B^t} = \mnorm{\H\backslash\H^t}$. Therefore,~\eqref{eqn:k_B_j_H} implies that
\begin{align*}
    \sum_{k \in \B^t} \norm{g_k^t} \leq \sum_{j \in \H\backslash\H^t} \norm{\nabla Q_j(x^t)}.
\end{align*}
Substituting from above in~\eqref{eqn:phi-t-2}, we obtain that
\begin{align*}
    \phi_t&\geq\gamma\mnorm{\H}\, \norm{x^t-x_{\H}}^2-(n-2f)\mu\epsilon\norm{x^t-x_{\H}}-\sum_{j\in\H\backslash\H^t}\norm{x^t-x_{\H}}\, \norm{\nabla Q_j(x^t)}.
\end{align*}
Substituting from \eqref{eqn:honest-bound-everywhere}, i.e., $\norm{\nabla Q_i(x)}\leq2n\mu\epsilon+\mu\norm{x-x_{\H}}$, above we obtain that
% . With \eqref{eqn:honest-bound-everywhere}, 
\begin{align*}
    \phi_t&\geq\gamma\mnorm{\H}\, \norm{x^t-x_{\H}}^2 - (n-2f)\mu\epsilon\norm{x^t-x_{\H}} - \mnorm{\H\backslash\H^t}\, \norm{x^t-x_{\H}}\, (2n\mu\epsilon+\mu\norm{x^t-x_{\H}}) \nonumber\\
    & \geq \left(\gamma\mnorm{\H}-\mu\mnorm{\H\backslash\H^t}\right)\norm{x^t-x_{\H}}^2 - (n-2f)\mu\epsilon\norm{x^t-x_{\H}}- 2(n-2f)\mu\epsilon \mnorm{\H\backslash\H^t}\, \norm{x^t-x_{\H}}.
\end{align*}
As $\mnorm{\H} = n-f$ and $\mnorm{\H\backslash\H^t}\leq f$, the above implies that
\begin{align}
\begin{split}
\label{eqn:phi-t-pre-final}
    \phi_t & \geq\left(\gamma(n-f)-\mu f\right)\norm{x^t-x_{\H}}^2-(n-2f)\mu\epsilon\norm{x^t-x_{\H}}-2(n-2f)\mu\epsilon f\, \norm{x^t-x_{\H}} \\
        & = \left(\gamma(n-f)-\mu f\right)\norm{x^t-x_{\H}}\, \left(\norm{x^t-x_{\H}}-\dfrac{(1+2f)(n-2f)\mu\epsilon}{\gamma(n-f)-\mu f} \right) \\
        & = n \gamma \, \left( 1 - \frac{f}{n} \left( 1 + \frac{\mu}{\gamma}\right)\right) \norm{x^t-x_{\H}} \, \left(\norm{x^t-x_{\H}} - \frac{(1+2f)(n-2f)\mu\epsilon}{n\gamma\left( 1 - \frac{f}{n}\left(1 + \frac{ \mu}{\gamma} \right)\right)} \right).
\end{split}
\end{align}
Recall from~\eqref{eqn:alpha} that
$$\alpha = 1-\dfrac{f}{n}\left(1+\dfrac{\mu}{\gamma}\right). $$
Substituting from above in~\eqref{eqn:phi-t-pre-final} we obtain that
% \[\D = \frac{4\mu f}{\alpha\gamma}\]
% and 
% $$\D = \dfrac{4n\mu f}{n\gamma\left(1-\dfrac{f}{n}\left(1+\dfrac{2\mu}{\gamma}\right)\right)}=\frac{4\mu f}{\alpha\gamma}.$$
% We have
\begin{align}
    \phi_t \geq \alpha \, n \gamma \,\norm{x^t-x_{\H}}\, \left(\norm{x^t-x_{\H}}- \frac{(1+2f)(n-2f)\mu}{\alpha n\gamma} \epsilon \right).
    \label{eqn:phi-t-final}
\end{align}
% Recall that in \eqref{eqn:D_cge_appdx} we defined $\D=\cfrac{4\mu f}{\alpha\gamma}$. 
As it is assumed that $\alpha > 0$,~\eqref{eqn:phi-t-final} implies that for an arbitrary $\delta>0$,
\begin{align*}
    \phi_t \geq \alpha n \gamma \delta\left(\cfrac{(1+2f)(n-2f)\mu}{\alpha n\gamma}\epsilon+\delta\right) > 0 ~ \text{ when } \norm{x^t-x_{\H}} \geq \cfrac{(1+2f)(n-2f)\mu}{\alpha n\gamma}\epsilon+\delta.
\end{align*}
Hence, the proof.
% $\lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \not> \D \, \epsilon$. Hence, and therefore, $\lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \leq \D \, \epsilon$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{Proof of Theorem~\ref{thm:conv-rate}}
\label{sub:proof_2}
From the update rule~\eqref{eqn:update}, and the non-expansion property of projection onto a convex set, we obtain that for all $t \geq 0$,
\begin{align}
    \norm{x^{t+1}-x_{\H}}^2 \leq \norm{x^t-x_{\H}}^2-2\eta_t\phi_t+\eta_t^2\norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2 \label{eqn:conv_exp_1}
\end{align}
where $\phi_t\triangleq\iprod{x^t-x_{\H}}{\sum_{j=1}^{n-f}g_{i_j}^t}$. From~\eqref{eqn:filtered-upperbound}, we obtain that
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2\leq(n-f)^2\left(2n\mu\epsilon+\mu\norm{x^t-x_{\H}}\right)^2. 
    \label{eqn:square-filtered-gradients}
\end{equation}
Substituting from~\eqref{eqn:square-filtered-gradients} and~\eqref{eqn:phi-t-final} in~\eqref{eqn:conv_exp_1} we obtain that
\begin{align*}
    \norm{x^{t+1}-x_{\H}}^2 &\leq (1-2\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+2\eta_t\alpha n \gamma\D\epsilon\norm{x^t-x_{\H}} \nonumber \\
        & + \eta_t^2\mu^2(n-f)^2 \left(\norm{x^t-x_{\H}}+2n\epsilon \right)^2 \\
        & \leq(1-2\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+2\eta_t\alpha n \gamma\D\epsilon\norm{x^t-x_{\H}} \nonumber \\
        & + \eta_t^2\mu^2n^2 \left(\norm{x^t-x_{\H}}+2n\epsilon \right)^2.
\end{align*}
As $2\D\epsilon\norm{x^t-x_{\H}}\leq\norm{x^t-x_{\H}}^2+\D^2\epsilon^2$ and $\norm{x^t - x_{\H}} \leq \Gamma$ for all $t$ (due to the projection of the estimates onto the hypercube $\W$), the above implies that
\begin{align}
    \norm{x^{t+1}-x_{\H}}^2&\leq(1-\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+\eta_t\alpha n\gamma\D^2\epsilon^2+\eta_t^2\mu^2n^2(\Gamma+2n\epsilon)^2. \label{eqn:before_step-size}
\end{align}
Upon substituting the step size $\eta_t=\left(\frac{2}{\alpha n\gamma}\right)\frac{1}{t+1}$ for all $t$ in~\eqref{eqn:before_step-size} we obtain that
\begin{equation*}
    \norm{x^{t+1}-x_{\H}}^2\leq\left(1-\dfrac{2}{t+1}\right)\norm{x^t-x_{\H}}^2+\dfrac{2}{t+1}\D^2\epsilon^2+\left(\dfrac{1}{t+1}\right)^2\dfrac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2.
\end{equation*}
We let
\begin{equation}
    \L = \dfrac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2.
\end{equation}
Thus, for all $t \geq 0$,
\begin{equation}
    \norm{x^{t+1}-x_{\H}}^2\leq\left(\dfrac{t-1}{t+1}\right)\norm{x^t-x_{\H}}^2+\dfrac{2}{t+1}\D^2\epsilon^2+\left(\dfrac{1}{t+1}\right)^2\L.
    \label{eqn:distance-recursive}
\end{equation}
Note that, as $\alpha < 1$ and $\mu \geq \gamma$ (under Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex}), 
\begin{equation*}
    \L \geq 4\Gamma^2.
\end{equation*}
Therefore, as $x^1 \in \W$,
\begin{align}
    \norm{x^1-x_{\H}}^2 \leq \Gamma^2 \leq \frac{\L}{4} \leq \frac{\L}{4} + \D^2\epsilon^2. \label{eqn:ind_1}
\end{align}
~

Next, we reason by induction that for all $t \geq 1$,
\begin{equation}
    \norm{x^t-x_{\H}}^2 \leq \dfrac{1}{t+1}\L + \D^2\epsilon^2. \label{eqn:main_conv}
\end{equation}
The above inequality holds true for $t = 1$ as shown above in~\eqref{eqn:ind_1}. Now, suppose that~\eqref{eqn:main_conv} is true for $t = \tau$ where $\tau$ is an arbitrary integer greater than $1$, i.e., 
\begin{equation*}
    \norm{x^\tau - x_{\H}} \leq \dfrac{1}{\tau+1}\L + \D^2\epsilon^2.
\end{equation*}
We show below that~\eqref{eqn:main_conv} also holds true for $t = \tau + 1$. Substituting from above in~\eqref{eqn:distance-recursive} for $t = \tau $ we obtain that
\begin{align}
    \norm{x^{\tau+1}-x_{\H}} &\leq \left( \dfrac{\tau-1}{\tau+1}\right) \left(\dfrac{\L}{\tau+1}+ \D^2\epsilon^2 \right) + \dfrac{2}{\tau+1} \D^2 + \left(\dfrac{1}{\tau+1}\right)^2 \L \nonumber \\
    &=\dfrac{\tau}{(\tau+1)^2}\L. \label{eqn:ind_last}%+\D^2\leq\dfrac{1}{t+2}\L(f,\epsilon)+\D^2.
\end{align}
Note that for $\tau \geq 0$, $\tau (\tau + 2) \leq (\tau +1)^2$, or
\begin{equation*}
    \dfrac{\tau}{(\tau+1)^2}\leq\dfrac{1}{\tau+2}.
\end{equation*}
Therefore,~\eqref{eqn:ind_last} implies that
\begin{equation}
    \norm{x^{\tau+1}-x_{\H}}=\dfrac{\tau}{(\tau+1)^2}\L + \D^2 \epsilon^2 \leq \dfrac{1}{\tau+2} \L + \D^2\epsilon^2. \label{eqn:last}
\end{equation}
As $\L = \frac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2 = \left(\frac{2 \mu (\Gamma + 2n\epsilon)}{\alpha \gamma} \right)^2$,~\eqref{eqn:last} proves the theorem.

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> gradient_proofs.tex <==
\section{Appendix: Proof of Theorem~\ref{thm:conv-guarantee}}
\label{app:proof_1}

% In this section, we present the proof of Theorem~\ref{thm:conv-guarantee}.
Throughout, we assume $f > 0$ to ignore the trivial case of $f = 0$.\\
% % Throughout this section we denote the set of non-faulty agents by $\H$. Recall that $\mnorm{\H} \geq n-f$. Recall that $x^*$ denotes the true minimum point of the non-faulty agents' aggregate cost function $\sum_{i \in \H} Q_i(x)$. We 

% \subsection{Proof of Theorem~\ref{thm:conv-guarantee}}
% \label{sub:proof_1}
Consider an arbitrary set $\H$ of non-faulty agents with $\mnorm{\H} = n-f$. Recall that under Assumptions~\ref{assum:strongly-convex} and~\ref{assum:compact}, the aggregate cost function $\sum_{i \in \H} Q_i(x)$ has a unique minimum point in set $\W$, which we denote by $x_{\H}$. Specifically, 
\begin{align}
    \left\{x_{\H} \right\} = \W \cap \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x). \label{eqn:x_H_W}
\end{align}
% \[x_{\H} = \arg \min_{x \in \R^d} \sum_{i \in \H} Q_i(x).\]
% To prove the theorem we make use of the result stated in Theorem~\ref{thm:upper-bound-D}. Specifically, we show is that the CGE gradient-filter satisfies the conditions of Theorem~\ref{thm:upper-bound-D} for $\D^* = \D \, \epsilon$, and $x^* = x_{\H}$. The rest follows easily from the convergence result stated in Theorem~\ref{thm:upper-bound-D}. 
Recall from~\eqref{eqn:cge_gf} that for CGE gradient-filter, in update rule~\eqref{eqn:update},
\begin{align}
    \gf\left(g^t_1, \ldots, \, g^t_n \right) = \sum_{j=1}^{n-f}g_{i_j}^t, \quad \forall t. \label{eqn:cge_grad_filter_proof}
\end{align}
~

First, we show that $\norm{\sum_{j=1}^{n-f}g_{i_j}^t} < \infty, ~ \forall t$. Consider a subset $S_1 \subset \H$ with $\mnorm{S_1} = n-2f$. From triangle inequality,
\begin{align*}
    \norm{\sum_{j\in S_1}\nabla Q_j(x)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \sum_{j \in S_1}\norm{\nabla Q_j(x) - \nabla Q_j(x_{\H})}, \quad \forall x \in \R^d.
\end{align*}
Under Assumption~\ref{assum:lipschitz}, i.e., Lipschitz continuity of non-faulty gradients, for each non-faulty agent $j$, $\norm{\nabla Q_j(x) - \nabla Q_j(x_{\H})} \leq \mu \norm{x - x_{\H}}$. Substituting this above implies that 
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \, \norm{x-x_{\H}}.
    \label{eqn:lipschitz-distance}
\end{equation}
As $\mnorm{S_1} = n-2f$, the $(2f,\epsilon)$-redundancy property defined in Definition~\ref{def:approx_red} implies that for all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$,
\[\norm{x_1-x_{\H}} \leq \epsilon.\]
Substituting from above in~\eqref{eqn:lipschitz-distance} implies that, for all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$,
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x_1)-\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \, \norm{x_1-x_{\H}} \leq \mnorm{S_1} \mu \epsilon.
    \label{eqn:lipschitz-distance-2}
\end{equation}
For all $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$, $\nabla Q_j(x_1) = 0$. Thus,~\eqref{eqn:lipschitz-distance-2} implies that
\begin{equation}
    \norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq \mnorm{S_1} \mu \epsilon.
    \label{eqn:lipschitz-distance-S1}
\end{equation}
Now, consider an arbitrary non-faulty agent $i \in \H\setminus S_1$. Let $S_2=S_1\cup\{i\}$. 
% Also suppose $i\in\H\backslash S_1$, and $S_2=S_1\cup\{i\}$. By Assumption \ref{assum:lipschitz}, there exists some $\mu$, such that %$(2f,\epsilon)$-redundancy, 
% For any $x_1\in\arg\min_x\sum_{j\in S_1}Q_j(x)$, by $(2f,\epsilon)$-redundancy, $\norm{x_1-x^*}\leq\epsilon$. Combining with \eqref{eqn:lipschitz-distance}
% \begin{equation}
%     \norm{\sum_{j\in S_1}\nabla Q_j(x^*)}=\norm{\sum_{j\in S_1}\nabla Q_j(x_1)-\sum_{j\in S_1}\nabla Q_j(x^*)}\leq\mu\epsilon.
% \end{equation}
Using similar arguments as above we obtain that under the $(2f, \, \epsilon)$-redundancy property and Assumption~\ref{assum:lipschitz}, for all $x_2\in\arg\min_x\sum_{j\in S_2}Q_j(x)$,
\begin{align}
    \norm{\sum_{j\in S_2}\nabla Q_j(x_{\H})}=\norm{\sum_{j\in S_2}\nabla Q_j(x_2)-\sum_{j\in S_2}\nabla Q_j(x_{\H})}\leq\mnorm{S_2}\mu\epsilon.
\end{align}
Note that $\sum_{j\in S_2}\nabla Q_j(x)=\sum_{j\in S_1}\nabla Q_j(x)+\nabla Q_i(x)$. From triangle inequality,
\begin{equation}
    \norm{\nabla Q_i(x_{\H})}-\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})}\leq\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})+\nabla Q_i(x_{\H})}.
\end{equation}
Therefore, for each non-faulty agent $i\in\H$, 
\begin{align}
    \norm{\nabla Q_i(x_{\H})}&\leq\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})+\nabla Q_i(x_{\H})}+\norm{\sum_{j\in S_1}\nabla Q_j(x_{\H})} \leq\mnorm{S_2}\mu\epsilon+\mnorm{S_1}\mu\epsilon \nonumber\\
    & = (n-2f+1)\mu \epsilon + (n-2f) \mu \epsilon = (2n-4f+1)\mu\epsilon.
    \label{eqn:honest-norm-bound}
\end{align}
Now, for all $x$ and $i\in\H$, by Assumption \ref{assum:lipschitz},
\begin{equation*}
    \norm{\nabla Q_i(x)-\nabla Q_i(x_{\H})}\leq\mu\norm{x-x_{\H}}.
\end{equation*}
By triangle inequality,
\begin{equation*}
    \norm{\nabla Q_i(x)}\leq\norm{\nabla Q_i(x_{\H})}+\mu\norm{x-x_{\H}}.
\end{equation*}
Substituting from~\eqref{eqn:honest-norm-bound} above we obtain that
\begin{equation}
    \norm{\nabla Q_i(x)}\leq(2n-4f+1)\mu\epsilon+\mu\norm{x-x_{\H}}\leq2n\mu\epsilon+\mu\norm{x-x_{\H}}.
    \label{eqn:honest-bound-everywhere}
\end{equation}
% The last inequality in~\eqref{eqn:honest-bound-everywhere} follows from the fact that $f > 0$.\\
We use the above inequality~\eqref{eqn:honest-bound-everywhere} to show below that $\norm{\sum_{j=1}^{n-f}g_{i_j}^t}$ is bounded for all $t$. Recall that for each iteration $t$, 
\begin{equation*}
    \norm{g_{i_1}^t}\leq...\leq\norm{g_{i_{n-f}}^t}\leq\norm{g_{i_{n-f+1}}^t}\leq...\leq\norm{g_{i_n}^t}.
\end{equation*}
%With \eqref{eqn:update}, the construction of $\widehat{g_j^t}$, we have
%\begin{equation}
%    \norm{\widehat{g_j^t}}\leq\norm{g_{i_{n-f}}^t}, ~\forall j\in[n],~t\in\mathbb{Z}_{\geq0}.
%    \label{eqn:norm-upperbound}
%\end{equation}
As there are at most $f$ Byzantine agents, for each $t$ there exists $\sigma_t\in\H$ such that
\begin{equation}
    \norm{g_{i_{n-f}}^t}\leq\norm{g_{i_{\sigma_t}}^t}.
    \label{eqn:honest-bound}
\end{equation}
As $g_j^t=\nabla Q_j(x^t)$ for all $j\in\H$, from~\eqref{eqn:honest-bound} we obtain that
\begin{equation*}
    \norm{g_{i_j}^t}\leq\norm{\nabla Q_{\sigma_t}(x^t)}, \quad \forall j \in \{1, \ldots, n-f\}, ~ t.
\end{equation*}
Substituting from~\eqref{eqn:honest-bound-everywhere} above we obtain that for every $j \in \{1, \ldots, n-f\}$,
\begin{equation*}
    \norm{g_{i_j}^t}\leq\norm{g_{i_{n-f}}^t}\leq2n\mu\epsilon+\mu\norm{x^t-x_{\H}}.
\end{equation*}
Therefore, from triangle inequality,
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t}\leq\sum_{j=1}^{n-f}\norm{g_{i_j}^t}\leq(n-f)\left(2n\mu\epsilon+\mu\norm{x^t-x_{\H}}\right). \label{eqn:filtered-upperbound}
\end{equation}
Recall from~\eqref{eqn:x_H_W} that $x_{\H} \in \W$. Let $\Gamma = \max_{x \in \W} \norm{x - x_{\H}}$. As $\W$ is a compact set, $\Gamma < \infty$. Recall from the update rule~\eqref{eqn:update} that $x^t \in \W$ for all $t$. Thus, $\norm{x^t - x_{\H}} \leq \max_{x \in \W} \norm{x - x_{\H}} = \Gamma < \infty$. Substituting this in~\eqref{eqn:filtered-upperbound} implies that
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t} \leq (n-f) \left( 2n \mu \epsilon + \mu \Gamma\right) < \infty. 
\end{equation}
Recall that in this particular case, $\sum_{j=1}^{n-f}g_{i_j}^t = \gf\left(g^t_1, \ldots, \, g^t_n \right)$ (see~\eqref{eqn:cge_grad_filter_proof}). Therefore, from above we obtain that
\begin{align}
    \norm{\gf\left(g^t_1, \ldots, \, g^t_n \right)} < \infty, \quad \forall t. \label{eqn:cge_bnd_grd}
\end{align}
~

% Recall from the update rule~\eqref{eqn:update} that, for all $t \geq 0$,
% \begin{align*}
%     \norm{x^{t+1}-x^*}^2 &= \norm{\left[x^t - \eta_t\sum_{j=1}^{n-f}g_{i_j}^t\right]_{\W} - x^*}^2.
% \end{align*}
% Due to the well-known non-expansion property of projection onto a convex set (see~\cite{boyd2004convex}) we obtain that
% \begin{align*}
%     \norm{x^{t+1}-x^*}^2 &\leq \norm{x^t - \eta_t\sum_{j=1}^{n-f}g_{i_j}^t - x^*}^2 \\
%     &=\norm{x^t-x^*}^2 - 2\eta_t\iprod{x^t-x^*}{\sum_{j=1}^{n-f}g_{i_j}^t}+\eta_t^2\norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2.
% \end{align*}
Next, we show that for an arbitrary $\delta > 0$ there exists $\xi > 0$ such that
\[\phi_t\triangleq\iprod{x^t-x_{\H}}{\sum_{j=1}^{n-f}g_{i_j}^t} \geq \xi ~ \text{ when } ~ \norm{x^t-x_{\H}} \geq \D \, \epsilon + \delta.\]

% Therefore, 
% \begin{equation}
%     \norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2\leq(n-f)^2\left(2n\mu\epsilon+\mu\norm{x^t-x^*}\right)^2. 
%     \label{eqn:square-filtered-gradients}
% \end{equation}


Consider an arbitrary iteration $t$. Note that, as $\mnorm{\H} = n-f$, there are at least $n-2f$ agents that are common to both sets $\H$ and $\{i_1,...,i_{n-f}\}$. We let $\H^t = \{i_1,...,i_{n-f}\} \cap \H$. The remaining set of agents $\B^t = \{i_1,...,i_{n-f}\} \setminus \H^t$ comprises of only faulty agents. Note that $\mnorm{\H^t} \geq n-2f $ and $\mnorm{\B^t} \leq f$. Therefore,
\begin{equation}
    \phi_t=\iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t}+\iprod{x^t-x_{\H}}{\sum_{k\in\B^t}g_k^t}.
    \label{eqn:phi-t-two-parts}
\end{equation}
Consider the first term in the right-hand side of~\eqref{eqn:phi-t-two-parts}. Note that
\begin{align*}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t}&=\iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t+\sum_{j\in\H\backslash\H^t}g_j^t-\sum_{j\in\H\backslash\H^t}g_j^t} \\ 
    &=\iprod{x^t-x_{\H}}{\sum_{j\in\H}g_j^t}-\iprod{x^t-x_{\H}}{\sum_{j\in\H\backslash\H^t}g_j^t}.
\end{align*}
Recall that $g_j^t=\nabla Q_j(x^t)$, $\forall j\in\H$. Therefore,
\begin{equation}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t}=\iprod{x^t-x_{\H}}{\sum_{j\in\H}\nabla Q_j(x^t)}-\iprod{x^t-x_{\H}}{\sum_{j\in\H\backslash\H^t}\nabla Q_j(x^t)}. \label{eqn:first_phi_1}
\end{equation}
~

\noindent Due to the strong convexity assumption (i.e., Assumption~\ref{assum:strongly-convex}), for all $x, \, y \in \R^d$,
\begin{equation*}
    \iprod{x- y}{\nabla \sum_{j\in\H}Q_j(x)-\nabla\sum_{j\in\H} Q_j(y)} \geq \mnorm{\H}\, \gamma\norm{x-y}^2.
\end{equation*}
As $x_{\H}$ is minimum point of $\sum_{j \in \H}Q_j(x)$, $\nabla \sum_{j \in \H} Q_j(x_{\H}) = 0$. Thus, 
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H}\nabla Q_j(x^t)} & = \iprod{x^t-x_{\H}}{\nabla\sum_{j\in\H}Q_j(x^t)-\nabla\sum_{j\in\H}Q_j(x_{\H})} \nonumber \\
    & \geq \mnorm{\H} \, \gamma\norm{x^t-x_{\H}}^2.
    \label{eqn:inner-prod-h}
\end{align}
Now, due to the Cauchy-Schwartz inequality, 
\begin{align}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H\backslash\H^t}\nabla Q_j(x^t)}&=\sum_{j\in\H\backslash\H^t}\iprod{x^t-x_{\H}}{\nabla Q_j(x^t)} \nonumber\\
    &\leq\sum_{j\in\H\backslash\H^t}\norm{x^t-x_{\H}}\, \norm{\nabla Q_j(x^t)}.
    \label{eqn:inner-prod-h-ht}
\end{align}
Substituting from~\eqref{eqn:inner-prod-h} and~\eqref{eqn:inner-prod-h-ht} in~\eqref{eqn:first_phi_1} we obtain that
\begin{equation}
    \iprod{x^t-x_{\H}}{\sum_{j\in\H^t}g_j^t} \geq \gamma\mnorm{\H}\, \norm{x^t-x_{\H}}^2-\sum_{j\in\H\backslash\H^t}\norm{x^t-x_{\H}}\, \norm{\nabla Q_j(x^t)}.
    \label{eqn:phi-t-first-part}
\end{equation}
~

Next, we consider the second term in the right-hand side of~\eqref{eqn:phi-t-two-parts}. From the Cauchy-Schwartz inequality, 
\begin{equation*}
    \iprod{x^t-x_{\H}}{g_k^t}\geq-\norm{x^t-x_{\H}}\, \norm{g_k^t}.
\end{equation*}
Substituting from~\eqref{eqn:phi-t-first-part} and above in~\eqref{eqn:phi-t-two-parts} we obtain that
\begin{equation}
    \phi_t\geq\gamma\mnorm{\H}\, \norm{x^t-x_{\H}}^2-\sum_{j\in\H\backslash\H^t}\norm{x^t-x_{\H}}\, \norm{\nabla Q_j(x^t)}-\sum_{k\in\B^t}\norm{x^t-x_{\H}}\, \norm{g_k^t}.
    \label{eqn:phi-t-2}
\end{equation}

Recall that, due to the sorting of the gradients, for an arbitrary $k \in \B^t$ and an arbitrary $j \in \H\backslash\H^t$,
% for each $k \in \B^t$ there exists $j \in \H\backslash\H^t$ such that 
\begin{equation}
    \norm{g_k^t}\leq\norm{g_j^t}=\norm{\nabla Q_j(x^t)}. \label{eqn:k_B_j_H}
\end{equation}
Recall that $\B^t = \{i_1, \ldots, \, i_{n-f}\} \setminus \H^t$. Thus, $\mnorm{\B^t} = n-f-\mnorm{\H^t}$. Also, as $\mnorm{\H} = n-f$, $\mnorm{\H\backslash\H^t} = n- f - \mnorm{\H^t}$. That is, $\mnorm{\B^t} = \mnorm{\H\backslash\H^t}$. Therefore,~\eqref{eqn:k_B_j_H} implies that
\begin{align*}
    \sum_{k \in \B^t} \norm{g_k^t} \leq \sum_{j \in \H\backslash\H^t} \norm{\nabla Q_j(x^t)}.
\end{align*}
Substituting from above in~\eqref{eqn:phi-t-2}, we obtain that
\begin{align*}
    \phi_t&\geq\gamma\mnorm{\H}\, \norm{x^t-x_{\H}}^2-2\sum_{j\in\H\backslash\H^t}\norm{x^t-x_{\H}}\, \norm{\nabla Q_j(x^t)}.
\end{align*}
Substituting from \eqref{eqn:honest-bound-everywhere}, i.e., $\norm{\nabla Q_i(x)}\leq2n\mu\epsilon+\mu\norm{x-x_{\H}}$, above we obtain that
% . With \eqref{eqn:honest-bound-everywhere}, 
\begin{align*}
    \phi_t&\geq\gamma\mnorm{\H}\, \norm{x^t-x_{\H}}^2 - 2\mnorm{\H\backslash\H^t}\, \norm{x^t-x_{\H}}\, (2n\mu\epsilon+\mu\norm{x^t-x_{\H}}) \nonumber\\
    & \geq \left(\gamma\mnorm{\H}-2\mu\mnorm{\H\backslash\H^t}\right)\norm{x^t-x_{\H}}^2 - 4n\mu\epsilon \mnorm{\H\backslash\H^t}\, \norm{x^t-x_{\H}}.
\end{align*}
As $\mnorm{\H} = n-f$ and $\mnorm{\H\backslash\H^t}\leq f$, the above implies that
\begin{align}
\begin{split}
\label{eqn:phi-t-pre-final}
    \phi_t & \geq\left(\gamma(n-f)-2\mu f\right)\norm{x^t-x_{\H}}^2-4n\mu\epsilon f\, \norm{x^t-x_{\H}} \\
        & = \left(\gamma(n-f)-2\mu f\right)\norm{x^t-x_{\H}}\, \left(\norm{x^t-x_{\H}}-\dfrac{4n\mu\epsilon f}{\gamma(n-f)-2\mu f} \right) \\
        & = n \gamma \, \left( 1 - \frac{f}{n} \left( 1 + \frac{2\mu}{\gamma}\right)\right) \norm{x^t-x_{\H}} \, \left(\norm{x^t-x_{\H}} - \frac{4 \mu f \, \epsilon}{\gamma\left( 1 - \frac{f}{n}\left(1 + \frac{2 \mu}{\gamma} \right)\right)} \right).
\end{split}
\end{align}
Recall from~\eqref{eqn:alpha} that
$$\alpha = 1-\dfrac{f}{n}\left(1+\dfrac{2\mu}{\gamma}\right). $$
Substituting from above in~\eqref{eqn:phi-t-pre-final} we obtain that
% \[\D = \frac{4\mu f}{\alpha\gamma}\]
% and 
% $$\D = \dfrac{4n\mu f}{n\gamma\left(1-\dfrac{f}{n}\left(1+\dfrac{2\mu}{\gamma}\right)\right)}=\frac{4\mu f}{\alpha\gamma}.$$
% We have
\begin{align}
    \phi_t \geq \alpha \, n \gamma \,\norm{x^t-x_{\H}}\, \left(\norm{x^t-x_{\H}}- \left( \frac{4\mu f}{\alpha\gamma} \right) \,\epsilon \right).
    \label{eqn:phi-t-final}
\end{align}
As it is assumed that $\alpha > 0$,~\eqref{eqn:phi-t-final} implies that for an arbitrary $\delta > 0$,
\begin{align*}
    \phi_t \geq \alpha \, n \gamma \, \delta \left( \left(\frac{4\mu f}{\alpha\gamma} \right)\, \epsilon + \delta \right) > 0 ~ \text{ when } \norm{x^t-x_{\H}} \geq \D \epsilon + \delta.
\end{align*}
Hence, the proof.
% $\lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \not> \D \, \epsilon$. Hence, and therefore, $\lim_{t\rightarrow\infty}\norm{x^t - x_{\H}} \leq \D \, \epsilon$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{Proof of Theorem~\ref{thm:conv-rate}}
\label{sub:proof_2}
From the update rule~\eqref{eqn:update}, and the non-expansion property of projection onto a convex set, we obtain that for all $t \geq 0$,
\begin{align}
    \norm{x^{t+1}-x_{\H}}^2 \leq \norm{x^t-x_{\H}}^2-2\eta_t\phi_t+\eta_t^2\norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2 \label{eqn:conv_exp_1}
\end{align}
where $\phi_t\triangleq\iprod{x^t-x_{\H}}{\sum_{j=1}^{n-f}g_{i_j}^t}$. From~\eqref{eqn:filtered-upperbound}, we obtain that
\begin{equation}
    \norm{\sum_{j=1}^{n-f}g_{i_j}^t}^2\leq(n-f)^2\left(2n\mu\epsilon+\mu\norm{x^t-x_{\H}}\right)^2. 
    \label{eqn:square-filtered-gradients}
\end{equation}
Substituting from~\eqref{eqn:square-filtered-gradients} and~\eqref{eqn:phi-t-final} in~\eqref{eqn:conv_exp_1} we obtain that
\begin{align*}
    \norm{x^{t+1}-x_{\H}}^2 &\leq (1-2\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+2\eta_t\alpha n \gamma\D\epsilon\norm{x^t-x_{\H}} \nonumber \\
        & + \eta_t^2\mu^2(n-f)^2 \left(\norm{x^t-x_{\H}}+2n\epsilon \right)^2 \\
        & \leq(1-2\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+2\eta_t\alpha n \gamma\D\epsilon\norm{x^t-x_{\H}} \nonumber \\
        & + \eta_t^2\mu^2n^2 \left(\norm{x^t-x_{\H}}+2n\epsilon \right)^2.
\end{align*}
As $2\D\epsilon\norm{x^t-x_{\H}}\leq\norm{x^t-x_{\H}}^2+\D^2\epsilon^2$ and $\norm{x^t - x_{\H}} \leq \Gamma$ for all $t$ (due to the projection of the estimates onto the hypercube $\W$), the above implies that
\begin{align}
    \norm{x^{t+1}-x_{\H}}^2&\leq(1-\eta_t\alpha n\gamma)\norm{x^t-x_{\H}}^2+\eta_t\alpha n\gamma\D^2\epsilon^2+\eta_t^2\mu^2n^2(\Gamma+2n\epsilon)^2. \label{eqn:before_step-size}
\end{align}
Upon substituting the step size $\eta_t=\left(\frac{2}{\alpha n\gamma}\right)\frac{1}{t+1}$ for all $t$ in~\eqref{eqn:before_step-size} we obtain that
\begin{equation*}
    \norm{x^{t+1}-x_{\H}}^2\leq\left(1-\dfrac{2}{t+1}\right)\norm{x^t-x_{\H}}^2+\dfrac{2}{t+1}\D^2\epsilon^2+\left(\dfrac{1}{t+1}\right)^2\dfrac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2.
\end{equation*}
We let
\begin{equation}
    \L = \dfrac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2.
\end{equation}
Thus, for all $t \geq 0$,
\begin{equation}
    \norm{x^{t+1}-x_{\H}}^2\leq\left(\dfrac{t-1}{t+1}\right)\norm{x^t-x_{\H}}^2+\dfrac{2}{t+1}\D^2\epsilon^2+\left(\dfrac{1}{t+1}\right)^2\L.
    \label{eqn:distance-recursive}
\end{equation}
Note that, as $\alpha < 1$ and $\mu \geq \gamma$ (under Assumptions~\ref{assum:lipschitz} and~\ref{assum:strongly-convex}), 
\begin{equation*}
    \L \geq 4\Gamma^2.
\end{equation*}
Therefore, as $x^1 \in \W$,
\begin{align}
    \norm{x^1-x_{\H}}^2 \leq \Gamma^2 \leq \frac{\L}{4} \leq \frac{\L}{4} + \D^2\epsilon^2. \label{eqn:ind_1}
\end{align}
~

Next, we reason by induction that for all $t \geq 1$,
\begin{equation}
    \norm{x^t-x_{\H}}^2 \leq \dfrac{1}{t+1}\L + \D^2\epsilon^2. \label{eqn:main_conv}
\end{equation}
The above inequality holds true for $t = 1$ as shown above in~\eqref{eqn:ind_1}. Now, suppose that~\eqref{eqn:main_conv} is true for $t = \tau$ where $\tau$ is an arbitrary integer greater than $1$, i.e., 
\begin{equation*}
    \norm{x^\tau - x_{\H}} \leq \dfrac{1}{\tau+1}\L + \D^2\epsilon^2.
\end{equation*}
We show below that~\eqref{eqn:main_conv} also holds true for $t = \tau + 1$. Substituting from above in~\eqref{eqn:distance-recursive} for $t = \tau $ we obtain that
\begin{align}
    \norm{x^{\tau+1}-x_{\H}} &\leq \left( \dfrac{\tau-1}{\tau+1}\right) \left(\dfrac{\L}{\tau+1}+ \D^2\epsilon^2 \right) + \dfrac{2}{\tau+1} \D^2 + \left(\dfrac{1}{\tau+1}\right)^2 \L \nonumber \\
    &=\dfrac{\tau}{(\tau+1)^2}\L. \label{eqn:ind_last}%+\D^2\leq\dfrac{1}{t+2}\L(f,\epsilon)+\D^2.
\end{align}
Note that for $\tau \geq 0$, $\tau (\tau + 2) \leq (\tau +1)^2$, or
\begin{equation*}
    \dfrac{\tau}{(\tau+1)^2}\leq\dfrac{1}{\tau+2}.
\end{equation*}
Therefore,~\eqref{eqn:ind_last} implies that
\begin{equation}
    \norm{x^{\tau+1}-x_{\H}}=\dfrac{\tau}{(\tau+1)^2}\L + \D^2 \epsilon^2 \leq \dfrac{1}{\tau+2} \L + \D^2\epsilon^2. \label{eqn:last}
\end{equation}
As $\L = \frac{4\mu^2}{\alpha^2\gamma^2}(\Gamma+2n\epsilon)^2 = \left(\frac{2 \mu (\Gamma + 2n\epsilon)}{\alpha \gamma} \right)^2$,~\eqref{eqn:last} proves the theorem.

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> intro-podc_new.tex <==
\section{Introduction}

The problem of distributed optimization in multi-agent systems has gained significant attention in recent years~\cite{boyd2011distributed, nedic2009distributed, duchi2011dual}. In this problem, each agent has a {\em local cost function} and, when the agents are fault-free, the goal is to design algorithms that allow the agents to collectively minimize the aggregate of their cost functions. To be precise, suppose that there are $n$ agents in the system and let $Q_i(x)$ denote the {local} cost function of agent $i$, where $x$ is a $d$-dimensional vector of real values, i.e., $x\in \R^d$. A traditional distributed optimization algorithm outputs a {\em global minimum} $x^*$ such that
\begin{align}
    x^* \in \arg \min_{x \in \R^d} ~ \sum_{i = 1}^n Q_i(x). \label{eqn:obj}
\end{align}
% The above equation specifies that $w^*$  equals an argument $w$that minimizes the specified global cost $\sum_{i = 1}^n Q_i(w)$.
As a simple example, $Q_i(x)$ may denote the cost for an agent $i$ (which may be a robot or a person) to travel to location $x$ from their current location,
and $x^*$ is a location that minimizes the total cost of meeting for all the agents. Such multi-agent optimization 
is of interest in many practical applications,
 including distributed machine learning~\cite{boyd2011distributed}, swarm robotics~\cite{raffard2004distributed}, and distributed sensing~\cite{rabbat2004distributed}.\\
 % Most of the prior work, however, assumes the agents to be fault-free, i.e.,~they cooperate and follow a prescribed algorithm. We consider a scenario wherein some of the agents may be faulty. \\

We consider the distributed optimization problem in the presence of up to $f$ Byzantine faulty agents, originally introduced by Su and Vaidya \cite{su2016fault}. The Byzantine faulty agents may behave arbitrarily~\cite{lamport1982byzantine}. In particular, the non-faulty agents
may share arbitrary incorrect and inconsistent information in order to bias the output of a distributed optimization algorithm. For example, consider an application
of multi-agent optimization in the case of distributed sensing where the agents (or {\em sensors}) observe a common {\em object} in order to collectively identify the object. However, the faulty agents may send arbitrary observations concocted to prevent the non-faulty agents from making the correct identification~\cite{chen2018resilient, chong2015observability, pajic2014robustness, su2016non}. Similarly, in the case of distributed learning, which is another application of distributed optimization, the faulty agents may send incorrect information based on {\em mislabelled} or arbitrary concocted data points to prevent the non-faulty agents from learning a {\em good} classifier~\cite{alistarh2018byzantine, bernstein2018signsgd, blanchard2017machine, cao2019distributed, charikar2017learning, chen2017distributed, gupta2019byzantine_allerton, xie2018generalized}. 

\subsection{Background: Exact Fault-Tolerance}
\label{sub:background}

In the {\em exact fault-tolerance} problem, the goal is to design a distributed algorithm that allows all the non-faulty agents to compute a minimum point of the aggregate cost of only the non-faulty agents~\cite{gupta2020fault}. Specifically, suppose that in a given
execution, set $\B$ with $\mnorm{\B} \leq f$ is the set of 
Byzantine agents, where notation $\mnorm{\cdot}$ denotes the set cardinality, and $\H = \{1, \ldots, \, n\} \setminus \B$ denotes the set of non-faulty (i.e., honest) agents. Then, a distributed optimization algorithm has exact fault-tolerance if it outputs a point $x^*_{\H}$ such that
\begin{align}
    x^*_{\H} \in \arg \min_{x \in \R^d} ~ \sum_{i \in \H} Q_i(x). \label{eqn:honest_obj}
\end{align}
% \begin{align*}
%     \arg \min_w ~ \sum_{i \in \H} \alpha_i Q_i(w).
% \end{align*}
% A distributed optimization algorithm that outputs $w^*_{\H}$ despite up to $f$ arbitrary Byzantine faulty agents is referred as {\em $f$-resilient}.
However, since the identity of the Byzantine agents is a priori unknown, in general, exact fault-tolerance is unachievable \cite{su2016fault}. Specifically, as shown in~\cite{gupta2020fault, gupta2020resilience}, exact fault-tolerance can be achieved {\em if and only if} the agents' cost functions satisfy the {\em $2f$-redundancy} property defined below. 
% In this paper, we precisely identify the condition under which the achievability of ideal fault-tolerance is guaranteed. In particular, we show that the $2f$-redundancy
% condition below is necessary and sufficient for achieving the ideal fault-tolerance goal of
% computing $x^*_{\H}$ that satisfies (\ref{eqn:honest_obj}).
% Recall that there are $n$ agents in the system, of which at most $f$ may be Byzantine faulty.\\

% unless the non-faulty cost functions $\{Q_i, ~ i \in \H\}$ have a property, named \mbox{\em $2f$-redundancy}.\\

% \noindent \fbox{\begin{minipage}{0.97\textwidth}
\begin{definition}[{\bf $2f$-redundancy}] 
\label{def:red}
% Suppose that $\H$ denotes the set of non-faulty agents. 
The agents' cost functions are said to have {\em $2f$-redundancy} property if and only if  
for every pair of subsets $S, \,\widehat{S} \subseteq \{1, \ldots, \, n\}$ with $\widehat{S} \subseteq S$, $\mnorm{S} = n-f$, and $\mnorm{\widehat{S}} \geq n-2f$,
% and $\widehat{S} \subseteq S$,
$$\arg \min_{x \in \R^d} ~ \sum_{i \in \widehat{S}}Q_i(x) = \arg \min_{x \in \R^d} ~ \sum_{i \in S} Q_i(x).$$
\end{definition}
% \end{minipage}}
% ~\\

In principle, the {$2f$-redundancy} property can be realized by design for many applications of multi-agent distributed optimization including distributed sensing and distributed learning (see~\cite{gupta2019byzantine, gupta2020fault}). However, practical realization of {$2f$-redundancy} can be difficult in the presence of {\em noise} in the real-world systems. Therefore, we propose a pragmatic generalization of exact fault-tolerance, namely {\em $(f,\epsilon)$-resilience}. 

\subsection{$(f,\epsilon)$-Resilience: A Relaxation of Exact Fault-Tolerance}
\label{sub:approx}

Intuitively, the proposed notion of {\em $(f,\epsilon)$-resilience} requires an algorithm to output {\em approximation} of a minimum point of the aggregate of the cost functions of sufficiently large subsets of non-faulty agents. We define {\em $(f, \, \epsilon)$-resilience} below, where $\epsilon \in \R_{\geq 0}$ is the measure of approximation and $\norm{\cdot}$ denotes the Euclidean norm. The Euclidean distance between a point $x$ and a non-empty set $X$ in space $\R^d$ is denoted by \dist{x}{X}, and is defined as
\begin{align}
    \dist{x}{X} = \inf_{y\in X}\norm{x-y}. \label{eqn:dist_pt_set}
\end{align}

\begin{definition}[\textbf{$(f, \, \epsilon)$-resilience}]
\label{def:approx_res}
A distributed optimization algorithm is said to be $(f, \, \epsilon)$-resilient if it outputs a point $\widehat{x} \in \R^d$ such that for every subset $S$ of non-faulty agents with $\mnorm{S} = n-f$, 
\[\dist{\widehat{x}}{\arg \min_{x \in \R^d} \sum_{i \in S}Q_i(x)} \leq \epsilon,\]
despite the presence of up to $f$ Byzantine agents.
\end{definition}

Thus, with {\em $(f, \, \epsilon)$-resilience}, the output is within distance $\epsilon$ of a minimum point of the aggregate cost function of any $n-f$ non-faulty agents. As there can be at most $f$ Byzantine faulty agents whose identity remains unknown, the following two scenarios are indistinguishable in general: (1) there are exactly $f$ Byzantine agents, and (2) there are less than $f$ Byzantine agents. Thus, estimation for the minimum point of the aggregate cost functions of $n-f$ non-faulty agents is indeed a reasonable goal~\cite{su2016fault}. 
Analogous resilience requirements have been previously studied in other contexts as well, such as robust statistics (e.g., robust mean estimation~\cite{charikar2017learning,steinhardt2017resilience}) and fault-tolerant linear state estimation~\cite{bhatia2015robust,fawzi2014secure, feng2014distributed,mishra2016secure, pajic2017attack, shoukry2017secure}. In this work, we address resilience in the context of distributed optimization.\\

In this paper, we only consider {\em deterministic} algorithms which, given a fixed set of inputs from the agents, always output the same point in $\R^d$. Thus, a deterministic $(f, \, \epsilon)$-resilient algorithm produces a unique output point in all of its executions with identical inputs from all the agents (including the faulty ones). 
% However, the output of a deterministic {$(f,\epsilon)$-resilient} algorithm with $\epsilon > 0$ may depend upon the inputs from the Byzantine agents, as long as it satisfies the condition stated in Definition~\ref{def:approx_res}. 
{\bf Note that} in the deterministic framework, exact fault-tolerance is equivalent to {$(f, \, 0)$-resilience}, i.e., a deterministic {$(f, \, 0)$-resilient} algorithm achieves exact fault-tolerance, and vice-versa.
%\footnote{Refer to Appendix~\ref{app:exact_approx} for proof.} 
Therefore, results on $(f, \, \epsilon)$-resilience for arbitrary $\epsilon \geq 0$ have a wider application compared to results applicable only to exact fault-tolerance, e.g.,~\cite{blanchard2017machine, guerraoui2018hidden, gupta2020fault, su2018finite}. \\
% To summarize, the output of a {$(f,\epsilon)$-resilient} algorithm in an execution may depend upon the behavior of Byzantine agents within the specified constraints.\\

We show that {\em $(f, \, \epsilon)$-resilience} requires a {\em weaker redundancy} condition, in comparison to $2f$-redundancy, named {\em $(2f, \, \epsilon)$-redundancy} defined in Definition \ref{def:approx_red} below. Recall that the {\em Euclidean Hausdorff distance} between two sets $X$ and $Y$ in $\R^d$, which we denote by $\dist{X}{Y}$, is defined as follows~\cite{munkres2000topology}:
\begin{equation}
    \dist{X}{Y}\triangleq\max\left\{\sup_{x\in X} \dist{x}{Y}, ~ \sup_{y\in Y}\dist{y}{X}\right\}. \label{eqn:hausdorff}
\end{equation}

\begin{definition}[\textbf{$(2f, \, \epsilon)$-redundancy}]
\label{def:approx_red}
% Given the set of non-faulty agents $\H$, the 
% Suppose that $\H$ denotes the set of non-faulty agents. 
The agents' cost functions are said to have {\em $(2f, \, \epsilon)$-redundancy} property if and only if for every pair of subsets $S, \,\widehat{S} \subseteq \{1, \ldots, \, n\}$ with
% $\widehat{S} \subseteq S \subseteq \H$, 
$\mnorm{S} = n-f$, $\mnorm{\widehat{S}} \geq n-2f$ and $\widehat{S} \subseteq S$,
% and $\widehat{S} \subseteq S$, 
\begin{equation}
    \dist{\arg\min_{x \in \R^d}\sum_{i\in S}Q_i(x)}{\arg\min_{x \in \R^d}\sum_{i\in \widehat{S}}Q_i(x)} \leq \epsilon. \label{eqn:red_dist}
    % \dist{X_{S}}{X_{\widehat{S}}}\leq\epsilon
\end{equation}
\end{definition}

It is easy to show that $2f$-redundancy (Definition~\ref{def:red}) is equivalent to $(2f, \, 0)$-redundancy (note that $\epsilon=0$ here). It is also obvious that $2f$-redundancy implies $(2f, \, \epsilon)$-redundancy for all $\epsilon \geq 0$. However, the converse need not be true. Thus, the $(2f, \, \epsilon)$-redundancy property with $\epsilon > 0$ is {\em weaker} than $2f$-redundancy. 

\input{applications}

\subsection{System architecture}
% {\bf System architecture:}

We consider {\em synchronous} systems.
Our results apply to the two architectures shown in Figure \ref{fig:sys}. In the server-based architecture, the server is assumed to be trustworthy, but up to $f$ agents may be Byzantine faulty.
% The trusted server helps solve the distributed optimization problem in coordination with the agents.
In the peer-to-peer architecture, the agents are connected by a complete network, and up to $f$ of these agents may be Byzantine faulty. Provided that $f<\frac{n}{3}$, an algorithm for the server-based architecture can be simulated in the peer-to-peer system using
the well-known {\em Byzantine broadcast} primitive~\cite{lynch1996distributed}. For simplicity of presentation, the rest of this paper considers the server-based architecture. 

\begin{figure}[htb!]
\centering
\includegraphics[width = 0.8\linewidth]{architecture.jpg}
\caption{System architecture.}
\label{fig:sys}
% \vspace{-4mm}
\end{figure}

\subsection{Summary of Our Contributions}
\label{sub:contri}
% The above property of deterministic algorithms is used later without stating it explicitly.\\

In the {\bf first part} of the paper, i.e., Section~\ref{sec:approx-fault-tolerance}, we obtain conditions on feasibility and achievability of approximate fault-tolerance of desirable accuracy. Specifically, we show that 

% which are summarized below.
% \noindent \fbox{\begin{minipage}{0.98\textwidth}
% \noindent \fbox{\begin{minipage}{0.97\linewidth}
\begin{itemize}%[nosep]
% \setlength{\itemsep}{0.3em}
    \item $(f, \epsilon)$-resilience is feasible only if $(2f, \epsilon)$-redundancy property holds true.
    \item If $(2f, \epsilon)$-redundancy property holds true then $(f, 2\epsilon)$-resilience is achievable.
\end{itemize}
% \end{minipage}}
% ~\\
% Note that the approximate fault-tolerance we can presently guarantee is depreciated by a factor of $2$ than what seems feasible according to our necessity result. 

In the {\bf second part}, i.e., Sections~\ref{sec:grad_des} and~\ref{sec:experiments}, we consider the case when agents' costs are differentiable, such as in machine learning~\cite{bottou2018optimization, yang2017byrdie}, or regression~\cite{gupta2019byzantine, su2018finite, su2016non}. We consider the distributed gradient-descent (DGD) method - an iterative distributed optimization algorithm commonly used in this particular case.

\begin{itemize}
\setlength{\itemsep}{0.3em}
    \item We propose a generic sufficient condition for convergence of the DGD method equipped with a {\em gradient-filter} (also referred as {\em robust gradient aggregation}), which is a common fault-tolerance mechanism, e.g., see~\cite{blanchard2017machine, chen2017distributed, gupta2020fault, yin2018byzantine}.
    
    \item Later, in Section~\ref{sec:grad_filters}, we utilize the above result to obtain approximate fault-tolerance properties of the following two specific gradient-filters, under $(2f, \, \epsilon)$-redundancy: (i) Comparative gradient elimination (CGE)~\cite{gupta2019byzantine}, and (ii) Coordinate-wise trimmed mean (CWTM)~\cite{su2018finite}.
    % begin{itemize}
       % \item Comparative gradient elimination (CGE) gradient-filter~\cite{gupta2019byzantine}.
        % \item Coordinate-wise trimmed mean (CWTM) gradient-filter~\cite{su2018finite}.
    % \end{itemize}
    These two gradient-filters are both easy to implement and versatile~\cite{gupta2020byzantine, gupta2020fault, su2018finite, yin2018byzantine}. 
    
    \item Finally, in Section~\ref{sec:experiments}, we present empirical comparisons between approximate fault-tolerance of the two gradient-filters by simulating a problem of distributed linear regression.
\end{itemize}
~

% \noindent \fbox{\begin{minipage}{0.97\linewidth}
{\bf Note:} As $(f, \, 0)$-resilience is equivalent to exact fault-tolerance (see Section~\ref{sub:approx}), our results on $(f, \, \epsilon)$-resilience encapsulate all the existing results applicable only to exact fault-tolerance, such as the ones in~\cite{blanchard2017machine, guerraoui2018hidden, gupta2020fault, su2018finite}.  
% \end{minipage}}
~\\

Compared to related works~\cite{karimireddy2020learning, kuwaranancharoen2020byzantine}, we present precise redundancy conditions needed for obtaining Byzantine fault-tolerance within a specified approximation error. Unlike them, our results on the impossibility and feasibility of approximate fault-tolerance are applicable to non-differentiable cost functions. Moreover, in the case when the cost functions are differentiable, we present a generic condition for convergence of the DGD method that can precisely model the approximate fault-tolerance property of a generic robust gradient-aggregation rule (a.k.a., gradient-filter). \\

A full version of this paper including omitted proofs, and additional experimental results and discussion can be found on arXiv \cite{liu2021approximate}.

% Additional comparisons with related works are presented below.

% In the first part of the paper, Section~\ref{sec:approx-fault-tolerance}, we precisely characterize the trade-off between the achievable approximate fault-tolerance guarantee and the relaxation of the {$2f$-redundancy} property. 

% , in the first part of the paper we precisely characterize a trade-off between the accuracy of fault-tolerance achievable and the {\em closeness} to $2f$-redundancy required. In the second part of the paper, we present a gradient-descent based distributed optimization algorithm that can guarantee approximate fault-tolerance in light of a {\em relaxed} {$2f$-redundancy} property.\\

% We review below other related work on approximate fault-tolerance.

% and better understand the impact of redundancy on fault-tolerance.\\

% In the first part of the paper, we formally define approximate fault-tolerance in terms of the Euclidean distance of an algorithm's output to a minimum point of the non-faulty aggregate cost function. We show that the approximation error is directly proportional to the  fault-tolerance can be achieved with 

% The {$2f$-redundancy} property implies that a minimum of the aggregate of any $n-2f$ non-faulty cost functions is also a minimum of the aggregate of all the non-faulty cost functions, and vice-versa.
% We consider Byzantine fault-tolerance problem for the most general distributed optimization framework where unlike Su and Vaidya, 2016~\cite{su2016fault}, the agents' {\em local} cost functions are {\em multivariate}, i.e.~the variable $w$ is high-dimensional. Upon presenting a necessary {\em redundancy} condition  Our proposed distributed optimization algorithm achieves 
% 
% In addition to showing the necessity of $2f$-redundancy, we present a distributed optimization algorithm that achieves ideal fault-tolerance if the non-faulty cost functions satisfy {$2f$-redundancy}, and the fraction of the faulty agents is bounded by a threshold dependent on certain
% properties of the non-faulty cost functions. Additional discussion on {$2f$-redundancy}, and characterization of fault-tolerance in the {\em absence} of {$2f$-redundancy}, can be found in our technical report~\cite{gupta2020resilience}.\\

% and~\cite{gupta2019byzantine}, respectively. The technical report~\cite{gupta2020resilience} presents a more general  alternate  \\
% To the best of our knowledge, this is the first distributed algorithm that achieves {\em ideal fault-tolerance} under $2f$-redundancy.\\
% for {\em multivariate} cost functions, i.e.,~ the vector argument $\w$ has dimension larger than 1. The related prior work applies only to {\em univariate} (or scalar) cost functions~\cite{su2016fault, sundaram2018distributed}. Further comparisons with related work are presented in Section~\ref{sec:prior}.\\

% {\bf Realizing $2f$-redundancy:} 



==> intro.tex <==
\section{Introduction}

The problem of distributed optimization in multi-agent systems has gained significant attention in recent years~\cite{boyd2011distributed, nedic2009distributed, duchi2011dual}. In this problem, each agent has a {\em local cost function} and, when the agents are fault-free, the goal is to design algorithms that allow the agents to collectively minimize the aggregate of their cost functions. To be precise, suppose that there are $n$ agents in the system and let $Q_i(x)$ denote the {local} cost function of agent $i$, where $x$ is a $d$-dimensional vector of real values, i.e., $x\in \R^d$. A traditional distributed optimization algorithm outputs a {\em global minimum} $x^*$ such that
\begin{align}
    x^* \in \arg \min_{x \in \R^d} ~ \sum_{i = 1}^n Q_i(x). \label{eqn:obj}
\end{align}
% The above equation specifies that $w^*$  equals an argument $w$that minimizes the specified global cost $\sum_{i = 1}^n Q_i(w)$.
As a simple example, $Q_i(x)$ may denote the cost for an agent $i$ (which may be a robot or a person) to travel to location $x$ from their current location,
and $x^*$ is a location that minimizes the total cost of meeting for all the agents. Such multi-agent optimization 
is of interest in many practical applications,
 including distributed machine learning~\cite{boyd2011distributed}, swarm robotics~\cite{raffard2004distributed}, and distributed sensing~\cite{rabbat2004distributed}.\\
 % Most of the prior work, however, assumes the agents to be fault-free, i.e.,~they cooperate and follow a prescribed algorithm. We consider a scenario wherein some of the agents may be faulty. \\

We consider the distributed optimization problem in the presence of up to $f$ Byzantine faulty agents, originally introduced by Su and Vaidya \cite{su2016fault}. The Byzantine faulty agents may behave arbitrarily~\cite{lamport1982byzantine}. In particular, the non-faulty agents
may share arbitrary incorrect and inconsistent information in order to bias the output of a distributed optimization algorithm. For example, consider an application
of multi-agent optimization in the case of distributed sensing where the agents (or {\em sensors}) observe a common {\em object} in order to collectively identify the object. However, the faulty agents may send arbitrary observations concocted to prevent the non-faulty agents from making the correct identification~\cite{chen2018resilient, chong2015observability, pajic2014robustness, su2016non}. Similarly, in the case of distributed learning, which is another application of distributed optimization, the faulty agents may send incorrect information based on {\em mislabelled} or arbitrary concocted data points to prevent the non-faulty agents from learning a {\em good} classifier~\cite{alistarh2018byzantine, bernstein2018signsgd, blanchard2017machine, cao2019distributed, charikar2017learning, chen2017distributed, gupta2019byzantine_allerton, xie2018generalized}. 

\subsection{Background: Exact Fault-Tolerance}
\label{sub:background}

In the {\em exact fault-tolerance} problem, the goal is to design a distributed algorithm that allows all the non-faulty agents to compute a minimum point of the aggregate cost of only the non-faulty agents~\cite{gupta2020fault}. Specifically, suppose that in a given
execution, set $\B$ with $\mnorm{\B} \leq f$ is the set of 
Byzantine agents, where notation $\mnorm{\cdot}$ denotes the set cardinality, and $\H = \{1, \ldots, \, n\} \setminus \B$ denotes the set of non-faulty (i.e., honest) agents. Then, a distributed optimization algorithm has exact fault-tolerance if it outputs a point $x^*_{\H}$ such that
\begin{align}
    x^*_{\H} \in \arg \min_{x \in \R^d} ~ \sum_{i \in \H} Q_i(x). \label{eqn:honest_obj}
\end{align}
% \begin{align*}
%     \arg \min_w ~ \sum_{i \in \H} \alpha_i Q_i(w).
% \end{align*}
% A distributed optimization algorithm that outputs $w^*_{\H}$ despite up to $f$ arbitrary Byzantine faulty agents is referred as {\em $f$-resilient}.
However, since the identity of the Byzantine agents is a priori unknown, in general, exact fault-tolerance is unachievable \cite{su2016fault}. Specifically, as shown in~\cite{gupta2020fault, gupta2020resilience}, exact fault-tolerance can be achieved {\em if and only if} the agents' cost functions satisfy the {\em $2f$-redundancy} property defined below. 
% In this paper, we precisely identify the condition under which the achievability of ideal fault-tolerance is guaranteed. In particular, we show that the $2f$-redundancy
% condition below is necessary and sufficient for achieving the ideal fault-tolerance goal of
% computing $x^*_{\H}$ that satisfies (\ref{eqn:honest_obj}).
% Recall that there are $n$ agents in the system, of which at most $f$ may be Byzantine faulty.\\

% unless the non-faulty cost functions $\{Q_i, ~ i \in \H\}$ have a property, named \mbox{\em $2f$-redundancy}.\\

% \noindent \fbox{\begin{minipage}{0.97\textwidth}
\begin{definition}[{\bf $2f$-redundancy}] 
\label{def:red}
% Suppose that $\H$ denotes the set of non-faulty agents. 
The agents' cost functions are said to have {\em $2f$-redundancy} property if and only if  
for every pair of subsets $S, \,\widehat{S} \subseteq \{1, \ldots, \, n\}$ with $\mnorm{S} = n-f$, $\mnorm{\widehat{S}} \geq n-2f$ and $\widehat{S} \subseteq S$,
% and $\widehat{S} \subseteq S$,
$$\arg \min_{x \in \R^d} ~ \sum_{i \in \widehat{S}}Q_i(x) = \arg \min_{x \in \R^d} ~ \sum_{i \in S} Q_i(x).$$
\end{definition}
% \end{minipage}}
% ~\\

In principle, the {$2f$-redundancy} property can be realized by design for many applications of multi-agent distributed optimization including distributed sensing and distributed learning (see~\cite{gupta2019byzantine, gupta2020fault}). However, practical realization of {$2f$-redundancy} can be difficult in the presence of {\em noise} in the real-world systems. Therefore, we propose a pragmatic generalization of exact fault-tolerance, namely {\em $(f,\epsilon)$-resilience}. 

\subsection{$(f,\epsilon)$-Resilience: A Relaxation of Exact Fault-Tolerance}
\label{sub:approx}

Intuitively, the proposed notion of {\em $(f,\epsilon)$-resilience} requires an algorithm to output {\em approximation} of a minimum point of the aggregate of the cost functions of sufficiently large subsets of non-faulty agents. We define {\em $(f, \, \epsilon)$-resilience} below, where $\epsilon \in \R_{\geq 0}$ is the measure of approximation and $\norm{\cdot}$ denotes the Euclidean norm. The Euclidean distance between a point $x$ and a non-empty set $X$ in space $\R^d$ is denoted by \dist{x}{X}, and is defined as
\begin{align}
    \dist{x}{X} = \inf_{y\in X}\norm{x-y}. \label{eqn:dist_pt_set}
\end{align}

\begin{definition}[\textbf{$(f, \, \epsilon)$-resilience}]
\label{def:approx_res}
A distributed optimization algorithm is said to be $(f, \, \epsilon)$-resilient if it outputs a point $\widehat{x} \in \R^d$ such that for every subset $S$ of non-faulty agents with $\mnorm{S} = n-f$, 
\[\dist{\widehat{x}}{\arg \min_{x \in \R^d} \sum_{i \in S}Q_i(x)} \leq \epsilon,\]
despite the presence of up to $f$ Byzantine agents.
\end{definition}

Thus, with {\em $(f, \, \epsilon)$-resilience}, the output is within distance $\epsilon$ of a minimum point of the aggregate cost function of any $n-f$ non-faulty agents. As there can be at most $f$ Byzantine faulty agents whose identity remains unknown, the following two scenarios are indistinguishable in general: (1) there are exactly $f$ Byzantine agents, and (2) there are less than $f$ Byzantine agents. Thus, estimation for the minimum point of the aggregate cost functions of $n-f$ non-faulty agents is indeed a reasonable goal~\cite{su2016fault}. 
Analogous resilience requirements have been previously studied in other contexts as well, such as robust statistics (e.g., robust mean estimation~\cite{charikar2017learning,steinhardt2017resilience}) and fault-tolerant linear state estimation~\cite{bhatia2015robust,fawzi2014secure, feng2014distributed,mishra2016secure, pajic2017attack, shoukry2017secure}. In this work, we address resilience in the context of distributed optimization.\\

In this paper, we only consider {\em deterministic} algorithms which, given a fixed set of inputs from the agents, always output the same point in $\R^d$. Thus, a deterministic $(f, \, \epsilon)$-resilient algorithm produces a unique output point in all of its executions with identical inputs from all the agents (including the faulty ones). 
% However, the output of a deterministic {$(f,\epsilon)$-resilient} algorithm with $\epsilon > 0$ may depend upon the inputs from the Byzantine agents, as long as it satisfies the condition stated in Definition~\ref{def:approx_res}. 
{\bf Note that} in the deterministic framework, exact fault-tolerance is equivalent to {$(f, \, 0)$-resilience}, i.e., a deterministic {$(f, \, 0)$-resilient} algorithm achieves exact fault-tolerance, and vice-versa.\footnote{Refer to Appendix~\ref{app:exact_approx} for proof.} Therefore, results on $(f, \, \epsilon)$-resilience for arbitrary $\epsilon \geq 0$ have a wider application compared to results applicable only to exact fault-tolerance, e.g.,~\cite{blanchard2017machine, guerraoui2018hidden, gupta2020fault, su2018finite}. \\
% To summarize, the output of a {$(f,\epsilon)$-resilient} algorithm in an execution may depend upon the behavior of Byzantine agents within the specified constraints.\\

We show that {\em $(f, \, \epsilon)$-resilience} requires a {\em weaker redundancy} condition, in comparison to $2f$-redundancy, named {\em $(2f, \, \epsilon)$-redundancy} defined in Definition \ref{def:approx_red} below. Recall that the {\em Euclidean Hausdorff distance} between two sets $X$ and $Y$ in $\R^d$, which we denote by $\dist{X}{Y}$, is defined as follows~\cite{munkres2000topology}:
\begin{equation}
    \dist{X}{Y}\triangleq\max\left\{\sup_{x\in X} \dist{x}{Y}, ~ \sup_{y\in Y}\dist{y}{X}\right\}. \label{eqn:hausdorff}
\end{equation}

\begin{definition}[\textbf{$(2f, \, \epsilon)$-redundancy}]
\label{def:approx_red}
% Given the set of non-faulty agents $\H$, the 
% Suppose that $\H$ denotes the set of non-faulty agents. 
The agents' cost functions are said to have {\em $(2f, \, \epsilon)$-redundancy} property if and only if for every pair of subsets $S, \,\widehat{S} \subseteq \{1, \ldots, \, n\}$ with
% $\widehat{S} \subseteq S \subseteq \H$, 
$\mnorm{S} = n-f$, $\mnorm{\widehat{S}} \geq n-2f$ and $\widehat{S} \subseteq S$,
% and $\widehat{S} \subseteq S$, 
\begin{equation}
    \dist{\arg\min_{x \in \R^d}\sum_{i\in S}Q_i(x)}{\arg\min_{x \in \R^d}\sum_{i\in \widehat{S}}Q_i(x)} \leq \epsilon. \label{eqn:red_dist}
    % \dist{X_{S}}{X_{\widehat{S}}}\leq\epsilon
\end{equation}
\end{definition}

It is easy to show that $2f$-redundancy (Definition~\ref{def:red}) is equivalent to $(2f, \, 0)$-redundancy (note that $\epsilon=0$ here). It is also obvious that $2f$-redundancy implies $(2f, \, \epsilon)$-redundancy for all $\epsilon \geq 0$. However, the converse need not be true. Thus, the $(2f, \, \epsilon)$-redundancy property with $\epsilon > 0$ is {\em weaker} than $2f$-redundancy. 

\input{applications}

\subsection{System architecture}
% {\bf System architecture:}

We consider {\em synchronous} systems.
Our results apply to the two architectures shown in Figure \ref{fig:sys}. In the server-based architecture, the server is assumed to be trustworthy, but up to $f$ agents may be Byzantine faulty.
% The trusted server helps solve the distributed optimization problem in coordination with the agents.
In the peer-to-peer architecture, the agents are connected by a complete network, and up to $f$ of these agents may be Byzantine faulty. Provided that $f<\frac{n}{3}$, an algorithm for the server-based architecture can be simulated in the peer-to-peer system using
the well-known {\em Byzantine broadcast} primitive~\cite{lynch1996distributed}. For simplicity of presentation, the rest of this paper considers the server-based architecture. 

\begin{figure}[htb!]
\centering
\includegraphics[width = 0.45\textwidth]{architecture.jpg}
\caption{System architecture.}
\label{fig:sys}
% \vspace{-4mm}
\end{figure}

\subsection{Summary of Our Contributions}
\label{sub:contri}
% The above property of deterministic algorithms is used later without stating it explicitly.\\

In the {\bf first part} of the paper, i.e., Section~\ref{sec:approx-fault-tolerance}, we obtain the {\em first-ever formal guarantees} for obtaining approximate fault-tolerance with a given approximation error. Specifically, we show that -\\

% which are summarized below.
% \noindent \fbox{\begin{minipage}{0.98\textwidth}
\noindent \fbox{\begin{minipage}{0.97\linewidth}
\begin{itemize}
\setlength{\itemsep}{0.3em}
    \item $(f, \, \epsilon)$-resilience is feasible only if $(2f, \, \epsilon)$-redundancy property holds true.
    \item If $(2f, \, \epsilon)$-redundancy property holds true then $(f, \, 2\epsilon)$-resilience is achievable.
\end{itemize}
\end{minipage}}
~\\
% Note that the approximate fault-tolerance we can presently guarantee is depreciated by a factor of $2$ than what seems feasible according to our necessity result. 

In the {\bf second part}, i.e., Sections~\ref{sec:grad_des} and~\ref{sec:experiments}, we consider the case when agents' costs are differentiable, such as in machine learning~\cite{bottou2018optimization, yang2017byrdie}, or regression~\cite{gupta2019byzantine, su2018finite, su2016non}. We consider the distributed gradient-descent (DGD) method - an iterative distributed optimization algorithm commonly used in this particular case.

\begin{itemize}
\setlength{\itemsep}{0.3em}
    \item We propose a generic sufficient condition for convergence of the DGD method equipped with a {\em gradient-filter} (also referred as {\em robust gradient aggregation}), which is a common fault-tolerance mechanism, e.g., see~\cite{blanchard2017machine, chen2017distributed, gupta2020fault, yin2018byzantine}.
    
    \item Later, in Section~\ref{sec:grad_filters}, we utilize the above result to obtain approximate fault-tolerance properties of the following two specific gradient-filters, under $(2f, \, \epsilon)$-redundancy: (i) Comparative gradient elimination (CGE) gradient-filter~\cite{gupta2019byzantine}, and (ii) Coordinate-wise trimmed mean (CWTM) gradient-filter~\cite{su2018finite}.
    % begin{itemize}
       % \item Comparative gradient elimination (CGE) gradient-filter~\cite{gupta2019byzantine}.
        % \item Coordinate-wise trimmed mean (CWTM) gradient-filter~\cite{su2018finite}.
    % \end{itemize}
    These two gradient-filters are easy to implement, and have a wide range of applicability~\cite{gupta2020byzantine, gupta2020fault, su2018finite, yin2018byzantine}. 
    
    \item Finally, in Section~\ref{sec:experiments}, we present empirical comparisons between approximate fault-tolerance of the two gradient-filters by simulating a special distributed optimization problem of distributed linear regression.
\end{itemize}
~

\noindent \fbox{\begin{minipage}{0.97\linewidth}
As $(f, \, 0)$-resilience is equivalent to exact fault-tolerance (see Section~\ref{sub:approx}), our results on $(f, \, \epsilon)$-resilience encapsulate all the existing results applicable only to exact fault-tolerance, such as the ones in~\cite{blanchard2017machine, guerraoui2018hidden, gupta2020fault, su2018finite}.  
\end{minipage}}
~\\

Compared to related works~\cite{karimireddy2020learning, kuwaranancharoen2020byzantine}, we present precise redundancy conditions needed for obtaining Byzantine fault-tolerance within a specified approximation error. Unlike them, our results on the impossibility and feasibility of approximate fault-tolerance are applicable to non-differentiable cost functions. Moreover, in the case when the cost functions are differentiable, we present a generic convergence result for the DGD method that can precisely model the approximate fault-tolerance property of any robust gradient-aggregation rule (a.k.a., gradient-filter). \\

Additional comparisons with other related works are presented below.

% In the first part of the paper, Section~\ref{sec:approx-fault-tolerance}, we precisely characterize the trade-off between the achievable approximate fault-tolerance guarantee and the relaxation of the {$2f$-redundancy} property. 

% , in the first part of the paper we precisely characterize a trade-off between the accuracy of fault-tolerance achievable and the {\em closeness} to $2f$-redundancy required. In the second part of the paper, we present a gradient-descent based distributed optimization algorithm that can guarantee approximate fault-tolerance in light of a {\em relaxed} {$2f$-redundancy} property.\\

% We review below other related work on approximate fault-tolerance.

% and better understand the impact of redundancy on fault-tolerance.\\

% In the first part of the paper, we formally define approximate fault-tolerance in terms of the Euclidean distance of an algorithm's output to a minimum point of the non-faulty aggregate cost function. We show that the approximation error is directly proportional to the  fault-tolerance can be achieved with 

% The {$2f$-redundancy} property implies that a minimum of the aggregate of any $n-2f$ non-faulty cost functions is also a minimum of the aggregate of all the non-faulty cost functions, and vice-versa.
% We consider Byzantine fault-tolerance problem for the most general distributed optimization framework where unlike Su and Vaidya, 2016~\cite{su2016fault}, the agents' {\em local} cost functions are {\em multivariate}, i.e.~the variable $w$ is high-dimensional. Upon presenting a necessary {\em redundancy} condition  Our proposed distributed optimization algorithm achieves 
% 
% In addition to showing the necessity of $2f$-redundancy, we present a distributed optimization algorithm that achieves ideal fault-tolerance if the non-faulty cost functions satisfy {$2f$-redundancy}, and the fraction of the faulty agents is bounded by a threshold dependent on certain
% properties of the non-faulty cost functions. Additional discussion on {$2f$-redundancy}, and characterization of fault-tolerance in the {\em absence} of {$2f$-redundancy}, can be found in our technical report~\cite{gupta2020resilience}.\\

% and~\cite{gupta2019byzantine}, respectively. The technical report~\cite{gupta2020resilience} presents a more general  alternate  \\
% To the best of our knowledge, this is the first distributed algorithm that achieves {\em ideal fault-tolerance} under $2f$-redundancy.\\
% for {\em multivariate} cost functions, i.e.,~ the vector argument $\w$ has dimension larger than 1. The related prior work applies only to {\em univariate} (or scalar) cost functions~\cite{su2016fault, sundaram2018distributed}. Further comparisons with related work are presented in Section~\ref{sec:prior}.\\

% {\bf Realizing $2f$-redundancy:} 



==> necessary_Niru.tex <==
\section{\color{red}{Lower Bound (Niru)}}

We assume $(2t, \, \epsilon)$-redundancy. Suppose that $|S| = n-2t$, and $x_{S} \in \arg \min \sum_{i \in S}Q_i(x)$. Let $S_1 \subset \{1, \ldots, \, n\} \setminus S$ with $|S_1| = t$ and let $S_2$ represents the set of remaining $t$ agents $\{1, \ldots, \, n\} \setminus S \setminus S_1$. Suppose that
\[x_1 \in \arg \min \sum_{i \in S \cup S_1} Q_i(x)\]
is $\epsilon$ far from $x_S$, as shown in the figure below. Suppose that 
\[x_2 \in \arg \min \sum_{i \in S \cup S_2} Q_i(x) \]
is also $\epsilon$ far from $x_S$, but on the opposite end as shown in the figure below.\\

\begin{center}
    \begin{tikzpicture}
        \node[dot] (x2) at (-4,0) {};
        \node[dot] (xs) at (0,0) {};
        \node[dot] (x1) at (4,0) {};
        \node at (-4,.35) {$x_2$};
        \node at (0,.35) {$x_S$};
        \node at (4,.35) {$x_1$};
        \draw (x1) -- (x0)
              (x0) -- (x2);
        
        \node at (-2,.35) {\footnotesize $\longleftarrow\epsilon\longrightarrow$};
        \node at (2,.35) {\footnotesize $\longleftarrow\epsilon\longrightarrow$};
        % \node at (-.7,-.3) {\textcolor{blue}{\footnotesize $\sigma$}};
        % \node at (-2.7,-.3) {\textcolor{blue}{\footnotesize $\sigma$}};
    \end{tikzpicture}
\end{center}

It is obvious from the figure above that $(t, \, \epsilon - \delta)$-resilience is impossible for any $\delta > 0$. \\

Next, we consider the fact that a deterministic algorithm cannot output a set, but rather a single point, to potentially improve the lower bound from $(t, \, \epsilon)$-resilience to $(t, \, 2\epsilon)$-resilience.

==> new-necessity.tex <==
\subsection{New necessity proof}

For necessity, we also need the following assumption.

\begin{assumption}
    We assume that each non-faulty cost function $Q_i(x)$ is convex.
    \label{assum:convex}
\end{assumption}

We derive a lemma that will be used later following this assumption:

\begin{lemma}
    \label{lemma:convex}
    Suppose Assumptions~\ref{asp:exists} and~\ref{assum:convex} hold. For any sets of agent $S$ and $\widehat{S}$ with $\widehat{S}\subsetneq S$, it cannot be that 
    \begin{align}
        \arg\min_x\sum_{i\in\widehat{S}}Q_i(x) \subsetneq \arg\min_x\sum_{i\in{S}}Q_i(x),
    \end{align}
    i.e., the minimum set of the aggregate cost function of agents in $\widehat{S}$ cannot be a strict subset of the minimum set of the aggregate cost function of agents in $S$.
\end{lemma}

\begin{proof}
    The proof is by contradiction. Suppose for some sets $S$ and $\widehat{S}$ with $\widehat{S}\subsetneq S$, we have
    \begin{align}\label{eqn:lemma-convex}
        \arg\min_x\sum_{i\in\widehat{S}}Q_i(x) \subsetneq \arg\min_x\sum_{i\in{S}}Q_i(x).
    \end{align}

    By Assumption~\ref{assum:convex}, cost functions $Q_i(x)$'s are convex. It follows that for any non-empty set $T$ of agents, the function $\sum_{i\in T}Q_i(x)$ is also convex. 
    
    By \eqref{eqn:lemma-convex}, for any point ${x_1}\in\arg\min_x\sum_{i\in\widehat{S}}Q_i(x)$, we also have $x_1\in\arg\min_x\sum_{i\in{S}}Q_i(x)$. On the other hand, there must exist at least one point $x_2$, such that $x_2\in\arg\min_x\sum_{i\in S}Q_i(x)$, but $x_2\notin\arg\min_x\sum_{i\in\widehat{S}}Q_i(x)$. Also, by Assumption~\ref{asp:exists}, since $\arg\min_x\sum_{i\in S}Q_i(x)$ is a closed set, $(x_1+x_2)/2\in\arg\min_x\sum_{i\in S}Q_i(x)$ as well.
    Therefore, by convexity, for $x_1$ and $x_2$, we have
    \begin{align}
        &\sum_{i\in S}Q_i(x_1)  = \sum_{i\in S}Q_i(x_2) = \sum_{i\in S}Q_i\left(\frac{x_1+x_2}{2}\right)\triangleq a,
        \label{eqn:equal-minimum-at-s} \\
        &\sum_{i\in\widehat{S}}Q_i(x_1) < \sum_{i\in\widehat{S}}Q_i(x_2).
        \label{eqn:unequal-minimum-at-shat}
    \end{align}
    Again by convexity, we also have 
    \begin{align}
        \sum_{i\in\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right)\leq \frac{\sum_{i\in\widehat{S}}Q_i(x_1)+\sum_{i\in\widehat{S}}Q_i(x_2)}{2},
    \end{align}
    % where the equation is achieved when $\sum_{i\in\widehat{S}}Q_i(x_1)=\sum_{i\in\widehat{S}}Q_i(x_2)=\sum_{i\in\widehat{S}}Q_i(x_1+x_2)$.
    % Combining \eqref{eqn:unequal-minimum-at-shat} and above, we have
    There are two cases from above: either (i)
    \begin{align}
        \sum_{i\in\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right)<\frac{\sum_{i\in\widehat{S}}Q_i(x_1)+\sum_{i\in\widehat{S}}Q_i(x_2)}{2},
        \label{eqn:convex-minimum-at-shat}
    \end{align}
    or (ii)
    \begin{align}
        \sum_{i\in\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right)=\frac{\sum_{i\in\widehat{S}}Q_i(x_1)+\sum_{i\in\widehat{S}}Q_i(x_2)}{2},
        \label{eqn:convex-minimum-at-shat-case-2}
    \end{align}
    
    For Case (i), consider the term $\sum_{i\in S\backslash\widehat{S}}Q_i\left({(x_1+x_2)}/{2}\right)$. Note that for any $x$, 
    \begin{align}
        \sum_{i\in S\backslash\widehat{S}}Q_i(x) = \sum_{i\in S}Q_i(x) - \sum_{i\in\widehat{S}}Q_i(x).
    \end{align}
    Therefore, 
    \begin{align}
        &\sum_{i\in S\backslash\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right) - \frac{\sum_{i\in S\backslash\widehat{S}}Q_i(x_1) + \sum_{i\in S\backslash\widehat{S}}Q_i(x_2)}{2} \nonumber \\
        =&\left(\sum_{i\in S}Q_i\left(\frac{x_1+x_2}{2}\right) - \sum_{i\in\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right)\right) - \frac{\sum_{i\in S}Q_i(x_1) - \sum_{i\in\widehat{S}}Q_i(x_1) + \sum_{i\in S}Q_i(x_2) - \sum_{i\in\widehat{x}}Q_i(x_2)}{2} \nonumber \\
        =&\left(\sum_{i\in S}Q_i\left(\frac{x_1+x_2}{2}\right) - \frac{\sum_{i\in S}Q_i(x_1) + \sum_{i\in S}Q_i(x_2)}{2}\right) - \left(\sum_{i\in\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right) - \frac{\sum_{i\in\widehat{S}}Q_i(x_1) + \sum_{i\in\widehat{S}}Q_i(x_2)}{2}\right) \nonumber \\
        =&\left( a - \frac{a+a}{2}\right) - \left(\sum_{i\in\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right) - \frac{\sum_{i\in\widehat{S}}Q_i(x_1) + \sum_{i\in\widehat{S}}Q_i(x_2)}{2}\right) \tag{by \eqref{eqn:equal-minimum-at-s}} \\
        =& - \left(\sum_{i\in\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right) - \frac{\sum_{i\in\widehat{S}}Q_i(x_1) + \sum_{i\in\widehat{S}}Q_i(x_2)}{2}\right) > 0 \tag{by \eqref{eqn:convex-minimum-at-shat}}
    \end{align}
    In other words,
    \begin{align}
        \sum_{i\in S\backslash\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right) > \frac{\sum_{i\in S\backslash\widehat{S}}Q_i(x_1) + \sum_{i\in S\backslash\widehat{S}}Q_i(x_2)}{2}.
        \label{eqn:lemma-2-contra-1}
    \end{align}
    However, since $\sum_{i\in S\backslash\widehat{S}}Q_i(x)$ is convex, for any points $x_1$ and $x_2$ we should have
    \begin{align}
        \sum_{i\in S\backslash\widehat{S}}Q_i\left(\frac{x_1+x_2}{2}\right) \leq \frac{\sum_{i\in S\backslash\widehat{S}}Q_i(x_1) + \sum_{i\in S\backslash\widehat{S}}Q_i(x_2)}{2}.
        \label{eqn:lemma-2-contra-2}
    \end{align}
    We have \eqref{eqn:lemma-2-contra-1} contradicts \eqref{eqn:lemma-2-contra-2}. 
    
    For Case (ii), Hence the proof.
\end{proof}

Recall that in a server-based architecture for distributed optimization, each agent $i$ has a local cost function $Q_i(x)$ as input. Among the $n$ agents, there are up to $f$ Byzantine agents that may behave arbitrarily. Communication occurs between the server and each agent. Suppose in an execution, from the server's perspective, each agent $i$ behaves as if its local cost function is $P_i(x)$. For a non-faulty agent $i$, $P_i(x) = Q_i(x)$. For a Byzantine agent $j$, $P_j(x)$ can be arbitrary. The server however does not know the identity of Byzantine agents a priori.

Let us first consider the following lemma:

\begin{lemma}
    \label{lemma:necessity}
    Suppose that Assumption~\ref{asp:exists} holds. There exists a deterministic $(f,\epsilon)$-resilient algorithm where $\epsilon>0$, only if there exists a point $\widehat{x}$, such that for each subset $S\subseteq[n]$ of agents with $\mnorm{S}\geq n-f$,
    \begin{align}
        \dist{\widehat{x}}{\arg\min_x\sum_{i\in S}Q_i(x)}\leq \epsilon.        
    \end{align}
\end{lemma}
\begin{proof}
    Suppose there is a deterministic $(f,\epsilon)$-resilient algorithm $\Pi$. Suppose in an execution, there is no Byzantine agent. Therefore, $P_i(x) = Q_i(x)$ for all $i$. However, from the server's perspective, since the number and identity of faulty agents are unknown, the following two scenarios are indistinguishable:
    \begin{enumerate}[label=(\roman*)]
        \item The set of agents $S_1=\{1,...,n-f\}$ are non-faulty, and 
        \item The set of agents $S_2=\{2,...,n-f+1\}$ are non-faulty.
    \end{enumerate}
    Therefore, the output of the algorithm $\widehat{x}$ should satisfy the following:
    \begin{align}
        &\dist{\widehat{x}}{\arg\min_x\sum_{i\in S_1}Q_i(x)}\leq \epsilon, \textrm{ for Scenario (i), and} \\
        &\dist{\widehat{x}}{\arg\min_x\sum_{i\in S_2}Q_i(x)}\leq \epsilon, \textrm{ for Scenario (ii)}.
    \end{align}
    With a similar argument but for other choices of sets $S_1$ and $S_2$, for all $S\subset[n]$ with $\mnorm{S}\geq n-f$,
    \begin{align}
        \dist{\widehat{x}}{\arg\min_x\sum_{i\in S}Q_i(x)}\leq \epsilon.
        \label{eqn:redundancy}
    \end{align}
\end{proof}

Inspired by the result in Lemma~\ref{lemma:necessity}, we consider a group of algorithms with the following constraints: Suppose each agent $i$ behaves as if its cost function is $P_i(x)$. The algorithms generate an output in the following way: Suppose for each set of $n-f$ agents $S$ and its subset $\widehat{S}\subseteq{S}$ with $\mnorm{\widehat{S}}= n-2f$, we define 
\begin{align}
    r_{S\widehat{S}}=\dist{\arg\min_x\sum_{i\in{S}}P_i(x)}{\arg\min_x\sum_{i\in\widehat{S}}P_i(x)}.
    \label{eqn:def-rsshat}
\end{align}
Furthermore, we define
\begin{align}
    r_{S} = \max_{\widehat{S}\subseteq{S},\mnorm{\widehat{S}}= n-2f}r_{S\widehat{S}}.
    \label{eqn:def-rs}
\end{align}
The algorithms generate an output by finding the set $S$ that minimizes $r_S$, and output a point in $\arg\min_x\sum_{i\in S}P_i(x)$.

Note that for a non-faulty agent $i$, $P_i(x)=Q_i(x)$. For a Byzantine agent $j$, $P_j(x)$ may be arbitrary. There are up to $f$ Byzantine agents.

\begin{theorem}
    Suppose that Assumptions~\ref{asp:exists} and~\ref{assum:convex} hold.
    % and $\arg\min_x\sum_{i\in T}Q_i(x)$ is a singleton for all $T\subseteq[n]$ with $\mnorm{T}\geq n-2f$. 
    There exists a deterministic $(f,\epsilon)$-resilient algorithm with the above constraints where $\epsilon>0$, only if the agents' cost functions satisfy $(2f,\epsilon)$-redundancy.
\end{theorem}
\begin{proof}
    This proof is by contradiction. Suppose there is a deterministic $(f,\epsilon)$-resilient algorithm with the above constraints exists, and $(2f,\epsilon)$-redundancy is not satisfied. That is, there exists a set $S$ and its subset $\widehat{S}_0$ with $\mnorm{S}=n-f$ and $\mnorm{\widehat{S}_0}= n-2f$, such that there exists some $\delta>0$,
    \begin{align}
        \dist{\arg\min_x\sum_{i\in S}Q_i(x)}{\arg\min_x\sum_{i\in\widehat{S}_0}Q_i(x)}=\epsilon+\delta.
        \label{eqn:contradict-assumption}
    \end{align}
    But the algorithm $\Pi$ is $(f,\epsilon)$-resilient. 
    By \eqref{eqn:contradict-assumption}, $r_S\geq r_{S\widehat{S}}=\epsilon+\delta>\epsilon$. 
    % Since we assume that $\arg\min_x\sum_{i\in T}Q_i(x)$ is a singleton, there always exist a point $\widehat{x}$ such that $\dist{\widehat{x}}{\arg\min_x\sum_{i\in S}Q_i(x)}=\epsilon$, and $\dist{\widehat{x}}{\arg\min_x\sum_{i\in \widehat{S}}Q_i(x)}>\epsilon$.
    
    %, meaning its output $\widehat{x}$ satisfies \eqref{eqn:redundancy} for $S_0$. 
    Let us denote $F = [n]\backslash S$. Suppose in an execution, $F$ is the set of Byzantine agents. For any point $\widehat{x}$, note that the faulty agents can choose to behave as if it has a cost function, such that for any set of agent $T\subseteq[n]$ where $T\cap F\neq\varnothing$, $\arg\min_x\sum_{i\in T}Q_i(x) =\widehat{x}$.\footnote{To achieve such a result, consider a function that values sufficiently small at $\widehat{x}$ and sufficiently large at anywhere else.} 
    
    Suppose the agents in $F$ behave in a way such that for all $i\in F$, for all $T$ with $\mnorm{T}\geq n-2f$ and $i\in T$, the point $\widehat{x}$ described above satisfies the following: (i) for all subset $\widehat{S}_k\subset S$ with size $n-2f$, 
    \begin{align}
        \dist{\widehat{x}}{\arg\min_x\sum_{i\in\widehat{S}_k}Q_i(x)}\geq\epsilon,
    \end{align}
    (ii) for at least one such set $\widehat{S}_j\subset S$ with size $n-2f$, 
    \begin{align}
        \dist{\widehat{x}}{\arg\min_x\sum_{i\in\widehat{S}_j}Q_i(x)}=\epsilon,
    \end{align}
    and (iii) for the set $S$,
    \begin{align}
        \dist{\widehat{x}}{\arg\min_x\sum_{i\in S}Q_i(x)}>\epsilon.
        \label{eqn:necessity-contradiction}
    \end{align}
    With Assumption~\ref{asp:exists}, we know that $\arg\min_x\sum_{i\in\widehat{S}_k}Q_i(x)$ for every $\widehat{S}_k$ is non-empty and closed.
    With Assumptions~\ref{asp:exists} and~\ref{assum:convex}, by Lemma~\ref{lemma:convex}, such an $\widehat{x}$ satisfying (i), (ii), and (iii) above always exists.
    % it is on the surface of a hypersphere centered at $\arg\min_x\sum_{i\in\widehat{S}_j}Q_i(x)$, and is not inside any hypersphere centered at $\arg\min_x\sum_{i\in\widehat{S}_k}Q_i(x)$ for all $k$ or centered at $\arg\min_x\sum_{i\in S}Q_i(x)$. \
    
    Note that, for every other set $T\neq S$ with $\mnorm{T}=n-f$ that is a superset of any $\widehat{S}_j$, $T\cap F\neq\varnothing$. Therefore, $\arg\min_x\sum_{i\in T}Q_i(x) = \widehat{x}$. By \eqref{eqn:def-rsshat}, for any subset $\widehat{T}\subset T$ with $\mnorm{\widehat{T}}=n-2f$, if $\widehat{T}=\widehat{S}_j$ for some $j$, $r_{T\widehat{S}_j}\geq \epsilon$; otherwise $\arg\min_x\sum_{i\in\widehat{T}}Q_i(x) = \widehat{x}$ and $r_{T\widehat{T}}=0$. Therefore, by \eqref{eqn:def-rs}, $r_T\geq\epsilon$. And only when $T=\widehat{S}_j\cap F$, we have $r_{\widehat{S}_j\cap F}=\epsilon$. 
    
    For an algorithm $\Pi$ with the constraints described above, it will output the point $\arg\min_x\sum_{i\in\widehat{S}_j\cup F}Q_i(x)$, i.e., the point $\widehat{x}$. However, by \eqref{eqn:necessity-contradiction}, for the only set $S$ of non-faulty agents of size $n-f$, 
    \begin{align*}
        \dist{\widehat{x}}{\arg\min_x\sum_{i\in S}Q_i(x)}>\epsilon.
    \end{align*}
    Thus, the algorithm is not $(f,\epsilon)$-resilient. Contradiction.
\end{proof}

==> new-redundancy.tex <==
\section{New redundancy condition}

Consider the following definitions.

\begin{definition}[$n$-function group]
    An $n$-function group is a multiset of size $n$, where each element of the multiset is a function defined on the same area $\W$.
\end{definition}

\begin{definition}[Distance between function groups]
    The distance between two $n$-function groups $e_1$ and $e_2$ is defined as 
    \begin{align}
        \dist{e_1}{e_2}= n - \mnorm{e_1\cap e_2}.
    \end{align}
\end{definition}

\begin{definition}
    A group of $n$ cost functions is said to be $2f$-redundant, if it is one entry in the following list, where the list satisfies the following conditions:
    \begin{enumerate}
        \item Each entry in the list is a $n$-function group,
        \item For any $n$-function group $e^*$, suppose all entries in the list that are within $f$ distance to $e^*$ constitute a set $E$. Then for each item in $E$, 
    \end{enumerate}
\end{definition}

==> nitin.tex <==


\section{+++++++++Proof added by Nitin +++++++++++}

For a set of agents $S$, let us define $$\mu(S)=\arg\min_x
\sum_{i\in S}f_i(x)$$. 

\newcommand{\hatt}{\widehat{T}}
\newcommand{\hats}{\widehat{S}}

Assume that the function argument is a scalar real.

Suppose that there exist sets $T$ and $\hatt$ such that $|T|\geq n-f$,
$|\hatt|\geq n-2f$, $\hatt\subset T$ and $d(\mu(T),\mu(\hatt))>\epsilon$. \\

Now we will show that 
there exist sets $S$ and $\hats$ such that $|S|<n$,
$|\hats|<|S|$, $\hats\subset S$, and $d(\mu(S),\mu(\hats))>\epsilon$.\\

Without loss of generality, suppose that $d(\mu(T) > \mu(\hatt))$. \\

\paragraph{Construct set $\hats$:} If $|T|<n$, then define $S=T$ $\hats=\hatt$.
Else we will choose $\hats$ to be a suitable subset of $\hatt$ and $\hats$ to be a suitable subset of $\hatt$.

COMMENT: For now, let us assume that the functions are differentiable and convex.

Now assume that $|T|=n$. We consider two cases: (A) $|\hatt|=n-2$ and (B) $\hatt=n-1$.

\subsection*{Case (A) $|\hatt|=n-2$}




In particular, define set $P\subset \hatt$ such that every function in $P(\hatt)$ has a negative gradient
at $\mu(\hatt)$.
% If the functions are not differentiable, then choose $P$ to contain those functions for which all the subgradients at $\mu(\hatt)$ are negative.


\begin{itemize}
    \item $P=\emptyset$: In this case, each function in $\hatt$ is minimized at $\mu(\hatt)$, and we can choose $\hats$ to be any size $(n-2f)$ subset of $\hatt$.
    \item $P\neq\emptyset$: In this case, remove
\end{itemize}



==> prior_work.tex <==
\section{Other Related Work}
\label{sec:prior}

In the past, different notions of approximate fault-tolerance, besides $(f, \, \epsilon)$-resilience, have been used to analyze Byzantine fault-tolerance of different distributed optimization algorithms~\cite{diakonikolas2018sever, su2016fault}. As we discuss below in Section~\ref{sub:alt_approx}, the difference between these other definitions and our definition of $(f, \, \epsilon)$-resilience arises mainly due to the applicability of the distributed optimization problems. Later, in Section~\ref{sub:gf_prior}, we discuss some prior work on gradient-filters used for achieving Byzantine fault-tolerance in the distributed gradient-descent method.
% We present below a comparison between the different definitions of approximate fault-tolerance and our definition of $(f, \, \epsilon)$-resilience.

\subsection{Alternate Notions of Approximation in Fault-Tolerance}
\label{sub:alt_approx}

As proposed by Su and Vaidya, 2016~\cite{su2016fault}, 
% an alternate way of measuring approximation in fault-tolerance is by use of weights. Specifically, 
instead of a minimum point of the {\em uniformly weighted} aggregate of non-faulty agents' cost functions, a distributed optimization algorithm may output a minimum point of a {\em non-uniformly weighted} aggregate of non-faulty costs, i.e., $\sum_{i \in \H} \alpha_i \, Q_i(x)$,
where $\H$ denotes the set of at least $n-f$ non-faulty agents, and $\alpha_i \geq 0$ for all $i \in \H$. As is suggested in~\cite{su2016fault}, upon re-scaling the coefficients such that $\sum_{i \in \H} \alpha_i = 1$, we can measure approximation in fault-tolerance using two metrics; (1) the number of coefficients in $\{\alpha_i, \, i \in \H\}$ that are positive, and (2) the minimum positive value amongst the coefficients: $\min \left\{ \alpha_i; \, \alpha_i > 0, \, i \in \H \right\}$. Results on the achievability of this particular form of approximation for the scalar case (i.e., $d = 1$) can be found in~\cite{su2016fault, su2020byzantine}. However, we are unaware of similar results for the case of higher-dimensional optimization problem, i.e., when $d > 1$. There is some work on this particular notion of approximate fault-tolerance in high-dimensions, such as~\cite{su2018finite, yang2017byrdie}, however their results only apply to special cost functions, specifically, quadratic or strictly convex functions, as opposed to the generic cost functions (that need not even be differentiable) considered in this paper. \\

Another way of measuring approximation is by the value of the aggregate cost function, or its gradient. For instance, as discussed in~\cite{diakonikolas2018sever}, for the case of differentiable cost functions a resilient distributed optimization algorithm $\Pi$ may output a point $x_{\Pi} \in \R^d$ such that each element of the aggregate non-faulty gradient $\sum_{i \in \H} \nabla Q_i(x_{\Pi})$ is bounded by $\epsilon$. As yet another alternative, a resilient algorithm $\Pi$ may aim to output a point $x_\Pi$
such that the non-faulty aggregate cost $\sum_{i \in \H} Q_i(x_\Pi)$ is within $\epsilon$ of the true minimum cost $\min_x \sum_{i \in \H} Q_i(x)$. However, these definitions of approximate resilience are sensitive to scaling of the cost functions. In particular, if the elements of $\sum_{i \in \H} \nabla Q_i(x_\Pi)$ are bounded by $\epsilon$ then the elements of $\sum_{i \in \H} \alpha \nabla Q_i(x_\Pi)$ are bounded by $\alpha \epsilon$, where $\alpha$ is a positive scalar value. On the other hand, both $\sum_{i \in \H} Q_i(x)$ and $\sum_{i \in \H} \alpha Q_i(x_\Pi)$ have identical minimum point regardless of the value of $\alpha$. Therefore, when the objective is to approximate a minimum point of the non-faulty aggregate cost $\arg \min_x \sum_{i \in \H} Q_i(x)$, which is the indeed the case in this paper, use of function (or gradient) values to measure approximation is not a suitable choice. 

% As mentioned above, an approximately fault-tolerant distributed optimization algorithm outputs a {\em sub-optimal point} that may only approximately minimize the non-faulty aggregate cost function. Now, as discussed below in Section~\ref{sub:alt_approx}, there are several ways of defining sub-optimality. However, as our goal is to find an approximate minimum point, we define approximate fault-tolerance in terms of the Euclidean distance between the output of a prescribed algorithm and a true minimum point (if it exists) of the non-faulty aggregate cost. Formally, we define approximate fault-tolerance by {\em $(f, \, \epsilon)$-resilience} where $\epsilon \in \R_{\geq 0}$. 

%There is some prior work focusing the aggregator of vectors as a key component of solving Byzantine fault-tolerance learning problems. As an example, Karimireddy et al. \cite{karimireddy2020learning} consider the following problem: Given an aggregation rule $\textsc{Agg}(\cdot)$ and $n$ vectors $\{\boldsymbol{x}_1,...,\boldsymbol{x}_n\}$, where $\mathcal{G}\in[n]$ are good and the rest are Byzantine. An ideal aggregator returning the average of only good vectors $\overline{\boldsymbol{x}}=\frac{1}{\mnorm{\G}}\sum_{j\in\G}\boldsymbol{x}_\G$ requires identifying the good workers, and hence may not be possible. An acceptable substitution would be to approximate the ideal outcome up to some error. They propose the definition of  \textit{$(\delta_{\max},c)$-robust aggregator}, that for some $\delta\leq\delta_{\max}$, the given $n$ vectors and the good subset $\G$ with $\G\geq(1-\delta)n$ satisfies $\expectation{\boldsymbol{x}_i}=\expectation{\boldsymbol{x}_j}$ and $\expectation{\norm{\boldsymbol{x}_i-\boldsymbol{x}_j}^2}\leq\rho^2$ for any $i,j\in\G$, a $(\delta_{\max},c)$-robust aggregator on the group of vectors $\textsc{Agg}\left(\boldsymbol{x}_1,\dots,\boldsymbol{x}_n\right)$ returns $\widehat{\boldsymbol{x}}$, that for some constant $c$, $\expectation{\norm{\widehat{\boldsymbol{x}}-\overline{\boldsymbol{x}}}^2}\leq c\delta\rho^2$. The definition of the robust aggregator bounds the error of its output, while the vectors or random variables $\{\boldsymbol{x}_i\}$ are not independent, but rather having their expected pair-wise distances bounded. When applied to distributed optimization, such dependency among the vectors or gradients implies some redundancy among data points from agents. The authors further present a Byzantine robust distributed optimization algorithm incorporating momentum SGD and any robust aggregator. Note that the authors only provide convergence analysis, and utilizing worker momentum is required; analysis on possible error between the output of an algorithm and the true minimum point is unclear.

\subsection{Gradient-Filters}
\label{sub:gf_prior}

In the past, several {gradient-filters} have been proposed to {\em robustify} the distributed gradient-descent (DGD) method against Byzantine faulty agents in a server-based architecture, e.g., see~\cite{alistarh2018byzantine, blanchard2017machine, damaskinos2018asynchronous, diakonikolas2018sever, gupta2020byzantine, prasad2018robust, su2016fault, yin2018byzantine}. 
% The DGD method is an iterative distributed optimization algorithm wherein the server maintain an estimate of the solution (a valid minimum point), and updates it iteratively using gradients computed by the agents of their respective cost functions. In the traditional DGD method, the server updates its estimates using the average (or sum) of agents' gradients. However, gradient averaging is rendered ineffective when Byzantine faulty agents send arbitrary incorrect gradients~\cite{su2016fault}.\\
A gradient-filter refers to {\em Byzantine robust aggregation} of agents' gradients that mitigates the detrimental impact of incorrect gradients sent by the Byzantine agents to the server. To name a few gradient-filters, that are provably effective against Byzantine agents, we have the comparative gradient elimination (CGE)~\cite{gupta2019byzantine, gupta2020byzantine}, coordinate-wise trimmed mean (CWTM)~\cite{su2016fault, yin2018byzantine}, geometric median-of-means (GMoM)~\cite{chen2017distributed}, KRUM~\cite{blanchard2017machine}, Bulyan~\cite{guerraoui2018hidden}, and other spectral gradient-filters~\cite{diakonikolas2018sever}. Different gradient-filters guarantee some fault-tolerance under different assumptions on non-faulty agents' cost functions. \\

In this paper, we propose a generic result, in Theorem~\ref{thm:upper-bound-D} in Section~\ref{sec:grad_des}, on the convergence of the DGD method equipped with a gradient-filter. The result holds true regardless of the gradient-filter used, and thus, can be utilized to obtain formal fault-tolerance property of a gradient-filter in context of the considered distributed optimization problem. We demonstrate this, in Section~\ref{sec:grad_filters}, by obtaining $(f, \, \epsilon)$-resilience properties of two specific gradient-filters; CGE and CWTM. As exact fault-tolerance is equivalent to $(f, \, 0)$-resilience (see Section~\ref{sub:approx}), our results generalize the prior work on exact fault-tolerance of these two filters, see~\cite{gupta2019byzantine, gupta2020byzantine, su2018finite}. Moreover, until now, exact fault-tolerance of the CWTM gradient-filter was only studied for special optimization problems of state estimation~\cite{su2018finite}, and machine learning~\cite{yin2018byzantine}. Our result presents the fault-tolerance property of CWTM for a much larger class of optimization problems.
% In Section~\ref{sec:grad_filters}, we present approximate fault-tolerance properties of CGE and CWTM gradient-filters that are applicable to the more general distributed optimization problem, and also encapsulates the special case of exact fault-tolerance. 

\subsection{Robust Statistics with Arbitrary Outliers}
As noted earlier, there has been work on the problem of robust statistics with arbitrary outliers~\cite{charikar2017learning,feng2014distributed,steinhardt2017resilience}. In this problem, we are given a finite set of data points; $\alpha$ fraction of which are sampled independently and identically from a common distribution $\mathcal{D}$ in $\R^d$, and the remaining $1 - \alpha$ fraction of data points may be arbitrary. The identity of arbitrary data points is a priori unknown, otherwise the problem is trivialized. The objective in this problem is to estimate statistical measures of distribution $\mathcal{D}$, such as mean, or variance, despite the presence of arbitrary outliers. The problem robust mean estimation can potentially be modelled as a fault-tolerant distributed optimization problem where for each non-faulty agent $i$, $Q_i(x): (x, \, x_i) \mapsto y \in \R$ for all $x \in \R^d$ where $x_i \sim \mathcal{D}$. A faulty agent may choose an arbitrary cost function. The cost functions can be designed in a manner such that the minimum point of the aggregate of non-faulty cost functions is equal to the mean for the non-faulty data points. 
% We note that our results are also applicable to the problem of robust statistics with arbitrary outliers~\cite{charikar2017learning,steinhardt2017resilience}. In this particular problem, we are given a finite set of data points; $\alpha$ fraction of which are sampled independently and identically from a common distribution $\mathcal{D}$ in $\R^d$, and the remaining $1 - \alpha$ fraction of data points may be arbitrary. The identity of arbitrary data points is a priori unknown, otherwise the problem is trivialized. The objective in this problem is to estimate statistical measures of distribution $\mathcal{D}$, such as mean, or variance, despite the presence of arbitrary outliers. The problem of robust statistics can be equivalently modelled as a fault-tolerant distributed optimization problem where for each non-faulty agent $i$, $Q_i(x): (x, \, x_i) \mapsto y \in \R$ for all $x \in \R^d$ where $x_i \sim \mathcal{D}$. A faulty agent may choose an arbitrary cost function. The cost functions can be designed in a manner such that the minimum point of the aggregate of non-faulty cost functions is equal to the statistical measure to be computed for the non-faulty data points. Consequentially, our necessary and sufficient conditions for approximate fault-tolerance in distributed optimization generalize the existing feasibility bounds on robust statistical estimations with arbitrary outliers~\cite{charikar2017learning,steinhardt2017resilience}. \\
%
In particular, suppose that for each non-faulty agent $i$, $Q_i(x) \triangleq \norm{x - x_i}^2$ where $x_i \sim \mathcal{D}$.
% A faulty agent $j$ may choose a cost function of $Q_j(x) \triangleq \norm{x - x_j}^2$ where $x_j$ is an arbitrary point in $\R^d$.
In this case, the minimum point of the non-faulty aggregate cost function is equal to the average of the non-faulty data points sampled from distribution $\mathcal{D}$.\\
% Here, our necessary and sufficient conditions for approximate fault-tolerance provide lower and upper bounds for robust mean estimation in presence of arbitrary outlying data points.

Prior work on robust statistics considers a centralized setting wherein, unlike a distributed setting, all the data points are accessible to a single machine. In this report, we also present distributed algorithms that do not require the agents to share their local data points. Moreover, in the centralized setting, our results are applicable to a larger class of cost functions, including non-convex functions.

\subsection{\bf Fault-tolerance in State Estimation} 
The problem of distributed optimization finds direct application in distributed state estimation~\cite{rabbat2004distributed}. In this problem, the system comprises multiple sensors, and each sensor makes partial observations about the system's state. The goal is to compute the entire state of the system using collective observations from all the sensors. However, if a sensor is faulty then it may share incorrect observations, preventing correct state estimation. The special case of distributed state estimation when the observations are {\em linear} in the system's state has gained significant attention in the past, e.g. see~\cite{bhatia2015robust, chong2015observability, mishra2016secure, pajic2017attack, pajic2014robustness, shoukry2015imhotep, shoukry2017secure, su2018finite}. These works have shown that the state can be determined despite up to $f$ (out of $n$) faulty observations {\em if and only if} the system is {\em $2f$-sparse observable}, i.e., the complete state can be determined using observations of only $n-2f$ non-faulty sensors. We note that, in this particular case, {\em $2f$-sparse observability} is equivalent to $2f$-redundancy. Additionally, some of these works, such as~\cite{mishra2016secure, su2018finite}, also consider the case of {\em approximate} linear state estimation when the observations are noisy. Our work is more general in that we consider the problem setting of distributed optimization, and our results apply to a larger class of cost functions.
% Note that the problem of fault-tolerant linear state estimation with noisy observations can be modelled easily as approximate fault-tolerance (defined in the paper). Therefore, our results apply easily to fault-tolerant linear state estimation with noisy observations. Moreover, unlike these works, our results are applicable to a much larger class of state estimation problems wherein the state observations can be nonlinear. 
% our presented feasibility conditions provide a tighter relationship (up to a multiplicative constant) between the accuracy of state estimation feasible (with faulty observations) and the magnitude of noise in the state observations.\\



% . We note that the property of {\em $2t$-sparse observability} is a special instance of the more general {\em $2t$-redundancy} property presented in this report. Moreover, the necessity and sufficiency of the \mbox{\em $2t$-redundancy} property proved in this report implies the necessity and sufficiency of {\em $2t$-sparse observability} for fault-tolerant state estimation for a more general setting wherein the sensor observations may be non-linear; however, the converse is not true.\\

==> sufficiency_necessity.tex <==
% \section{Approximate Fault-Tolerance}
% 
% In this section, we present the notion of approximate fault-tolerance. 

% Alternately, for the set of all non-faulty agents $\H$, a
% % if $\mathcal{B}\in\{1,...,n\}$ with $\mnorm{\mathcal{B}} \leq f$ denotes the set of faulty agents, and $\mathcal{H}=\{1,...,n\}\\\mathcal{B}$ denotes the set of non-faulty agents, 
% $(f, \,\epsilon)$-resilient distributed optimization algorithm outputs a point within a Euclidean distance of $\epsilon$ from the set of true minimums
% \[\arg\min_x\sum_{i\in\mathcal{H}}Q_i(x).\]

% In this paper, we show that for achieving $(f, \, \epsilon)$-resilience we only require a relaxed redundancy property named {\em $(2f, \, \epsilon)$-redundancy}, which is defined below, instead of the more stringent {$2f$-redundancy} property defined in Definition~\ref{def:red}  above. \\

\subsection{Necessary and Sufficient Conditions for $(f, \, \epsilon)$-Resilience}
\label{sub:cond_res}

In this section, we first show in Theorem~\ref{thm:necc} that $(f,\epsilon)$-resilience can be achieved only if the non-faulty cost functions satisfy the {\em $(2f, \, \epsilon)$-redundancy} property, stated below in Definition~\ref{def:approx_red}, which is a relaxation of the {\em $2f$-redundancy} property introduced in our prior work \cite{gupta2020fault}. Then, in Theorem~\ref{thm:suff} we show that if the {\em $(2f, \, \epsilon)$-redundancy} property is satisfied then $(f, \, 2\epsilon)$-resilience is achievable. Throughout this section, we assume that $f > 0$, otherwise the problem becomes trivial.\\
% The factor of $2$ separating the necessary condition from the sufficient . .... \\

To be able to formally state our results 
% define $(2f, \, \epsilon)$-redundancy for an arbitrary real value $\epsilon \geq 0$ 
we review below definitions of; i) the Euclidean distance between a point and a set, and ii) the Euclidean norm based {Hausdorff distance} -- a {metric} for measuring distance between sets~\cite{munkres2000topology}. 

\begin{definition}
The Euclidean distance between a point $x$ and a set $X$ in the real space $\R^d$, denoted by \dist{x}{X}, is defined as follows:
\begin{align*}
    \dist{x}{X} = \inf_{y\in X}\norm{x-y}.
\end{align*}
\end{definition}

% To define the approximate redundancy, we first introduce the following notation: 
\begin{definition}
    The Euclidean norm based Hausdorff distance between two sets $X$ and $Y$ in the real space $\R^d$, denoted by $\dist{X}{Y}$, is defined as follows:
    % between two sets $X$ and $Y$ is defined as follows:
    \begin{equation*}
        \dist{X}{Y}\triangleq\max\left\{\sup_{x\in X}\inf_{y\in Y}\norm{x-y}, ~ \sup_{y\in Y}\inf_{x\in X}\norm{y-x}\right\}.
    \end{equation*}
\end{definition}

We now define the $(2f, \, \epsilon)$-redundancy property as follows.
% It can be induced that the distance between any two point $x$ and $y$ is 
% \begin{equation*}
%     \dist{x}{y}=\norm{x-y},
% \end{equation*}
% while the distance $\dist{x}{Y}$ between a point $x$ and a set $Y$ is the infimum of the distance between $x$ and any point in $Y$. When using distance induced by Euclidean norms, we have
% \begin{equation*}
%     \dist{x}{Y}=\inf_{y\in Y}\dist{x}{y}=\inf_{y\in Y}\norm{x-y}.
% \end{equation*}
% %Note that if $Y$ is closed, we further have $\dist{x}{Y}=\min_{y\in Y}\dist{x}{y}$. 
% Under this definition, the distance on non-empty compact sets allows triangle inequality.

% \begin{definition}[\textbf{$(2f,\epsilon)$-redundancy}]
% Let $Q_i(x)$ denote the true cost function of agent $i$. The $n$ agents are said to satisfy $(2f,\epsilon)$-redundancy if there exists some real number $\epsilon\geq0$, such that the following holds for any subset $S$ containing \emph{at least} $n-2f$ agents: let $X^*=\arg\min_x\sum_{i\in\H}Q_i(x)$, and $X_S=\arg\min_x\sum_{i\in S}Q_i(x)$,
% \begin{equation*}
%     \dist{X^*}{X_S}\leq\epsilon.
% \end{equation*}
% %\begin{itemize}
% %    \item For all $x_S\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in S}Q_i(x)$, there exists $x^*\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in \mathcal{H}}Q_i(x)$ such that
% %    \[\norm{x^*-x_S}\leq\epsilon.\]
% %    \item For all $x^*\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in \mathcal{H}}Q_i(x)$, there exists $x_S\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in S}Q_i(x)$ such that
% %    \[\norm{x^*-x_S}\leq\epsilon.\]
% %\end{itemize}
% \end{definition}

\begin{definition}[\textbf{$(2f, \, \epsilon)$-redundancy}]
\label{def:approx_red}
% Given the set of non-faulty agents $\H$, the 
% Suppose that $\H$ denotes the set of non-faulty agents. 
The non-faulty cost functions are said to satisfy the {\em $(2f, \, \epsilon)$-redundancy} property if and only if for every pair of subsets $S, \,\widehat{S} \subseteq \{1, \ldots, \, n\}$ with
% $\widehat{S} \subseteq S \subseteq \H$, 
$\mnorm{S} \geq n-f$, $\mnorm{\widehat{S}} \geq n-2f$ and $\widehat{S} \subseteq S$,
% and $\widehat{S} \subseteq S$, 
\begin{equation}
    \dist{\arg\min_x\sum_{i\in S}Q_i(x)}{\arg\min_x\sum_{i\in \widehat{S}}Q_i(x)} \leq \epsilon. \label{eqn:red_dist}
    % \dist{X_{S}}{X_{\widehat{S}}}\leq\epsilon
\end{equation}
% where $X_{S} = \arg\min_x\sum_{i\in S}Q_i(x)$ and $X_S = \arg\min_x\sum_{i\in \widehat{S}}Q_i(x)$.
%\begin{itemize}
%    \item For all $x_S\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in S}Q_i(x)$, there exists $x^*\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in \mathcal{H}}Q_i(x)$ such that
%    \[\norm{x^*-x_S}\leq\epsilon.\]
%    \item For all $x^*\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in \mathcal{H}}Q_i(x)$, there exists $x_S\in\arg\min_{x\in\mathbb{R}^d}\sum_{i\in S}Q_i(x)$ such that
%    \[\norm{x^*-x_S}\leq\epsilon.\]
%\end{itemize}
\end{definition}

By Definitions~\ref{def:red} and~\ref{def:approx_red}, the property of $2f$-redundancy is equivalent to $(2f, \, 0)$-redundancy. Alternately, $2f$-redundancy implies $(2f, \, \epsilon)$-redundancy for all $\epsilon \geq 0$. Therefore, $(2f, \, \epsilon)$-redundancy for some $\epsilon > 0$ is a weaker condition in comparison to $2f$-redundancy. \\

We present below our key result on the {\bf necessity of the $(2f, \, \epsilon)$-redundancy property for $(f, \, \epsilon)$-resilience}. In particular, we show that if the $(2f, \, \epsilon)$-redundancy property is violated for a pair of subsets $S, \, \widehat{S}$ with $\mnorm{S} = n-f$, $\mnorm{\widehat{S}} = n-2f$ and $\widehat{S} \subseteq S$ then $(f, \epsilon)$-resilience cannot be achieved.

% Also, we note the following implication of the violation of the {$(2f, \, \epsilon)$-redundancy} property

% \begin{lemma}
% \label{lem:red_imply}
% Suppose that Assumption~\ref{assum:compact} holds true, $d = 1$, and that the agents' cost functions are strictly convex. If $f > 0$ and the $(2f, \, \epsilon)$-redundancy property is violated for some $\epsilon \geq 0$ then there exists a pair of subsets $T, \, \widehat{T} \subset \{1, \ldots, \, n\}$ with $\mnorm{T} = n-f$, $\mnorm{\widehat{T}} = n-2f$ and $\widehat{T} \subset T$ such that
% \begin{align*}
%     \dist{\arg\min_x\sum_{i\in T}Q_i(x)}{\arg\min_x\sum_{i\in \widehat{T}}Q_i(x)} > \epsilon.
% \end{align*}
% \end{lemma}
% The proof of Lemma~\ref{lem:red_imply} is deferred to Appendix~\ref{app:red_imply}. 
% Now, we present our {key result} on the necessity of {$(2f, \, \epsilon)$-redundancy} for {$(f, \, \epsilon)$-resilience}.

% \begin{lemma}
%     Suppose there are two real numbers $\epsilon$ and $\epsilon$, $0<\epsilon<\epsilon$.
%     \begin{enumerate}[label=(\arabic*)]
%         \item A $(f,\epsilon)$-resilient algorithm is also $(f,\epsilon)$-resilient;
%         \item A $(f,\epsilon)$-resilient algorithm is not necessarily $(f,\epsilon)$-resilient.
%     \end{enumerate}
%     \label{lem:resil}
% \end{lemma}

% \begin{proof}
%     A $(f,\epsilon)$-resilient algorithm outputs $\widehat{x}$ that satisfies the following: $\widehat{x}\in B(x^*,\epsilon)$. Since $\epsilon>\epsilon$, $B(x^*,\epsilon)\subsetneq B(x^*,\epsilon)$. Therefore, $\widehat{x}$ must also satisfy $\widehat{x}\in B(x^*,\epsilon)$, which proves (1).
    
%     Suppose an algorithm always output $\widehat{x}$ on the circle $C(x^*,\epsilon)$, since $C(x^*,\epsilon)\subsetneq B(x^*,\epsilon)$, the algorithm is $(f,\epsilon)$-resilient. However, for any real number $\epsilon<\epsilon$, $C(x^*,\epsilon)\cap B(x^*,\epsilon)=\varnothing$, or $\widehat{x}\notin B(x^*,\epsilon)$. Therefore, the algorithm is not $(f,\epsilon)$-resilient, which proves (2).
% \end{proof}

% The definition of $(f,\epsilon)$-resilience directly leads to the following lemma:
% \begin{lemma}
%     Suppose there are two real numbers $\epsilon$ and $\epsilon$, $0<\epsilon<\epsilon$.
%     \begin{enumerate}[label=(\arabic*)]
%         \item A group of true cost functions that are $(2f,\epsilon)$-redundant are also $(2f,\epsilon)$-redundant;
%         \item A group of true cost functions that are $(2f,\epsilon)$-redundant are not necessarily $(2f,\epsilon)$-redundant;
%     \end{enumerate}
%     \label{lem:resil}
% \end{lemma}

% Next, we show that $(f, \, \epsilon)$-resilience can be achieved only if the agents' cost functions satisfy a {\em relaxed} $2f$-redundancy property named {\em $(2f, \, \epsilon)$-redundancy}. To be able to define $(2f, \, \epsilon)$-redundancy we introduce below a standard metric to measure distances between sets called Hausdorff distance~\cite{}.\\



% ow, differentiability of $\sum_{i\in S}Q_i(x)$ also implies that 

% By Assumption~\ref{assum:compact}, for any subset $S\subseteq[n]$, $\arg\min_x\sum_{i\in S}Q_i(x)$ is also compact.\\
%\begin{definition}[$(f,\epsilon)$-resilience]
%A distributed optimization algorithm is $(f,\epsilon)$-resilient if it outputs an approximation $\widehat{x}$ of a minimum of the aggregate cost of all the non-faulty agents, such that $\distance(X^*,\widehat{x})\leq\epsilon$, despite the presence of up to $t$ Byzantine faulty agents.
%\end{definition}



\begin{theorem}
% [Necessity]
\label{thm:necc}
% Suppose that the non-faulty cost functions are differentiable and convex. 
For $\epsilon \geq 0$, there exists a deterministic $(f, \,\epsilon)$-resilient distributed optimization algorithm {\em only if} the non-faulty cost functions satisfy the distance condition~\eqref{eqn:red_dist} of $(2f,\epsilon)$-redundancy for all pairs of subsets $S, \, \widehat{S}$ with $\mnorm{S} = n-f$, $\mnorm{\widehat{S}} = n-2f$ and $\widehat{S} \subseteq S$.
\end{theorem}

\begin{proof}

We prove the theorem for the case of strictly convex scalar cost functions, i.e. $d = 1$ and for each agent $i$, $Q_i: \R \to \R$. First, note that if the condition is necessary for the scalar case then it is so for the general vector case. Second, our arguments can be easily extended for the case when $d > 1$. As the theorem is rendered vacuous when $f = 0$, we assume that $f > 0$.\\

To prove the necessity condition, we also assume that the server has full knowledge of all the agents' cost functions. This may not hold true in practice, where instead the server may only have partial information about the agents' cost functions. Indeed, this forces the Byzantine faulty agents to a priori fix their cost functions. However, in reality the Byzantine agents may send arbitrary information over time to the server that need not be consistent with a fixed cost function. Thus, necessity of $(2f,\epsilon)$-redundancy under this assumption implies its necessity in general. \\

The proof is by contradiction. Specifically, we show the following:
\begin{quote}
    %If the non-faulty cost functions satisfy $(2f,\epsilon)$-redundancy for some $\epsilon$, deterministic distributed optimization algorithm cannot guarantee $(f,\epsilon-\delta)$-resilience, for any $\delta$, $0\geq\delta<\epsilon$.
    %For some $\epsilon>0$, if the non-faulty cost functions do not satisfy $(2f,\epsilon)$-redundancy, deterministic distributed optimization algorithm cannot guarantee $(f,\epsilon)$-resilience.
    %, for any $\delta$, $0\geq\delta<\epsilon$.
    {\em If the non-faulty cost functions do not satisfy the $(2f,\epsilon)$-redundancy property for a pair of subsets $S, \widehat{S}$, with $\mnorm{S} = n-f$, $\mnorm{\widehat{S}} = n-2f$ and $\widehat{S} \subseteq S$, then there cannot exist a deterministic  $(f,\epsilon)$-resilient distributed optimization algorithm.}
\end{quote}
% We show that the above statement is

\noindent Suppose that the non-faulty costs {\bf do not} satisfy the $(2f,\epsilon)$-redundancy property for the aforementioned pair of subsets $S, \, \widehat{S}$. Recall that, as the cost functions are assumed strictly convex, for a non-empty set of agents $S$ the aggregate cost function $\sum_{i \in S} Q_i(x)$ has a unique minimum point that we denote by $x_S$. Specifically, for a subset of agents $S$, let 
\[x_S = \arg \min_x \sum_{i \in S} Q_i(x).\]
The violation of $(2f,\epsilon)$-redundancy property implies that
% there exits a pair of sets $S, \, \widehat{S} \subseteq \{1, \ldots, \, n\}$ with $\mnorm{S} \geq n-f$, $\mnorm{\widehat{S}} \geq n-2f$ and $\widehat{S} \subseteq S$ such that 
% \begin{align*}
%     \norm{x_{\widehat{S}} - x_S} = \epsilon + \delta
% \end{align*}
% where $\delta > 0$. As shown in Lemma~\ref{lem:red_imply} presented in Appendix~\ref{app:red_imply}, the above implies that 
% there exists a pair of sets $T, \, \widehat{T} \subset \{1, \ldots, \, n\}$ with $\mnorm{T} = n-f$, $\mnorm{\widehat{T}} = n-2f$ and $\widehat{T} \subset T$ such that
\begin{align}
    \norm{x_{\widehat{S}} - x_S} \geq \epsilon + \delta \label{eqn:no_red_asp}
\end{align}
where $\delta > 0$.\\
% \textcolor{red}{\bf ++++ editing +++++ }
% \\

% For a subset $S_0$ comprising of $n-2f$ non-faulty agents, suppose that the minimum point of the aggregated cost function of the agents in $S_0$ is unique. We denote
% \begin{equation}
%     x_0=\arg\min\sum_{i\in S_0}Q_i(x).
% \end{equation}
% Let set $S_1$ denote the remaining $f$ non-faulty agents. Suppose that the minimum point of the aggregated cost function of all the non-faulty agents in $S_0 \cup S_1$ is also unique. We denote
% % A set $S_1\subset\{1,...,n\}\backslash S_0$ of $t$ agents has
% \begin{equation}
%     x_1=\arg\min_x\sum_{i\in S_0\cup S_1}Q_i(x)
% \end{equation}
% As we have assumed that the non-faulty agents do not satisfy the $(2f,\epsilon)$-redundancy, there exist the aforementioned sets $S_0$ and $S_1$, and $\delta > 0$, such that $x_0$ is $\epsilon + \delta$ distance away from $x_1$, i.e.,
% \begin{align*}
%     \norm{x_0 - x_1} = \epsilon + \delta.
% \end{align*}
Suppose that all the remaining $f$ agents in the set $\B = \{1, \ldots, \, n\} \setminus S$ are Byzantine faulty that choose to send strictly convex scalar cost functions, similar to the non-faulty agents, such that - 
\begin{quote}
the aggregate cost function of the agents in the set $\B \cup \widehat{S}$ minimizes at point $x_{\B \cup \widehat{S}}$ which is also $\norm{x_{\widehat{S}} - x_{S}}$ distance away from $x_{\widehat{S}}$, similar to $x_S$, but lies on the other side of $x_{\widehat{S}}$ as shown in the figure below.
\end{quote}

% The remaining $f$ agents denoted by set $S_2 = \{1,...,n\} \setminus S_0 \setminus S_1$ are Byzantine faulty. A Byzantine faulty agent $i \in S_2$ chooses a cost function $Q_i(x): \R \to \R$ with similar properties as a non-faulty cost function such that the following conditions hold true. 
% \begin{itemize}
%     \item The minimum point of the aggregated cost function of the agents in $S_0 \cup S_2$ is unique. We denote 
%     \begin{equation*}
%         x_2=\arg\min_x\sum_{i\in S_0\cup S_2}Q_i(x).
%     \end{equation*}
%     \item The distance between $x_0$ and $x_2$ is $\epsilon + \delta$, i.e., $\norm{x_0 - x_2} = \epsilon + \delta$. However, the point $x_2$ lies in the other half of the real line $\R$ than the point $x_1$ as shown in the figure below.
% \end{itemize}

\begin{center}
    \begin{tikzpicture}
        \node[dot] (x1) at (-2,0) {};
        \node[dot] (x0) at (0,0) {};
        \node[dot] (x2) at (2,0) {};
        \node at (-2,-.35) {$x_S$};
        \node at (0,-.35) {$x_{\widehat{S}}$};
        \node at (2,-.35) {$x_{\B \cup \widehat{S}}$};
        \draw (-4,0) -- (x0)
              (x0) -- (4,0);
        %\node[dot] at (-2,0) {};
        %\node[dot] at (2,0) {};
              
        %\node[dot, color=red] (xhat) at (-1.7,0) {};
        %\node at (-1.7,-.4) {\textcolor{red}{$x^*_{(1)}$}};
        %\node[dot, color=red] (xhat2) at (1.6,0) {};
        %\node at (1.6,-.4) {\textcolor{red}{$x^*_{(2)}$}};
        
        \node at (-.3,0) {]};
        \node at (-3.7,0) {[};
        \node at (-1,.36) {\footnotesize\textcolor{blue}{$\leftarrow\epsilon+\delta\rightarrow$}};
        \node at (1,.36) {\footnotesize\textcolor{blue}{$\leftarrow\epsilon+\delta\rightarrow$}};
        \node at (-1.2,-.3) {\textcolor{blue}{\footnotesize $\epsilon$}};
        \node at (-2.8,-.3) {\textcolor{blue}{\footnotesize $\epsilon$}};

        \node[dot, color=red] (xhat) at (-.5,0) {};
        \node at (-.5,-.4) {\textcolor{red}{$\widehat{x}$}};
        \label{fig:illustrate}
    \end{tikzpicture}
\end{center}

\noindent Note that the distance between the two points $x_S$ and $x_{\B \cup \widehat{S}}$ is $2\epsilon + 2\delta$, i.e.,
\begin{align}
    \norm{x_S - x_{\B \cup \widehat{S}}} = 2\epsilon + 2\delta. \label{eqn:dist_x1_x2}
\end{align}
% The functions can be constructed. Suppose each cost function $Q_i(x)$, $i\in S_0$ satisfies $Q_i(x)=Q_i(2x_0-x)$. To satisfy the conditions stated above, for every cost function $Q_i(x)$, $i\in S_1$, one can construct another function $Q_j(x)=Q_i(2x_0-x)$, to be the cost function of an agent $j\in S_2$. \\%(See Figure~\ref{fig:constructQ})\\
%$\distance(x_0,x_1)=\distance(x_0,x_2)=\epsilon$. And functions in $S_0$, $S_1$, and $S_2$ are symmetric with respect to $x_0$, meaning for any $Q_i$ in $X_0$, $Q_i(x)=Q_i(2x_0-x)$, and for any $Q_i\in S_1$ and $Q_j\in S_2$, $Q_i(x)=Q_j(2x_0-x),~\forall x$. \\
We now show below, by contradiction, that there cannot exist a deterministic $(f, \, \epsilon)$-resilient distributed optimization algorithm.\\

Suppose that there exists an $(f, \, \epsilon)$-resilient deterministic optimization algorithm named $\Pi$. As the identity of Byzantine faulty agents is a priori unknown to the server, and the Byzantine faulty agents also send strictly scalar functions to the server,
% and the faulty cost functions are assumed differentiable and convex, 
the server cannot distinguish between the two possible scenarios with equal number of Byzantine faults; i) $S$ is the set of non-faulty agents, and ii) $\B \cup \widehat{S}$ is the set of non-faulty agents. \\

As the cost functions received by the server is identical in both the scenarios, the output of algorithm $\Pi$ should also be identical. We let $\widehat{x}$ denote the output of $\Pi$. Now, consider scenario (i) when the set of honest agents is $S$. As algorithm $\Pi$ is $(f,\epsilon)$-resilient, by Definition~\ref{def:approx_res}, the output $\widehat{x} \in  [x_S - \epsilon, \, x_S + \epsilon]$ as shown in the figure above. By the same logic, in scenario (ii) where the set of honest agents is $\B \cup \widehat{S}$ the output $\widehat{x} \in  [x_{\B\cup \widehat{S}} - \epsilon, \, x_{\B\cup \widehat{S}} + \epsilon]$. However, ~\eqref{eqn:dist_x1_x2} implies that $\widehat{x}$ cannot belong to both the intervals simultaneously. Therefore, if algorithm $\Pi$ is $(f,\epsilon)$-resilient then it cannot be so in scenario (ii), and vice-versa. This contradicts the assumption that $\Pi$ is $(f, \, \epsilon)$-resilient. Consequently, there cannot exist a deterministic $(f, \, \epsilon)$-resilient algorithm if the $(2f, \, \epsilon)$-redundancy property is violated.

% By $(2f,\epsilon+\delta)$-redundancy, since $\mnorm{\H_{(0)}}=n-f$ while $\mnorm{S_0}=n-2f$, we should have
% \[\dist{\arg\min_x\sum_{i\in\H_{(1)}}Q_i(x)}{\arg\min_x\sum_{i\in S_0}Q_i(x)}\leq(\epsilon+\delta).\] %Suppose $\mathcal{H}$ denotes the set of non-faulty agents in an execution of $\Pi$. Recall that $|\mathcal{H}|\geq n-f$ and $n>2f$. 
% Note that $\arg\min_x\sum_{i\in\H_{(1)}}Q_i(x)=x_1$ and $\arg\min_x\sum_{i\in S_0}Q_i(x)=x_0$, the condition above is satisfied. On the other hand, since $\Pi$ is $(f,\epsilon)$-resilient, the output $\widehat{x}$ of $\Pi$ would be within range $[-\epsilon+x_1,\epsilon+x_1]$, as shown in the figure below.\\


% Now consider scenario (2) where the honest agents are in the set $\mathcal{H}_{(2)}=S_0\cup S_2$. Since $S_1$ and $S_2$ are symmetric, the optimum of aggregation of true cost functions from honest agents is now $x_2=\arg\min_x\sum_{i\in\mathcal{H}_{(2)}}Q_i(x)$. However, since $\Pi$ is deterministic and all functions from agents are not changed, it would still output the same $\widehat{x}$ as it would in scenario (1). The distance $\norm{x_2-\widehat{x}}>\epsilon+\delta>\delta$. Therefore, $\widehat{x}$ does not satisfy $(f,\epsilon)$-resilience. Contradiction.
%
%%%%%%%%%%%%%%% Vector Case %%%%%%%%%%%%%%%%
%\begin{center}
%    $\mathsection~~~\mathsection~~~\mathsection$
%\end{center} 
%
%We consider a subset $S_0$ comprising of $n-2f$ non-faulty agents, and denote by $x_0$ a minimum point of the aggregate costs of the agents in $S_0$. Specifically, 
%\[x_0\in\arg\min\sum_{i\in S_0}Q_i(x).\]
%Suppose a set $S_1\subset\{1,...,n\}\backslash S_0$ of $t$ agents has 
%\begin{equation*}
%    x_1\in\arg\min_x\sum_{i\in S_0\cup S_1}Q_i(x)
%\end{equation*}
%such that $\norm{x_0-x_1}=\epsilon$, while the remaining $t$ agents $S_2=\{1,...,n\}\backslash S_0\backslash S_1$ have
%\begin{equation*}
%    x_2\in\arg\min_x\sum_{i\in S_0\cup S_2}Q_i(x)
%\end{equation*}
%such that $\norm{x_0-x_2}=\epsilon$ and $\norm{x_1-x_2}=2\epsilon$.\\
%
%Consider a possible scenario where points $x_0$, $x_1$, and $x_2$ are collinear in the space $\R^d$. That is, there exists a unique straight line $L$ passing through all $x_0$, $x_1$, and $x_2$. Now, let $P$ be a hyperplane passing through $x_0$ and perpendicular to $L$. Suppose each cost function $Q_i(x)$, $i\in S_0$ is self-symmetric to $P$. To satisfy the conditions stated above, for every cost function $Q_i(x)$, $i\in S_1$, one can construct another function $Q_j(x)$ to be the cost function of an agent $j\in S_2$, such that $Q_i$ and $Q_j$ are also symmetric with respect to $P$.\\
%
%Suppose that a deterministic optimization algorithm $\Pi$ that is $(f,\epsilon-\delta)$-resilient, $\delta>0$. As the identity of Byzantine faulty agents is a priori unknown to the server, and the faulty cost functions are assumed differentiable and convex, $\Pi$ cannot distinguish between the following two possibilities: (1) $\mathcal{H}_{(1)}=S_0\cup S_1$ is the set of non-faulty agents, or (2) $\mathcal{H}_{(2)}=S_0\cup S_2$ is the set of non-faulty agents. 
%
%Suppose we are in scenario (1) where the honest agents are in the set $\mathcal{H}_{(1)}=S_0\cup S_1$. By $(2f,\epsilon)$-redundancy, $x_0\in B(x^*_{(1)},\epsilon)$, where $x^*_{(1)}\in\arg\min_x\sum_{i\in\mathcal{H}}Q_i(x)$, which is satisfied, since in this case, $x^*_{(1)}=x_1$. %Suppose $\mathcal{H}$ denotes the set of non-faulty agents in an execution of $\Pi$. Recall that $|\mathcal{H}|\geq n-f$ and $n>2f$. 
%The output $\widehat{x}$ of $\Pi$ would be within the ball $B(x_1,\epsilon-\delta)$.
%
%Now consider scenario (2) where the honest agents are in the set $\H_{(2)}=S_0\cup S_2$. Since $S_1$ and $S_2$ are symmetric, an optimum of aggregation of true cost functions from the honest agents is now $x_2\in\arg\min_{x}\sum_{i\in\H_{(2)}}Q_i(x)$. However, since $\Pi$ is deterministic and no function from any agent is changed, $\Pi$ would still output the same $\hat{x}$ as it would in scenario (1). The distance $\norm{x_2-\widehat{x}}\geq\epsilon+\delta>\epsilon$. Therefore, the output does not satisfy $(f,\epsilon)$-resilience. Contradiction.
\end{proof}

% The argument presented for the scalar case (when $d = 1$) in the above proof can be easily extended to the higher-dimensional case when $d>1$ as follows. The Byzantine faulty agents can choose cost functions such that the points $x_0$, $x_1$, and $x_2$ are collinear in the space $\R^d$. Thus, there exists a unique straight line $L$ passing through $x_0$, $x_1$, and $x_2$. Let $P$ be a hyperplane passing through $x_0$ and perpendicular to $L$. Suppose each cost function $Q_i(x)$, $i\in S_0$ is self-symmetric to $P$. To satisfy the conditions stated in the proof, for every cost function $Q_i(x)$, $i\in S_1$, a Byzantine agent $j \in S_2$ can concoct a function $Q_j(x)$ such that $Q_i$ and $Q_j$ are also symmetric with respect to hyperplane $P$.\\

In our {next key result} in Theorem~\ref{thm:suff} below {\bf we show that $(2f, \, \epsilon)$-redundancy is sufficient for $(f, \, 2\epsilon)$-resilience}. We make the following assumption on the differentiability of the cost functions.

\begin{assumption}
For each non-faulty agent $i$, we assume that the cost function $Q_i(x)$ is differentiable.
% the set $\arg\min_x Q_i(x)$ is a compact set.
\label{assum:compact}
\end{assumption}
% To formally present the sufficiency result we assume differentiability of the agents' cost functions.
% We also make the following assumption for the true cost functions:
Assumption~\ref{assum:compact} implies that for a non-empty subset $S$ of non-faulty agents, the aggregate function $\sum_{i\in S}Q_i(x)$ is also differentiable. The differentiability of the cost functions implies that their set of minimum points is {\em closed}~\cite{boyd2004convex}. Specifically, if $\sum_{i\in S}Q_i(x)$ is differentiable then the set $\arg \min_x \sum_{i\in S}Q_i(x)$ is closed.

\begin{theorem}[Sufficiency]
\label{thm:suff}
Suppose that Assumption~\ref{assum:compact} holds true. For a real value $\epsilon \geq 0$, if the non-faulty agents satisfy the $(2f,\epsilon)$-redundancy property then $(f,2\epsilon)$-resilience is achievable.
\end{theorem}

\begin{proof}

The proof is constructive where we assume that all the agents send their individual cost functions to the server. As all the non-faulty agents are assumed to have differentiable cost functions (see Assumption~\ref{assum:compact}), if the server receives a non-differentiable cost function from an agent then that agent must be faulty, and is eliminated from the system. However, we assume the worst-case scenario when all the Byzantine faulty agents will indeed send differentiable cost functions to the server. We also assume that $f > 0$ to avoid the trivial case of $f = 0$.\\

Specifically, we propose an algorithm constituting of the following three steps and show that it is $(f,2\epsilon)$-resilient under $(2f,\epsilon)$-redundancy. Recall that under Assumption~\ref{assum:compact}, for an arbitrary non-empty set of agents $S$ the set of minimum points of its aggregate cost function, i.e., $X_S = \arg\min_x\sum_{i\in\widehat{S}}Q_i(x)$, is closed. Thus, the Euclidean distance between an arbitrary point $x \in \R^d$ and $X_S$, is well defined. 
% Every agents send their cost function to the server. An honest agent sends its actual cost function, while a faulty agent sends an arbitrary function. The server iterates each set $S$ of the received functions of size $n-f$. For each set $S$, the server compute $x_S\in\arg\min_x\sum_{i\in S}Q_i(x)$. Furthermore, for each subset $\widehat{S}\subset S$, $\mnorm{\widehat{S}}=n-2f$, compute \[r_{S\widehat{S}}\triangleq\dist{x_S}{\arg\min_x\sum_{i\in\widehat{S}}Q_i(x)}.\]
% Let 
% \[r_S=\max_{\begin{subarray}{c}\widehat{S}\subset S,\\\mnorm{\widehat{S}}=n-2f\end{subarray}}r_{S\widehat{S}}~,\]
% for each $S$. The algorithm outputs the $x_S$ with minimum $r_S$.\\

\begin{description}
    \item[Step 1:] Each agent sends their cost function to the server. An honest agent sends its actual cost function, while a faulty agent may send an arbitrary function.
    \item[Step 2:] For each set $S$ of received functions, $\mnorm{S}=n-f$, the server computes a point
        \begin{equation*}
            x_S\in\arg\min_x\sum_{i\in S}Q_i(x).
        \end{equation*}
        For each subset $\widehat{S}\subset S$, $\mnorm{\widehat{S}}=n-2f$, the server computes 
        \begin{equation}
            r_{S\widehat{S}}\triangleq\dist{x_S}{\arg\min_x\sum_{i\in\widehat{S}}Q_i(x)}, \label{eqn:r_SS}
        \end{equation}
        and 
        \begin{equation}
            r_S=\max_{\begin{subarray}{c}\widehat{S}\subset S,\\\mnorm{\widehat{S}}=n-2f\end{subarray}}r_{S\widehat{S}.} \label{eqn:r_S}
        \end{equation}
    \item[Step 3:] The server outputs $x_S$ such that the set $S$ of $n-f$ agents has the smallest value of $r_S$ (with ties broken arbitrarily).
\end{description}

\noindent We show below that above algorithm is $(f, \, \epsilon)$-resilient. For a set of agents $S$, we denote 
\[X_S = \arg\min_x\sum_{i\in S}Q_i(x).\]
~

% the notation $X_S$ to denote the set $\arg\min_x\sum_{i\in S}Q_i(x)$.
Recall that there are at least $n-f$ non-faulty agents in the system. Thus, there exists a set $G$ with $\mnorm{G} = n-f$ comprising of only non-faulty agents. For set $G$, by definition of $(2f, \, \epsilon)$-redundancy (in Definition~\ref{def:approx_red}), for all $\widehat{S}\subset G$ with $\mnorm{\widehat{S}}=n-2f$, 
\begin{align}
    r_{G\widehat{S}}\leq\dist{X_G}{X_{\widehat{S}}}\leq\epsilon \implies r_G\leq\epsilon. \label{eqn:r_S_eps}
\end{align}
% \[r_{S\widehat{S}}\leq\dist{X_S}{X_{\widehat{S}}}\leq\epsilon.\] 
% Consequently, $r_S\leq\epsilon$.\\

Next, we separately consider the two possible cases.

\begin{description}
    \item[Case 1:] Suppose that the set $S$ associated with the output $x_S$ comprises only non-faulty agents. Then, by definition of $(2f,\epsilon)$-redundancy, $x_S$ is within $\epsilon$ distance from a minimum point of the aggregate non-faulty cost function.
    
    \item[Case 2:] Suppose that the set $S$ comprises of non-zero number of Byzantine faulty agents. From~\eqref{eqn:r_S_eps}, we note that there exists a set $G$ with $\mnorm{G}=n-f$ comprising of only non-faulty agents such that $r_G\leq\epsilon$. Thus, since the algorithm outputs $x_S$ instead of $x_G$, 
    \begin{align}
        r_S \leq r_G \leq \epsilon. \label{eqn:rsg}
    \end{align}
    As there are at most $f$ Byzantine faulty agents, there exists a subset $\widehat{S}\subset S$ with $\mnorm{\widehat{S}}=n-2f$ comprising of only non-faulty agents. From~\eqref{eqn:r_S} and~\eqref{eqn:r_S_eps}, note that $\dist{x_S}{X_{\widehat{S}}}\leq r_S$. Therefore, substituting from~\eqref{eqn:rsg}, 
    \[\dist{x_S}{X_{\widehat{S}}}\leq\epsilon.\]
    Therefore, there exists a point $x_{\widehat{S}}\in X_{\widehat{S}}$ such that 
    \begin{equation}
        \dist{x_S}{x_{\widehat{S}}}=\norm{x_S-x_{\widehat{S}}}\leq\epsilon. \label{eqn:case_2_1}
    \end{equation}
    For such as point $x_{\widehat{S}}$, $(2f, \epsilon)$-redundancy property implies that
        % Moreover, 
        % \begin{equation*}
        %     \dist{X_{\widehat{S}}}{X_\H}\leq\epsilon.
        % \end{equation*}
        % Therefore, 
        there exists a true minimum point $x^*$ of the aggregate non-faulty cost function such that
        \begin{equation}
            \dist{x_{\widehat{S}}}{x^*}=\norm{x_{\widehat{S}}-x^*}\leq\epsilon.
        \end{equation}
        Therefore, by triangle inequality, 
        \begin{equation*}
            \norm{x_S-x^*}\leq\norm{x_S-x_{\widehat{S}}}+\norm{x_{\widehat{S}}-x^*}\leq2\epsilon.
        \end{equation*}
\end{description}

Thus, the proposed algorithm guarantees $(f, \, 2\epsilon)$-resilience.
\end{proof}

%Before we proceed to necessity proof, we need the following lemmas:
%\begin{lemma}
%    For every non-empty subset $S$ of $\{1,...,n\}$, if 
%    \begin{equation}
%        \bigcap_{i\in S}\arg\min_xQ_i(x)\neq\varnothing,
%    \end{equation}
%    we have
%    \begin{equation}
%        \arg\min_x\sum_{i\in S}Q_i(x)=\bigcap_{i\in S}\arg\min_xQ_i(x).
%    \end{equation}
%    \label{lem:ele}
%\end{lemma}
%Proof for Lemma \ref{lem:ele} can be found in \cite{gupta2020fault}.

% The two theorems above show the correspondence between our definitions of approximated redundancy and resilience conditions, that if an approximated result of a distributed optimization problem in presence of Byzantine faulty agents in the system within certain bound to a true optimum can be obtained, the true cost functions must meet some kind of resilience conditions; and it is possible to obtain an approximated result, so long as the true cost functions have certain degree of resilience. 

% It is worth mentioning that the necessity and sufficiency statements we proved above are not symmetrical; the necessity condition is tighter.

Next, we present a gradient-descent based fault-tolerant distributed optimization algorithm and present it fault-tolerance property. The presented algorithm can be easily implemented for both server-based and peer-to-peer system architectures. For simplified presentation, we assume the server-based architecture. 

==> sufficiency_necessity_v2.tex <==
% \section{Approximate Fault-Tolerance}
% 
% In this section, we present the notion of approximate fault-tolerance. 

% Alternately, for the set of all non-faulty agents $\H$, a
% % if $\mathcal{B}\in\{1,...,n\}$ with $\mnorm{\mathcal{B}} \leq f$ denotes the set of faulty agents, and $\mathcal{H}=\{1,...,n\}\\\mathcal{B}$ denotes the set of non-faulty agents, 
% $(f, \,\epsilon)$-resilient distributed optimization algorithm outputs a point within a Euclidean distance of $\epsilon$ from the set of true minimums
% \[\arg\min_x\sum_{i\in\mathcal{H}}Q_i(x).\]

% In this paper, we show that for achieving $(f, \, \epsilon)$-resilience we only require a relaxed redundancy property named {\em $(2f, \, \epsilon)$-redundancy}, which is defined below, instead of the more stringent {$2f$-redundancy} property defined in Definition~\ref{def:red}  above. \\

% \subsection{Necessary and Sufficient Conditions for $(f, \, \epsilon)$-Resilience}
% \label{sub:cond_res}

% We first show in Theorem~\ref{thm:necc} that $(f,\epsilon)$-resilience can be achieved only if the non-faulty cost functions satisfy the {\em $(2f, \, \epsilon)$-redundancy} property, stated below in Definition~\ref{def:approx_red}, which is a relaxation of the {\em $2f$-redundancy} property introduced in our prior work \cite{gupta2020fault}. Then, in Theorem~\ref{thm:suff} we show that if the {\em $(2f, \, \epsilon)$-redundancy} property is satisfied then $(f, \, 2\epsilon)$-resilience is achievable. Throughout this section, we assume that $f > 0$, otherwise the problem becomes trivial.\\
We also assume that $f < n/2$. Lemma~\ref{lem:n_2f} below shows that $(f, \, \epsilon)$-resilience is impossible in general when $f \geq n/2$. Proof of Lemma~\ref{lem:n_2f} is easy, and can be found in Appendix~\ref{app:n_2f}.
% Before we show the necessity of the {\em $(2f, \, \epsilon)$-redundancy} property for $(f,\epsilon)$-resilience in Theorem~\ref{thm:necc}, we show below in Lemma~\ref{lem:n_2f} that $(f, \, \epsilon)$-resilience is impossible in general when $f \geq n/2$. Therefore, throughout the rest of this paper we assume that $f < n/2$. 

\begin{lemma}
\label{lem:n_2f}
If $f \geq n/2$ then there cannot exist a deterministic $(f, \, \epsilon)$-resilient algorithm for any $\epsilon \geq 0$.
\end{lemma}
% \begin{proof}
% We prove the lemma by contradiction. We consider a case when $n = 2$, $d = 1$, i.e., $Q_i: \R \to \R$ for all $i$, and all the cost functions have unique minimum points. Suppose that $f = 1$, and that there exists a deterministic $(f, \, \epsilon)$-resilient algorithm $\Pi$ for some $\epsilon \geq 0$. Without loss of generality, we suppose that agent $2$ is Byzantine faulty. We denote $x_1 = \arg \min_{x \in \R}Q_1(x)$. \\

% The Byzantine agent $2$ can choose to behave as a non-faulty agent with cost function $\widetilde{Q}_2(x) = Q_1(x - x_1 - 2\epsilon - \delta)$ where $\delta$ is some positive real value. Now, note that the minimum point of $\widetilde{Q}_2(x)$, which we denoted by $x_2$, is unique and equal to $x_1 + 2\epsilon + \delta$. Therefore, $\mnorm{x_1 - x_2} = 2 \epsilon + \delta > 2 \epsilon$. As the identity of Byzantine agent is a priori unknown, the server cannot distinguish between scenarios; (i) agent $1$ is non-faulty, and (ii) agent $2$ is non-faulty. Now, being deterministic algorithm, $\Pi$ should produce the same output in both the scenarios. In scenario (i), as $\Pi$ is assumed $(f, \, \epsilon)$-resilient, its output must lie in the interval $[x_1 - \epsilon, \, x_1 + \epsilon]$. Similarly, in scenario (ii), the output of $\Pi$ must lie in the interval $[x_2 - \epsilon, \, x_2 + \epsilon]$. However, as $\mnorm{x_1 - x_2} > 2\epsilon$, the two intervals  $[x_1 - \epsilon, \, x_1 + \epsilon]$ and $[x_2 - \epsilon, \, x_2 + \epsilon]$ do not overlap. Therefore, $\Pi$ cannot be $(f, \, \epsilon)$-resilient in both the scenarios simultaneously, which is a contradiction to the assumption that $\Pi$ is $(f, \, \epsilon)$-resilient. \\

% The above argument extends easily for the case when $n > 2$, and $f > n/2$.
% \end{proof}

\subsection{Necessary Condition}
% We first show below the {\bf necessity of $(2f, \, \epsilon)$-redundancy for $(f, \, \epsilon)$-resilience}. 

\begin{theorem}
\label{thm:necc}
% Suppose that the non-faulty cost functions are differentiable and convex. 
Suppose that Assumption~\ref{asp:exists} holds true. There exists a deterministic $(f, \,\epsilon)$-resilient distributed optimization algorithm where $\epsilon \geq 0$ {\em only if} the agents' cost functions satisfy the $(2f,\epsilon)$-redundancy property.
\end{theorem}

\begin{proof}

To prove the theorem we present a scenario when the agents' cost functions (if non-faulty) are scalar functions, i.e., $d = 1$ and for all $i$, $Q_i: \R \to \R$, and the minimum point of an aggregate of one or more agents' cost functions is uniquely defined. Obviously, if a condition is necessary in this particular scenario then it is so in the general case involving vector functions with non-unique minimum points.\\

% Second, our arguments can be easily extended for the case when $d > 1$. As the theorem is rendered vacuous when $f = 0$, we assume that $f > 0$.\\

To prove the necessary condition, we also assume that the server has full knowledge of all the agents' cost functions. This may not hold true in practice, where instead the server may only have partial information about the agents' cost functions. Indeed, this assumption forces the Byzantine faulty agents to a priori fix their cost functions. However, in reality the Byzantine agents may send arbitrary information over time to the server that need not be consistent with a fixed cost function. Thus, necessity of $(2f,\epsilon)$-redundancy under this strong assumption implies its necessity in general. \\

The proof is by contradiction. Specifically, we show that {\em If the non-faulty cost functions do not satisfy the $(2f,\epsilon)$-redundancy property then there cannot exist a {\em deterministic} $(f,\epsilon)$-resilient distributed optimization algorithm.}\\
% \begin{quote}
%     %If the non-faulty cost functions satisfy $(2f,\epsilon)$-redundancy for some $\epsilon$, deterministic distributed optimization algorithm cannot guarantee $(f,\epsilon-\delta)$-resilience, for any $\delta$, $0\geq\delta<\epsilon$.
%     %For some $\epsilon>0$, if the non-faulty cost functions do not satisfy $(2f,\epsilon)$-redundancy, deterministic distributed optimization algorithm cannot guarantee $(f,\epsilon)$-resilience.
%     %, for any $\delta$, $0\geq\delta<\epsilon$.
% 
% \end{quote}
% We show that the above statement is
% 
Recall that we have assumed that for a non-empty set of agents $T$ the aggregate cost function $\sum_{i \in T} Q_i(x)$ has a unique minimum point. To be precise, for each non-empty subset of agents $T$, we define
\[x_T = \arg \min_x \sum_{i \in T} Q_i(x).\]

Suppose that the agents' cost functions {\bf do not} satisfy the $(2f,\epsilon)$-redundancy property stated in Definition~\ref{def:approx_red}. 
Then, there exists a real number $\delta > 0$ and a pair of subsets $S, \, \widehat{S}$ with $\widehat{S} \subset S$, $\mnorm{S} = n-f$, and $n-2f \leq \mnorm{\widehat{S}} < n-f$ such that
% there exits a pair of sets $S, \, \widehat{S} \subseteq \{1, \ldots, \, n\}$ with $\mnorm{S} \geq n-f$, $\mnorm{\widehat{S}} \geq n-2f$ and $\widehat{S} \subseteq S$ such that 
% \begin{align*}
%     \norm{x_{\widehat{S}} - x_S} = \epsilon + \delta
% \end{align*}
% where $\delta > 0$. As shown in Lemma~\ref{lem:red_imply} presented in Appendix~\ref{app:red_imply}, the above implies that 
% there exists a pair of sets $T, \, \widehat{T} \subset \{1, \ldots, \, n\}$ with $\mnorm{T} = n-f$, $\mnorm{\widehat{T}} = n-2f$ and $\widehat{T} \subset T$ such that
\begin{align}
    \norm{x_{\widehat{S}} - x_S} \geq \epsilon + \delta. \label{eqn:no_red_asp}
\end{align}
% \textcolor{red}{\bf ++++ editing +++++ }
% \\
% For a subset $S_0$ comprising of $n-2f$ non-faulty agents, suppose that the minimum point of the aggregated cost function of the agents in $S_0$ is unique. We denote
% \begin{equation}
%     x_0=\arg\min\sum_{i\in S_0}Q_i(x).
% \end{equation}
% Let set $S_1$ denote the remaining $f$ non-faulty agents. Suppose that the minimum point of the aggregated cost function of all the non-faulty agents in $S_0 \cup S_1$ is also unique. We denote
% % A set $S_1\subset\{1,...,n\}\backslash S_0$ of $t$ agents has
% \begin{equation}
%     x_1=\arg\min_x\sum_{i\in S_0\cup S_1}Q_i(x)
% \end{equation}
% As we have assumed that the non-faulty agents do not satisfy the $(2f,\epsilon)$-redundancy, there exist the aforementioned sets $S_0$ and $S_1$, and $\delta > 0$, such that $x_0$ is $\epsilon + \delta$ distance away from $x_1$, i.e.,
% \begin{align*}
%     \norm{x_0 - x_1} = \epsilon + \delta.
% \end{align*}
Now, suppose that $n - f - \mnorm{\widehat{S}}$ agents in the remainder set $\{1, \ldots, \, n\} \setminus S$ are Byzantine faulty. Let us denote the set of faulty agents by $\B$. Note that $\B$ is non-empty with $\mnorm{\B} = n - f - \mnorm{\widehat{S}} \leq f$. 
% Now, let all the remaining $f$ agents in the set $\B = \{1, \ldots, \, n\} \setminus S$ be Byzantine faulty. 
Similar to the non-faulty agents, the faulty agents send to the server cost functions that are scalar, and the aggregate of one of more agents' cost functions in the set $S \cup \B$ is unique. However, 
\begin{quote}
the aggregate cost function of the agents in the set $\B \cup \widehat{S}$ minimizes at a unique point $x_{\B \cup \widehat{S}}$ which is $\norm{x_{\widehat{S}} - x_{S}}$ distance away from $x_{\widehat{S}}$, similar to $x_S$, but lies on the other side of $x_{\widehat{S}}$ as shown in the figure below. Note that it is always possible to pick such functions for the faulty agents.
\end{quote}

% The remaining $f$ agents denoted by set $S_2 = \{1,...,n\} \setminus S_0 \setminus S_1$ are Byzantine faulty. A Byzantine faulty agent $i \in S_2$ chooses a cost function $Q_i(x): \R \to \R$ with similar properties as a non-faulty cost function such that the following conditions hold true. 
% \begin{itemize}
%     \item The minimum point of the aggregated cost function of the agents in $S_0 \cup S_2$ is unique. We denote 
%     \begin{equation*}
%         x_2=\arg\min_x\sum_{i\in S_0\cup S_2}Q_i(x).
%     \end{equation*}
%     \item The distance between $x_0$ and $x_2$ is $\epsilon + \delta$, i.e., $\norm{x_0 - x_2} = \epsilon + \delta$. However, the point $x_2$ lies in the other half of the real line $\R$ than the point $x_1$ as shown in the figure below.
% \end{itemize}

\begin{center}
    \begin{tikzpicture}
        \node[dot] (x1) at (-2,0) {};
        \node[dot] (x0) at (0,0) {};
        \node[dot] (x2) at (2,0) {};
        \node at (-2,-.35) {$x_S$};
        \node at (0,-.35) {$x_{\widehat{S}}$};
        \node at (2,-.35) {$x_{\B \cup \widehat{S}}$};
        \draw (-4,0) -- (x0)
              (x0) -- (4,0);
        %\node[dot] at (-2,0) {};
        %\node[dot] at (2,0) {};
              
        %\node[dot, color=red] (xhat) at (-1.7,0) {};
        %\node at (-1.7,-.4) {\textcolor{red}{$x^*_{(1)}$}};
        %\node[dot, color=red] (xhat2) at (1.6,0) {};
        %\node at (1.6,-.4) {\textcolor{red}{$x^*_{(2)}$}};
        
        \node at (-.3,0) {]};
        \node at (-3.7,0) {[};
        \node at (-1,.36) {\footnotesize\textcolor{blue}{$\leftarrow\epsilon+\delta\rightarrow$}};
        \node at (1,.36) {\footnotesize\textcolor{blue}{$\leftarrow\epsilon+\delta\rightarrow$}};
        \node at (-1.2,-.3) {\textcolor{blue}{\footnotesize $\epsilon$}};
        \node at (-2.8,-.3) {\textcolor{blue}{\footnotesize $\epsilon$}};

        \node[dot, color=red] (xhat) at (-.5,0) {};
        \node at (-.5,-.4) {\textcolor{red}{$\widehat{x}$}};
        \label{fig:illustrate}
    \end{tikzpicture}
\end{center}

\noindent Note that the distance between the two points $x_S$ and $x_{\B \cup \widehat{S}}$ is $2\epsilon + 2\delta$, i.e.,
\begin{align}
    \norm{x_S - x_{\B \cup \widehat{S}}} = 2\epsilon + 2\delta. \label{eqn:dist_x1_x2}
\end{align}
% The functions can be constructed. Suppose each cost function $Q_i(x)$, $i\in S_0$ satisfies $Q_i(x)=Q_i(2x_0-x)$. To satisfy the conditions stated above, for every cost function $Q_i(x)$, $i\in S_1$, one can construct another function $Q_j(x)=Q_i(2x_0-x)$, to be the cost function of an agent $j\in S_2$. \\%(See Figure~\ref{fig:constructQ})\\
%$\distance(x_0,x_1)=\distance(x_0,x_2)=\epsilon$. And functions in $S_0$, $S_1$, and $S_2$ are symmetric with respect to $x_0$, meaning for any $Q_i$ in $X_0$, $Q_i(x)=Q_i(2x_0-x)$, and for any $Q_i\in S_1$ and $Q_j\in S_2$, $Q_i(x)=Q_j(2x_0-x),~\forall x$. \\
% We now show below, by contradiction, that there cannot exist a deterministic $(f, \, \epsilon)$-resilient algorithm.\\

Now, suppose, toward a contradiction, that there exists an $(f, \, \epsilon)$-resilient deterministic optimization algorithm named $\Pi$. As the identity of Byzantine faulty agents is a priori unknown to the server, and the cost functions sent by the Byzantine faulty agents have similar properties as the non-faulty agents, 
% and the faulty cost functions are assumed differentiable and convex, 
the server cannot distinguish between the following two possible scenarios; i) $S$ is the set of non-faulty agents, and ii) $\B \cup \widehat{S}$ is the set of non-faulty agents. Note that both the sets $S$ and $\B \cup \widehat{S}$ contain $n-f$ agents. \\
% Thus, the output of algorithm $\Pi$ assumed to be $(f, \, \epsilon)$-resilient should be located within $\epsilon$ distance from the minimum point of the aggregate cost functions of the non-faulty agents in both the scenarios. \\

As the cost functions received by the server are identical in both of the above scenarios, being a deterministic algorithm, $\Pi$ should have identical output in both the cases. We let $\widehat{x}$ denote the output of $\Pi$. In scenario (i) when the set of honest agents is given by $S$ with $\mnorm{S} = n-f$, as $\Pi$ is assumed $(f,\epsilon)$-resilient, by Definition~\ref{def:approx_res} the output
\begin{align}
    \widehat{x} \in  [x_S - \epsilon, \, x_S + \epsilon] \label{eqn:scn_1}
\end{align}
as shown in the figure above. Similarly, in scenario (ii) when the set of honest agents is $\B \cup \widehat{S}$ with $\mnorm{\B \cup \widehat{S}} = n-f$,
\begin{align}
    \widehat{x} \in  [x_{\B\cup \widehat{S}} - \epsilon, \, x_{\B\cup \widehat{S}} + \epsilon]. \label{eqn:scn_2}
\end{align}
However,~\eqref{eqn:dist_x1_x2} implies that~\eqref{eqn:scn_1} and~\eqref{eqn:scn_2} cannot be satisfied simultaneously. That is, if $\Pi$ is $(f,\epsilon)$-resilient in scenario (i) then it cannot be so in scenario (ii), and vice-versa. This contradicts the assumption that $\Pi$ is $(f, \, \epsilon)$-resilient. \qedhere
% , and therefore proves the impossibility of $(f, \, \epsilon)$-resilience when the $(2f, \, \epsilon)$-redundancy property is violated.

% By $(2f,\epsilon+\delta)$-redundancy, since $\mnorm{\H_{(0)}}=n-f$ while $\mnorm{S_0}=n-2f$, we should have
% \[\dist{\arg\min_x\sum_{i\in\H_{(1)}}Q_i(x)}{\arg\min_x\sum_{i\in S_0}Q_i(x)}\leq(\epsilon+\delta).\] %Suppose $\mathcal{H}$ denotes the set of non-faulty agents in an execution of $\Pi$. Recall that $|\mathcal{H}|\geq n-f$ and $n>2f$. 
% Note that $\arg\min_x\sum_{i\in\H_{(1)}}Q_i(x)=x_1$ and $\arg\min_x\sum_{i\in S_0}Q_i(x)=x_0$, the condition above is satisfied. On the other hand, since $\Pi$ is $(f,\epsilon)$-resilient, the output $\widehat{x}$ of $\Pi$ would be within range $[-\epsilon+x_1,\epsilon+x_1]$, as shown in the figure below.\\


% Now consider scenario (2) where the honest agents are in the set $\mathcal{H}_{(2)}=S_0\cup S_2$. Since $S_1$ and $S_2$ are symmetric, the optimum of aggregation of true cost functions from honest agents is now $x_2=\arg\min_x\sum_{i\in\mathcal{H}_{(2)}}Q_i(x)$. However, since $\Pi$ is deterministic and all functions from agents are not changed, it would still output the same $\widehat{x}$ as it would in scenario (1). The distance $\norm{x_2-\widehat{x}}>\epsilon+\delta>\delta$. Therefore, $\widehat{x}$ does not satisfy $(f,\epsilon)$-resilience. Contradiction.
%
%%%%%%%%%%%%%%% Vector Case %%%%%%%%%%%%%%%%
%\begin{center}
%    $\mathsection~~~\mathsection~~~\mathsection$
%\end{center} 
%
%We consider a subset $S_0$ comprising of $n-2f$ non-faulty agents, and denote by $x_0$ a minimum point of the aggregate costs of the agents in $S_0$. Specifically, 
%\[x_0\in\arg\min\sum_{i\in S_0}Q_i(x).\]
%Suppose a set $S_1\subset\{1,...,n\}\backslash S_0$ of $t$ agents has 
%\begin{equation*}
%    x_1\in\arg\min_x\sum_{i\in S_0\cup S_1}Q_i(x)
%\end{equation*}
%such that $\norm{x_0-x_1}=\epsilon$, while the remaining $t$ agents $S_2=\{1,...,n\}\backslash S_0\backslash S_1$ have
%\begin{equation*}
%    x_2\in\arg\min_x\sum_{i\in S_0\cup S_2}Q_i(x)
%\end{equation*}
%such that $\norm{x_0-x_2}=\epsilon$ and $\norm{x_1-x_2}=2\epsilon$.\\
%
%Consider a possible scenario where points $x_0$, $x_1$, and $x_2$ are collinear in the space $\R^d$. That is, there exists a unique straight line $L$ passing through all $x_0$, $x_1$, and $x_2$. Now, let $P$ be a hyperplane passing through $x_0$ and perpendicular to $L$. Suppose each cost function $Q_i(x)$, $i\in S_0$ is self-symmetric to $P$. To satisfy the conditions stated above, for every cost function $Q_i(x)$, $i\in S_1$, one can construct another function $Q_j(x)$ to be the cost function of an agent $j\in S_2$, such that $Q_i$ and $Q_j$ are also symmetric with respect to $P$.\\
%
%Suppose that a deterministic optimization algorithm $\Pi$ that is $(f,\epsilon-\delta)$-resilient, $\delta>0$. As the identity of Byzantine faulty agents is a priori unknown to the server, and the faulty cost functions are assumed differentiable and convex, $\Pi$ cannot distinguish between the following two possibilities: (1) $\mathcal{H}_{(1)}=S_0\cup S_1$ is the set of non-faulty agents, or (2) $\mathcal{H}_{(2)}=S_0\cup S_2$ is the set of non-faulty agents. 
%
%Suppose we are in scenario (1) where the honest agents are in the set $\mathcal{H}_{(1)}=S_0\cup S_1$. By $(2f,\epsilon)$-redundancy, $x_0\in B(x^*_{(1)},\epsilon)$, where $x^*_{(1)}\in\arg\min_x\sum_{i\in\mathcal{H}}Q_i(x)$, which is satisfied, since in this case, $x^*_{(1)}=x_1$. %Suppose $\mathcal{H}$ denotes the set of non-faulty agents in an execution of $\Pi$. Recall that $|\mathcal{H}|\geq n-f$ and $n>2f$. 
%The output $\widehat{x}$ of $\Pi$ would be within the ball $B(x_1,\epsilon-\delta)$.
%
%Now consider scenario (2) where the honest agents are in the set $\H_{(2)}=S_0\cup S_2$. Since $S_1$ and $S_2$ are symmetric, an optimum of aggregation of true cost functions from the honest agents is now $x_2\in\arg\min_{x}\sum_{i\in\H_{(2)}}Q_i(x)$. However, since $\Pi$ is deterministic and no function from any agent is changed, $\Pi$ would still output the same $\hat{x}$ as it would in scenario (1). The distance $\norm{x_2-\widehat{x}}\geq\epsilon+\delta>\epsilon$. Therefore, the output does not satisfy $(f,\epsilon)$-resilience. Contradiction.
\end{proof}

% The argument presented for the scalar case (when $d = 1$) in the above proof can be easily extended to the higher-dimensional case when $d>1$ as follows. The Byzantine faulty agents can choose cost functions such that the points $x_0$, $x_1$, and $x_2$ are collinear in the space $\R^d$. Thus, there exists a unique straight line $L$ passing through $x_0$, $x_1$, and $x_2$. Let $P$ be a hyperplane passing through $x_0$ and perpendicular to $L$. Suppose each cost function $Q_i(x)$, $i\in S_0$ is self-symmetric to $P$. To satisfy the conditions stated in the proof, for every cost function $Q_i(x)$, $i\in S_1$, a Byzantine agent $j \in S_2$ can concoct a function $Q_j(x)$ such that $Q_i$ and $Q_j$ are also symmetric with respect to hyperplane $P$.\\

% Next, we show that $(2f, \, \epsilon)$-redundancy suffices for $(f, \, 2\epsilon)$-resilience.

\subsection{Sufficient Condition}

% We make the following assumption on the differentiability of the cost functions.

% \begin{assumption}
% For each non-faulty agent $i$, we assume that the cost function $Q_i(x)$ is differentiable.
% \label{assum:compact}
% \end{assumption}
% Assumption~\ref{assum:compact} implies that for a non-empty subset $S$ of non-faulty agents, the aggregate function $\sum_{i\in S}Q_i(x)$ is also differentiable. The differentiability of the cost functions implies that their set of minimum points is {\em closed}~\cite{boyd2004convex}. Specifically, if $\sum_{i\in S}Q_i(x)$ is differentiable then the set $\arg \min_x \sum_{i\in S}Q_i(x)$ is closed.

\begin{theorem}
% [Sufficiency]
\label{thm:suff}
Suppose that Assumption~\ref{asp:exists} holds true. 
For a real value $\epsilon \geq 0$, if the agents' cost functions satisfy the $(2f,\epsilon)$-redundancy property then $(f,2\epsilon)$-resilience is achievable.
\end{theorem}

\begin{proof}

The proof is constructive where we assume that all the agents send their individual cost functions to the server. We assume that $f > 0$ to avoid the trivial case of $f = 0$. Throughout the proof we write the notation $\arg \min_{x \in \R^d}$ simply as $\arg \min$, unless otherwise stated.
% As all the non-faulty agents are assumed to have differentiable cost functions (see Assumption~\ref{assum:compact}), if the server receives a non-differentiable cost function from an agent then that agent must be faulty, and is eliminated from the system. However, 
% We assume the worst-case scenario when all the Byzantine faulty agents will indeed send differentiable cost functions to the server. 
We begin by presenting an algorithm below, comprising three steps.

% We present below an algorithm constituting of three steps and then show that it is $(f,2\epsilon)$-resilient under $(2f,\epsilon)$-redundancy. 
% Recall that under Assumption~\ref{assum:compact}, for an arbitrary non-empty set of agents $S$ the set of minimum points of its aggregate cost function, i.e., $X_S = \arg\min_x\sum_{i\in\widehat{S}}Q_i(x)$, is closed. Thus, the Euclidean distance between an arbitrary point $x \in \R^d$ and $X_S$, is well defined. 
% Every agents send their cost function to the server. An honest agent sends its actual cost function, while a faulty agent sends an arbitrary function. The server iterates each set $S$ of the received functions of size $n-f$. For each set $S$, the server compute $x_S\in\arg\min_x\sum_{i\in S}Q_i(x)$. Furthermore, for each subset $\widehat{S}\subset S$, $\mnorm{\widehat{S}}=n-2f$, compute \[r_{S\widehat{S}}\triangleq\dist{x_S}{\arg\min_x\sum_{i\in\widehat{S}}Q_i(x)}.\]
% Let 
% \[r_S=\max_{\begin{subarray}{c}\widehat{S}\subset S,\\\mnorm{\widehat{S}}=n-2f\end{subarray}}r_{S\widehat{S}}~,\]
% for each $S$. The algorithm outputs the $x_S$ with minimum $r_S$.\\

\begin{description}
    \item[Step 1:] Each agent sends their cost function to the server. An honest agent sends its actual cost function, while a faulty agent may send an arbitrary function.
    \item[Step 2:] For each set $T$ of received functions, $\mnorm{T}=n-f$, the server computes a point
        \begin{equation*}
            x_T\in\arg\min \sum_{i\in T}Q_i(x).
        \end{equation*}
        For each subset $\widehat{T}\subset T$, $\mnorm{\widehat{T}}=n-2f$, the server computes 
        \begin{equation}
            r_{T\widehat{T}}\triangleq\dist{x_T}{\arg\min \sum_{i\in\widehat{T}}Q_i(x)}, \label{eqn:r_SS}
        \end{equation}
        and 
        \begin{equation}
            r_T=\max_{\begin{subarray}{c}\widehat{T}\subset T,\\\mnorm{\widehat{T}}=n-2f\end{subarray}}r_{T\widehat{T}.} \label{eqn:r_S}
        \end{equation}
    \item[Step 3:] The server outputs $x_S$ such that 
    \begin{align}
        S = \underset{\begin{subarray}{c}T \subset \{1, \ldots, \, n\},\\ \mnorm{T} = n-f\end{subarray}}{\arg \min} r_T. \label{eqn:out_S}
    \end{align}
    % the set $S$  of $n-f$ agents has the smallest value of $r_S$ (with ties broken arbitrarily).
\end{description}

\noindent We show that above algorithm is $(f, \, 2\epsilon)$-resilient under $(2f, \, \epsilon)$-redundancy. For a non-empty set of agents $T$, we denote 
\[X_T = \arg\min \sum_{i\in T}Q_i(x).\]
~

% the notation $X_S$ to denote the set $\arg\min_x\sum_{i\in S}Q_i(x)$.
Consider an arbitrary set of non-faulty agents $G$ with $\mnorm{G} = n-f$. Such a set is guaranteed to exist as there are at most $f$ faulty agents, and therefore, at least $n-f$ non-faulty agents exist in the system.
% Recall that there are at least $n-f$ non-faulty agents in the system. Thus, there exists a set $G$ with $\mnorm{G} = n-f$ comprising of only non-faulty agents. 
Consider an arbitrary set $\widehat{T}$ such that $\widehat{T}\subset G$ and $\mnorm{\widehat{T}}=n-2f$. By Definition~\ref{def:approx_red} of $(2f, \, \epsilon)$-redundancy, 
\begin{align}
    \dist{X_G}{X_{\widehat{T}}}\leq\epsilon. \label{eqn:G_T_eps}
\end{align}
Recall from~\eqref{eqn:r_SS} that $r_{G \widehat{T}} = \dist{x_G}{X_{\widehat{T}}}$. As $x_G \in X_G$, by Definition~\eqref{eqn:hausdorff} of Hausdorff set distance, $\dist{x_G}{X_{\widehat{T}}} \leq \dist{X_G}{X_{\widehat{T}}}$. Therefore, $r_{G \widehat{T}} \leq \dist{X_G}{X_{\widehat{T}}}$, and
% \begin{align*}
%     r_{G \widehat{T}} \leq \dist{X_G}{X_{\widehat{T}}}.
% \end{align*}
substituting from~\eqref{eqn:G_T_eps} implies that
\begin{align}
    r_{G \widehat{T}} \leq \epsilon.  \label{eqn:r_G_T}
\end{align}
Now, recall from~\eqref{eqn:r_S} that $r_G = \max\left\{r_{G\widehat{T}} ~ \vline ~ \widehat{T}\subset G, \, \mnorm{\widehat{T}}=n-2f \right\}$.
% \[r_G = \max_{\begin{subarray}{c}\widehat{T}\subset G,\\\mnorm{\widehat{T}}=n-2f\end{subarray}} r_{G\widehat{T}}.\]
As $\widehat{T}$ in~\eqref{eqn:r_G_T} is an arbitrary subset of $G$ with $\mnorm{\widehat{T}}=n-2f$, 
\begin{align}
    r_G = \max_{\begin{subarray}{c}\widehat{T}\subset G,\\\mnorm{\widehat{T}} = n-2f\end{subarray}} r_{G\widehat{T}}  ~ \leq ~ \epsilon. \label{eqn:r_S_eps}
\end{align}
% \[r_{S\widehat{S}}\leq\dist{X_S}{X_{\widehat{S}}}\leq\epsilon.\] 
% Consequently, $r_S\leq\epsilon$.\\
From~\eqref{eqn:out_S} and~\eqref{eqn:r_S_eps} we obtain that
\begin{align}
    r_S \leq r_G \leq \epsilon. \label{eqn:rsg}
\end{align}

As $\mnorm{G} = n-f$, for every set of agents $T$ with $\mnorm{T} = n-f$, $\mnorm{T \cap G} \geq n-2f$. Therefore, for the set $S$ defined in~\eqref{eqn:out_S}, there exists a subset $\widehat{G}$ of $G$ such that $\widehat{G} \subset S$ and $\mnorm{\widehat{G}} = n-2f$. For such a set $\widehat{G}$, by definition of $r_S$ in~\eqref{eqn:r_S}, we obtain that
\begin{align*}
    r_{S\widehat{G}} \triangleq \dist{x_S}{X_{\widehat{G}}} \leq r_S.
\end{align*}
Substituting from~\eqref{eqn:rsg} above, we obtain that 
\begin{align}
    \dist{x_S}{X_{\widehat{G}}}\leq\epsilon. \label{eqn:dist_bnd_eps}
\end{align}
As $\widehat{G}$ is a subset of $G$, all the agents in $\widehat{G}$ are non-faulty. Therefore, by Assumption~\ref{asp:exists}, $X_{\widehat{G}}$ is a closed set. Recall that $\dist{x_S}{X_{\widehat{G}}} = \inf_{x \in X_{\widehat{G}}} \norm{x_S - x}$. The closedness of $X_{\widehat{G}}$ implies that there exists a point $z \in X_{\widehat{G}}$ such that 
\[\norm{x_S - z} = \inf_{x \in X_{\widehat{G}}} \norm{x_S - x} = \dist{x_S}{X_{\widehat{G}}}.\]
The above, in conjunction with~\eqref{eqn:dist_bnd_eps}, implies that
\begin{align}
    \norm{x_S - z} \leq \epsilon. \label{eqn:pt_1}
\end{align}
Moreover, as $z \in X_{\widehat{G}}$ where $\widehat{G} \subset G$ with $\mnorm{\widehat{G}} = n-2f$ and $\mnorm{G} = n-f$, the $(2f, \, \epsilon)$-redundancy condition stated in Definition~\ref{def:approx_red} implies that $\dist{z}{X_G} \leq \epsilon$.
% \begin{align*}
%     \dist{z}{X_G} \leq \epsilon. 
% \end{align*}
Similar to an argument made above, under Assumption~\ref{asp:exists}, $X_G$ is a closed set, and therefore, there exists $x^* \in X_G$ such that
\begin{align}
    \norm{z - x^*} = \dist{z}{X_G} \leq \epsilon.  \label{eqn:pt_2}
\end{align}
% Consider an arbitrary set of $n-f$ non-faulty agents $\H$. Such a set if guar
% As there are at most $f$ Byzantine faulty agents, there exists a subset $\widehat{S}\subset S$ with $\mnorm{\widehat{S}}=n-2f$ comprising of only non-faulty agents. From~\eqref{eqn:r_S} and~\eqref{eqn:r_S_eps}, note that $\dist{x_S}{X_{\widehat{S}}}\leq r_S$. Therefore, substituting from~\eqref{eqn:rsg}, 
% \begin{align}
%     \dist{x_S}{X_{\widehat{S}}}\leq\epsilon. \label{eqn:dist_bnd_eps}
% \end{align}
% As $\widehat{S}$ is a set comprising only non-faulty agents, $X_{\widehat{S}}$ is a closed set by Assumption~\ref{asp:exists}. Thus,~\eqref{eqn:dist_bnd_eps} implies that there exists a point $x_{\widehat{S}}\in X_{\widehat{S}}$ such that 
% \begin{equation}
%     \dist{x_S}{x_{\widehat{S}}}=\norm{x_S-x_{\widehat{S}}}\leq\epsilon. \label{eqn:case_2_1}
% \end{equation}
% For such as a point $x_{\widehat{S}}$, due to $(2f, \epsilon)$-redundancy,
%         % Moreover, 
%         % \begin{equation*}
%         %     \dist{X_{\widehat{S}}}{X_\H}\leq\epsilon.
%         % \end{equation*}
%         % Therefore, 
% there exists a point $x^*$ that minimizes the aggregate cost function of $n-f$ non-faulty agents such that
% \begin{equation}
%     \dist{x_{\widehat{S}}}{x^*}=\norm{x_{\widehat{S}}-x^*}\leq\epsilon. \label{eqn:case_2_2}
% \end{equation}
By triangle inequality,~\eqref{eqn:pt_1} and~\eqref{eqn:pt_2} implies that $\norm{x_S - x^*} \leq \norm{x_S-z} + \norm{z - x^*} \leq 2\epsilon$.
% \begin{equation}
%     \norm{x_S - x^*} \leq \norm{x_S-z} + \norm{z - x^*} \leq 2\epsilon. \label{eqn:final_suff_proof}
% \end{equation}
Recall that set $G$ here is an arbitrary set of $n-f$ non-faulty agents. 
% Therefore,~\eqref{eqn:final_suff_proof} proves the theorem.
% proposed algorithm is $(f, \, 2\epsilon)$-resilient.
% \begin{align}
%     r_S \leq r_G \leq \epsilon.
% \end{align}
% Now, we separately consider the two possibilities below.
% \textcolor{red}{++++ editing ++++} \\
% \begin{description}
%     \item[Case 1:] Suppose that the set $S$ associated with the output $x_S$ comprises only non-faulty agents. Then, $x_S$ is a minimum point of the aggregate cost function of at least $n-f$ non-faulty agents, and therefore the algorithm is obviously $(f, \, \epsilon)$-resilient.
%     \item[Case 2:] Suppose that the set $S$ comprises of non-zero number of Byzantine faulty agents. From~\eqref{eqn:r_S_eps}, we note that there exists a set $G$ with $\mnorm{G}=n-f$ comprising of only non-faulty agents such that $r_G\leq\epsilon$. Thus, since the algorithm outputs $x_S$ instead of $x_G$, 
% \end{description}
\end{proof}

%Before we proceed to necessity proof, we need the following lemmas:
%\begin{lemma}
%    For every non-empty subset $S$ of $\{1,...,n\}$, if 
%    \begin{equation}
%        \bigcap_{i\in S}\arg\min_xQ_i(x)\neq\varnothing,
%    \end{equation}
%    we have
%    \begin{equation}
%        \arg\min_x\sum_{i\in S}Q_i(x)=\bigcap_{i\in S}\arg\min_xQ_i(x).
%    \end{equation}
%    \label{lem:ele}
%\end{lemma}
%Proof for Lemma \ref{lem:ele} can be found in \cite{gupta2020fault}.

% The two theorems above show the correspondence between our definitions of approximated redundancy and resilience conditions, that if an approximated result of a distributed optimization problem in presence of Byzantine faulty agents in the system within certain bound to a true optimum can be obtained, the true cost functions must meet some kind of resilience conditions; and it is possible to obtain an approximated result, so long as the true cost functions have certain degree of resilience. 

% It is worth mentioning that the necessity and sufficiency statements we proved above are not symmetrical; the necessity condition is tighter.

In the next part of the paper, i.e., Sections~\ref{sec:grad_des} and~\ref{sec:experiments}, we consider the case when the (non-faulty) agents' cost functions are differentiable. Specifically, we study approximate fault-tolerance in the distributed gradient-descent (DGD) method. 
% The presented fault-tolerance can be easily implemented for both server-based and peer-to-peer system architectures. For simplified presentation, we assume the server-based architecture. 
